How does unlabeled data improve generalization in self-training? A one-hidden-layer theoretical analysis

Self-training, a semi-supervised learning algorithm, leverages a large amount of unlabeled data to improve learning when the labeled data are limited. Despite empirical successes, its theoretical characterization remains elusive. To the best of our knowledge, this work establishes the first theoretical analysis for the known iterative self-training paradigm and proves the benefits of unlabeled data in both training convergence and generalization ability. To make our theoretical analysis feasible, we focus on the case of one-hidden-layer neural networks. However, theoretical understanding of iterative self-training is non-trivial even for a shallow neural network. One of the key challenges is that existing neural network landscape analysis built upon supervised learning no longer holds in the (semi-supervised) self-training paradigm. We address this challenge and prove that iterative self-training converges linearly with both convergence rate and generalization accuracy improved in the order of $1/\sqrt{M}$, where $M$ is the number of unlabeled samples. Experiments from shallow neural networks to deep neural networks are also provided to justify the correctness of our established theoretical insights on self-training.

==> Self-training (6)/Introduction.tex <==
\section{Introduction}

\iffalse
\SL{[Prefer to start this paragraph directly with \textbf{Self-training}]}
In practice, generating a large size of reliable labels is either expensive or unavailable, which leads to the study of semi-supervised learning (SSL) \SL{[Not a good terminology as SSL could be confused with self-supervised learning; maybe {\Semi}]} \citep{GVV13,CSZ09,Joa03,ZGL03}.
The goal of SSL algorithms is to thus suppress the demand on the labeled data through exploiting the unlabeled data. 
Due to the easy access of the unlabeled data, research has seen the diversified developments of the SSL approaches \citep{Yar95,GB05,LA16,SBCZZRCKL20,LWHL19}, and the key differences lie in how to generate or make use of the unlabeled data. 
Self-training,  one of the most powerful ssl algorithms, which first utilizes the teacher model obtained from a small set of labeled data to generate the pseudo labels for a large set of unlabeled data, and then the teacher model is re-trained through the joint labeled and unlabeled data \citep{Scu65,Yar95,Lee13,HLW19}.
\SL{[Better to be more specific on applications: E.g., {\Semi} for few-shot image classification \citep{su2020does},   robustness-aware model training against adversarial attacks \citep{CRSD19}, continual lifelong learning \citep{lee2019overcoming}]}
\fi

Self-training \citep{Scu65,Yar95,Lee13,HLW19}, one of the most powerful \underline{semi}-\underline{s}upervised \underline{l}earning (SemiSL) algorithms, augments a limited number of labeled data with  unlabeled data so as to achieve
%to learn a model that has
improved   generalization performance   on test data, compared with the model trained by  supervised learning using the labeled data only.  %suppress the demand for the labeled data and thus achieve considerable or even better performance than supervised learning with limited number of labeled data. Due to the easy access of unlabeled data, research has seen the success
%Because labeled data are often costly to obtain, while unlabeled data are usually vastly available, 
Self-training has shown empirical success in diversified applications such as few-shot image classification \citep{su2020does,XLHL20,CKSNH20,YJCPM19,ZGLC20}, objective detection \citep{RHS05}, robustness-aware model training against adversarial attacks \citep{CRSD19}, continual lifelong learning \citep{lee2019overcoming}, and natural language processing \citep{HGSR19,klh20}.  The terminology ``self-training'' has been used to describe various SemiSL algorithms in the literature, while this paper is centered on  the commonly-used iterative   self-training method in particular.  In this setup, an  initial teacher model (learned from the labeled data) is applied to the unlabeled data to generate pseudo labels. One then trains a student model   by minimizing the weighted empirical risk of both the labeled and unlabeled data. The student model is then used as the new teacher to update the pseudo labels of the unlabeled data. This process is repeated multiple times to improve the eventual student model. {We refer readers to Section \ref{sec: problem} for algorithmic details.}
%Finally, the student model acts as the new teacher model and repeat the steps above several times.    


Despite the empirical achievement of self-training  methods {with neural networks}, the theoretical justification of such success is very limited, even in the field of SemiSL. % was established.
% This approach enlarges the training data by introducing the pseudo label and benefits the training performance with the enlarged  dataset, and recent work \citep{ZGLC20} suggests that self-training is more efficient than pre-training  based methods in using extra datasets. 
% In spite of the numerical success through self-training based methods, theoretical understanding of how the unlabeled data affect the generalization performance via iterative self-training algorithms are still unknown.
% The authors in \citep{BMB10} show that unlabeled data can reduce the hypothesis space size and thus improve the generalization bound \citep{BM02}. However, the analysis \tcr{cannot be extended to modern neural network learning problems without additional restrictions on the weights space}. 
% %Even enlarging to the field of SemiSL via pseudo-labels, one can see 
The majority of the theoretical results on general SemiSL are limited to linear networks \citep{CWKM20,RXYDL20, OG20, OADAR11}.  
 The authors in \citep{BMB10} 
 show that unlabeled data can improve the generalization bound if the unlabeled data distribution and target model are compatible. For instance, the unlabeled data need to be well-chosen such that the target function for labeled data can separate the unlabeled data clusters, which, however, may not be able to be verified ahead.
% show that unlabeled data can reduce the hypothesis space size and thus improve the generalization bound \citep{BM02}.
% However, the data distribution and target model need to be compatible. %needs to satisfy a good notation of compatibility. 
% For instance, the unlabeled data are %needs to be
% clustered, and not all the models in the hypothesis set can separate the clusters, which leads to a restriction of the hypothesis space. %needs to be able to well separate the clusters.}
\Revise{Moreover, \citep{Rig07,SNZ08} proves that unlabeled data can improve the convergence rate and generalization error under a similar clustering assumption, where the data contains clusters that have homogeneous labels. 
A recent work by \citet{WSCM20}   analyzes SemiSL on nonlinear neural networks  and proves that an infinite number of unlabeled data can improve the generalization compared with training with labeled data only.}  
However, \citet{WSCM20} considers  single shot  rather than iterative SemiSL, and the training problem aims to  minimize the consistency regularization rather than the risk function in the conventional self-training method \citep{Lee13}. Moreover, 
% no discussion is provided about what algorithm to find the global optimum of the nonconvex training problem in 
\citet{WSCM20}  directly analyzes  the global optimum of the nonconvex training problem without any discussion about how to achieve the global optimum.   To the best of our knowledge, there exists no analytical characterization of how the unlabeled data affect the generalization of the learned model by iterative self-training on nonlinear neural networks. 


%To the best of our knowledge, \citet{WSCM20} is the most relevant work with proof that infinite many unlabeled data can improve the performance over training with only labeled data, 
%however,  there are still significant differences with the iterative self-training method studied in this paper. First, built upon the assumption of input consistency, the learning problem in \citep{WSCM20} is to minimize a weighted sum of the consistency regularization rather than the risk function of the labeled and unlabeled data, which differs from the conventional self-training method \citep{Lee13}. Second, although the existence of the improved model via solving the optimization problem with additional unlabeled data are confirmed in \citep{WSCM20},
%the attainability of such minimizers via existing algorithms are missing. Third, the framework in \citep{WSCM20} is based on one-shot method and cannot directly provide insight for iterative self-training methods. To this end, theoretical explanations for iterative self-training algorithms are still absent.}

\begin{wrapfigure}{r}{0.42\textwidth}
    \vspace{-4mm}
   	\centering
   	\includegraphics[width=1.0\linewidth]{Figure/real.pdf}
   	\vspace{-2mm}
     \caption{The trend of test accuracy improvement (\%) on CIFAR-10 by self-training  on CIFAR-10 (labeled) with different amount of unlabeled data from 80 Million Tiny Images matches our theoretical prediction.}
     \label{fig: intro}
     \vspace{-4mm}
\end{wrapfigure}
\textbf{Contributions.} This paper provides the first theoretical study of iterative self-training on nonlinear neural networks. Focusing on one-hidden-layer neural networks, this paper provides a quantitative analysis of the generalization performance of iterative self-training as a function of the number of labeled and unlabeled samples. 
%\tcr{In this paper, we focus on studying finite number of unlabeled data in improving the generalization via iterative self-training. In brief, this paper characterizes the convergence analysis of self-training method given limited labeled data and provides quantitative analysis of the unlabeled data amount on improving generalization accuracy and convergence rate. 
Specifically, our contributions include
% Moreover, we develop the new techniques in analyzing the performance of iterative self-training algorithm in low labeled data regime, where the number of labeled data is not sufficiently large to guarantee zero generalization error in supervised learning. 
% \PY{(why improving training? it's a bit confusing to me. I thought it directly deals with generalization)}

% \begin{wrapfigure}{r}{0.45\textwidth}
%     \vspace{-4mm}
%   	\centering
%   	\includegraphics[width=1.0\linewidth]{Figure/landscape.png}
%     \caption{Landscape of the generalization function, and the objective functions with/without unlabeled data. \SL{After taking a second thought, do you think it is better to place this figure in Sec. 3.1?}
%     \PY{Should we put Fig. 8 and Fig. 1 Together as a teaser graph?}
%     }
%     \label{fig: landscape_1}
%     \vspace{-5mm}
% \end{wrapfigure}
\textbf{1. Quantitative justification of generalization improvement by unlabeled data.} Assuming the existence of a ground-truth model with weights $\bfW^*$ that maps the features to the corresponding labels, we prove that the learned model {via iterative self-training} moves closer to $\bfW^*$ as the number $M$ of unlabeled data increases, indicating a better testing performance. Specifically, we prove that the Frobenius distance to $\bfW^*$, which is approximately linear in the generalization error, decreases in the order of $1/\sqrt{M}$. 
{As an example, Figure\,\ref{fig: intro} shows that the   proposed theoretical bound matches the empirical self-training performance versus the number of unlabeled data for image classification; see details in Section \ref{sec: result_practice}.}
%and this theoretical bound matches the empirical observation such as Figure    \ref{fig: intro}. %One intuitive explanation of the advantage of using unlabeled data with pseudo labels is that with the additional second term, 

% The intuition is that with more unlabeled data, the landscape of the empirical risk becomes smoother near  $\bfW^*$, and starting from a nearby initialization, the gradient descent method converges to a local minimum that is closer to $\bfW^*$.  We quantify the distance of the learned model to $\bfW^*$ analytically as  a function of  the numbers of labeled and unlabeled samples.

%The increase of unlabeled data can compress the landscape of the objective function and force the local minima near the initial point towards the ground truth, as shown in Figure \ref{fig: landscape_1}(a) and (b), and thus the generalization error is improved. However, the improvements from increasing unlabeled data are not sufficient to achieve zero generalization error.  In particular, we characterize the distance of the convergent local minima to the ground truth and provide quantitative analysis of the number of unlabeled data in improving the generalization error in Theorem \ref{Thm: p_convergence}.

\textbf{2. Analytical justification of iterative self-training over single shot alternative.}  We prove that the student models returned by the iterative self-training method \textit{converges linearly} to a model close to $\bfW^*$, {with the rate improvement in the order of $1/\sqrt{M}$}. 

%with limited number of labeled data, and the rate of convergence improves in the order of $1/\sqrt{M}$, indicating a faster convergence when $M$ increases.  Thus, the iterative approach enhances the generalization of the learned model over the single-shot alternatives.


%and the convergence rate becomes faster if we have larger size of labeled or unlabeled data.

\textbf{3. Sample complexity analysis of labeled and unlabeled data for learning a proper model.} 
{We quantify the impact of labeled and unlabeled data on the generalization of the learned model. In particular, we prove that the sample complexity of labeled data   can be reduced compared with supervised learning.}
% We quantify the impact of labeled and unlabeled data on the generalization of the learned model.  In particular, when the number of labeled data is less than the sample complexity requirement of existing works in supervised learning, we show that self-training still returns a model with reasonable generalization error. 
% \SL{[did not understand it. You want to say:
% We prove that even in the self-training paradigm, the number of labeled data  also matters. We prove that if xxx, then self-training still suffers a non-trivial generalization error. ?
% ]}
%With limited number of labeled data, we provide the required number of unlabeled data to guarantee the learned model is improved over the preliminary teacher model.  
% In addition, the sample complexity for unlabeled data decreases if we increase the number of labeled data. 
%Moreover, given sufficient   unlabeled data, we prove that the sample complexity of labeled data for reaching zero generalization error is reduced compared with supervised learning methods. 

%\textbf{3. Convergence analysis of iterative self-training algorithm.}
%This paper, for the first time, proves that the iterations from iterative self-training algorithm converge linearly to some local minima with limited number of labeled data,
%and the convergence rate becomes faster if we have larger size of labeled or unlabeled data.

\iffalse
The Neural network has attracted the attentions in recent years for its state-of-the-art performance in solving machine learning problems. Although the generalization error, which defers to the difference of test accuracy and training accuracy, is not fully understood and bounded,
recent theoretical works suggest that, with enough training samples, the generalization error is negligible or even zero \citep{BG17,ZSJB17,ZWLC20_1,ZWLC20_2}. However, generating a large size of reliable labels in practice is either expensive or unavailable, which leads to the study of semi-supervised learning (SSL) \citep{GVV13,CSZ09,Joa03,ZGL03}.
The goal of semi-SL algorithms is to thus suppress the demand on the labeled data through exploiting the unlabeled data. Due to the easy access of the unlabeled data, research has seen the diversified developments of the semi-SL approaches \citep{Yar95,GB05,LA16,SBCZZRCKL20,LWHL19,MMLI18}, and the key differences lie in how to generate and make use of the unlabeled data. 

Self-training,  one of the most powerful semi-SL algorithms, which first utilizes the teacher model obtained from a small set of labeled data to generate the pseudo labels for a large set of unlabeled data, and then the teacher model is re-trained through the joint labeled and unlabeled data \citep{Scu65,Yar95,Lee13,HLW19}.
This approach enlarges the training data by introducing the pseudo label and benefits the training performance with the enlarged  dataset, and recent work \citep{ZGLC20} suggests that self-training is more efficient than pre-training  based methods in using extra datasets.
 In spite of the numerical success through self-training based methods \citep{SBLZCCKZR20, XLHL20, CKSNH20, YJCPM19,HGSR19,klh20}, theoretical understanding of how the unlabeled data affect the training process are still unknown \citep{WSCM20}, especially self-training approaches require an explanation for that unlabeled data indeed reduce the dependency of labeled data.
\fi


% Based on the number of labeled data, we consider three cases: (1) low labeled data regime, where the learned model cannot converge to the ground truth with no matter how many unlabeled data; (2) moderate labeled data regime, where the learned model can only converge to the ground truth with sufficient number of unlabeled data; (3) high labeled data regime, where the learned model can converge to the ground truth without any unlabeled data. As the third case has been studied in \citep{ZSJB17} and its relative works, this paper focus on the first two cases. 




% Under the framework of consistency regularization, recent work \citep{WSCM20} studies non-linear model and prove that the unlabeled data can improve the performance over the model trained via pure labeled data. The consistency regularization are built upon the assumption that the output are stable to small perturbations on the input, and thus the margins among different classes need to be sufficiently large. In this sense, introducing unlabeled data benefits the training process mainly from digging the information from the large margins. Therefore, the objective function in \citep{WSCM20} is a weighted sum of consistency regularizer and risk function for fitting unlabeled data, which, however, differs from the traditional self-training method \citep{Lee13}.

% However, to the best of our knowledge, there are only limited number of 
% of the theoretical results in the field of self-training \citep{CWKM20,RXYDL20, OG20, OADAR11, WSCM20}. All the works among the works mentioned above, except \citep{WSCM20}, only study the learning problems with linear activation functions. Under the expansion and separation assumptions for labeled data,
% \citep{WSCM20} proves that unlabeled data indeed improves the test accuracy. Compared with \citep{WSCM20}, this paper characterizes the  order dependence of the generalization error and convergence rate with the number of unlabeled data quantitatively. Additionally, \citep{WSCM20} only provides the sample complexity analysis for unsupervised learning problems when
% the labeled data have sufficiently large margins between different classes, and the sample complexity is a polynomial function of the margins. While this paper considers regression problems and  presents the sample complexity bound for self-training methods, and the bound is a linear function of the input dimension, which is order-wise optimal as well.


% \textit{Notations.}
% %Vectors are bold lowercase, matrices and tensors are bold uppercase.  Scalars are in normal font, and sets are in calligraphy and blackboard bold font. 
% %  $\bfI$ denote the identity matrix. $\mathbb{N}$ and $\mathbb{R}$ denote the sets of nature number and  real number, respectively.
% $\|\bfz\|$ denotes the $\ell_2$-norm of a vector $\bfz$, and $\|\bfZ\|_2$, $\|\bfZ\|_F$ and $\|\bfZ\|_{\infty}$ denote the spectral norm, Frobenius norm and maximum value of the matrix $\bfZ$, respectively.
% [$Z$] stands for the set of $\{ 1, 2, \cdots, Z  \}$ for any number $Z\in\mathbb{N}$.
% In addition, $f(r)=\mathcal{O}(g(r))$ (or $f(r)=\Omega(g(r))$) if  $f\le C\cdot g$ (or $f\ge C\cdot g$) for some constant $C>0$ when $r$ is large enough. $f(r)=\Theta(g(r))$ if both $f(r)=\mathcal{O}(g(r))$ and $f(r)=\Omega(g(r))$ holds, where $c\cdot g \le f \le C\cdot g$ for some constant $0\le c\le C$ when $r$ is large enough.


\subsection{Related works}\label{sec: related}
% \textbf{Self-training.} Self-training is one of the most popular SSL methods and can achieve similar or even better performance with a relative small size of labeled data by taking advantages of the unlabeled data.  The majority of the theoretical results are limited to linear classifiers \citep{CWKM20,RXYDL20, OG20, OADAR11}. By introducing the compatibility of the risk function, the authors in \citep{BMB10} are able to prove that unlabeled data can reduce the hypothesis space size and thus improve the generalization bound \citep{BM02}, however, the analyses are limited to
% Principal Component Analysis (PCA) problems. Only the authors in \citep{WSCM20} studies the non-linear model under the assumptions of  expansion and separation for the input data. 
% \tcr{However, \citep{WSCM20} only provides the sample complexity analysis for unsupervised learning problems when
% the labeled data have sufficiently large margins between different classes, and the sample complexity is a polynoimal function of the margins. While this paper considers regression problems and  presents the sample complexity bound for self-training methods, and the bound is a linear function of the input dimension, which is order-wise optimal as well.}
% However,  compared with unsupervised learning, the theoretical results in \citep{WSCM20} imply that self-training may require higher assumptions for the convergence, and the population risk is not guaranteed to be improved by using unlabeled data. 

\textbf{Semi-supervised learning.}  Besides self-training, many recent SemiSL algorithms exploit either consistency regularization or entropy minimization.  Consistency regularization is  based on the assumption that the learned model will return same or similar output when the input is perturbed \citep{LA16,BAP14,SJT16,TV17,RLASER15}.  \citep{GB05}  claims that the unlabeled data are more informative if the 
pseudo labels of the unlabeled data have lower entropy. Therefore, a line of works \citep{GB05,MMKI18} adds a regularization term that minimizes the entropy of the outputs of the unlabeled data. % which is named as entropy minimization approach. 
In addition, hybrid algorithms that unify both the above regularizations have been developed like  \citep{BCNKSZR19,BCGOR19,SBCZZRCKL20}. % methods above are common as well and are included in \citep{BCNKSZR19,BCGOR19,SBCZZRCKL20} to name a few.

\textbf{Domain adaptation.} Domain adaptation exploits abundant data in the source domain to learn a model for the target domain, where only limited training data are available \citep{LS10,VLMPG13,ZSMW13,LCWJ15,THZSD14}. Source and target domain are related but different. Unsupervised domain adaptation \citep{GL15,GUAGLLML16,GGS13,BTSKE16}, where   training data in target domain are unlabeled,  is similar to SemiSL, and self-training   methods have been used  for analysis \citep{ZYKW18,TRLK12,FMF18}. % to analyze such problems due to its similarity to SemiSL \citep{ZYKW18,TRLK12,FMF18}.
However,  self-training and unsupervised domain adaptation are fundamentally different. The former   learns a model for the domain where there is limited labeled data, with the help of a large number of \textit{unlabeled} data from a different domain.  The latter learns a model for the domain where the training data are unlabeled, with the help of sufficient \textit{labeled} data from a different domain. 

\iffalse
analyzes the problem such that the training processes are accessible to an only limited number of data from the target domain but plenty of data from a different distribution, named source domain.
% , and the goal is to learn a model that generalizes well for data in the target domain. 
For unsupervised domain adaptation where the data in target domain are unlabeled \citep{GL15,GUAGLLML16,GGS13,BTSKE16},  self-training based methods become the powerful tools to analyze such problems due to its similarity to SemiSL \citep{ZYKW18,TRLK12,FMF18}. However, self-training method aims for a model that generalizes well for the labeled data space with small size, while unsupervised domain adaptation are available to plenty of labeled data from source domain and seeks a way to modify the learned model such that it has guaranteed performance for the unlabeled data in target domain. 
% The fundamental difference leads to the  separations in theoretical analysis, and the generalization bound for domain adaptation mainly relies on the ``domain gap'', which is measured by the divergence between the distributions of the data in source and target domains \citep{BBJKK10,GGS13,ZDZG19,JSR19,CMM15,GHLF16,ZTLJ19}. 
% Therefore, bounded domain gap becomes a common assumption in domain adaptation \citep{DLLP10}, which, however, is irrelevant and unnecessary in SSL settings.
\fi

\textbf{Generalization analysis of supervised learning.}
% \SL{[Needs a better paragraph title. Generalization ability analysis?]}
In theory, the testing error is upper bounded by the training error plus the generalization gap between training and testing. These two quantities are often analyzed separately and cannot be proved to be small simultaneously for deep neural networks. For example, neural tangent kernel (NTK) method \citep{JGH18,DZPS18,LBNSSPS18} shows the training error can be zero, and the Rademacher complexity in \citep{BM02} bounds  the generalization gap \citep{ADHLW19}. For one-hidden-layer neural networks \citep{SS18}, the testing error can be proved to be zero under mild conditions. One common assumption is that the input data belongs to the Gaussian distribution \citep{ZSJB17,GLM17,kkms08,BJW19,ZLJ16,BG17,LY17,SJL18}. Another line of approaches \citep{BGM18,LL18,WGC19} consider  linearly separable data.
%study the convergence analysis under the framework of structured data, i.e., the data are assumed to be linear separable.

\iffalse 
In the field of theoretical works, few techniques \citep{ALL19} can understand the behaviors of  multi-layer neural networks with characterized generalization. Even for shallow neural networks \citep{SS18}, to provide bounded generalization analysis, a widely used assumption in the community is that the input data belongs to the Gaussian distribution \citep{ZSJB17,GLM17,kkms08,BJW19,ZLJ16,BG17,LY17,SJL18}. Another popular line of approaches \citep{BGM18,LL18,WGC19} study the convergence analysis under the framework of structured data, i.e., the data are assumed to be linear separable.
% Overall, even in the field of supervised learning, the performance of stochastic gradient descent algorithm in solving non-convex neural network training problems have not been fully understood yet. 
\fi 

The rest of this paper is organized as follows. %Section \ref{sec: related} briefly discusses some related works.
Section \ref{sec: problem} introduces the problem formulation and self-training algorithm. Major results are summarized in Section \ref{sec: theoretical}, and empirical evaluations are presented in Section \ref{sec: empirical_results}. Section \ref{sec: conclusion} concludes the whole paper.
All the proofs are in the Appendix.



% \begin{figure}[H]
%   	\centering
%   	\includegraphics[width=0.90\linewidth]{Figure/Influence_M_N_Part2.pdf}
%     \caption{}
%     \label{fig: Convergence analysis}
% \end{figure}

==> Self-training (6)/Proof.tex <==
\section{Proof of Theorem \ref{Thm: p_convergence}}
\label{sec: insuff}
% \begin{wrapfigure}{r}{0.40\linewidth}
%      \centering
%      \vspace{-4mm}
%      \includegraphics[width=1.0\linewidth]{Figure/sketch_proof.pdf}
%      \caption{The landscapes of the objection function and population risk function.}
%      \vspace{-4mm}
%      \label{fig: landscape}
% \end{wrapfigure}
Instead of proving Theorem \ref{Thm: p_convergence}, we turn to prove a stronger version, as shown in Theorem \ref{Thm: p_main_thm}. \Revise{One can verify that Theorem \ref{Thm: p_convergence} is a special case of Theorem \ref{Thm: p_main_thm} by  selecting $\hat{\lambda}$ in the order of $p$ and $\w[\varepsilon]$ is in the order of $(2p-1)$.}

The major idea in proving Theorem \ref{Thm: p_main_thm} is similar to that of Theorem \ref{Thm: sufficient_number}.
The first step is
to characterize the gradient descent term on the population risk function by \Revise{the MVT in Lemma \ref{Lemma: MVT}} as shown in \eqref{eqn: Thm1_temp1} and \eqref{eqn: Thm1_temp2}.  Then,  the connection between $\|\W[\ell+1,0] -\Wp \|_F$  and $\|\W[\ell,0]-\Wp\|_F$ are characterized in \eqref{eqn:p_outer_loop}. Compared with proving Theorem \ref{Thm: sufficient_number}, where the induction over $\ell$ holds naturally with large size of labeled data, the induction over $\ell$ requires a proper value of $p$ as shown in \eqref{eqn_temp: 2.2}. By induction over $\ell$ on \eqref{eqn:p_outer_loop}, the relative error $\| \W[L,0] -\Wp \|_F$ can be characterized by $\|\W[0,0] -\Wp\|_F$ as shown in \eqref{eqn:p_outer_loop_2}.
\begin{theorem}\label{Thm: p_main_thm}
    Suppose the initialization $\W[0,0]$  satisfies 
    with 
    \begin{equation}\label{eqn: p_0}
       \Revise{|p -\hat{\lambda}| \le\frac{2(1-\w[\varepsilon])p-1}{\mu\sqrt{K}}}
    \end{equation}
    for some constant $\w[\varepsilon]\in (0, 1/2)$, where
    \begin{equation}
        \hat{\lambda} : =\frac{\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2}
        = \big(\frac{N}{\kappa^2\gamma K^3\mu^2 d \log q}\big)^{\frac{1}{2}} 
    \end{equation}
    and 
    \begin{equation}
        \mu
        = \mu( \delta, \de) 
        = \frac{\lambda\delta^2+\w[\lambda]\de^2}{\lambda\rho(\delta)+\w[\lambda]\rho(\de)}.
    \end{equation}
    Then, if the number of samples in $\w[\mathcal{D}]$ further satisfies
    % \begin{equation}\label{eqn: p_main_sample}
    % \begin{split}
    %     &N= \Omega\Big( \varepsilon^{-2}\mu^{2}\big(\frac{\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2}\big)^2K^3 d\log q \Big),\\
    %     \end{split}
    % \end{equation}
    \begin{equation}
        \begin{split}
        M \gtrsim \tilde{\varepsilon}^{-2} \kappa^2\gamma \mu^2 \big( 1-  \hat{\lambda}\big)^2 K^3 d\log q,
        \end{split}
    \end{equation}
    the iterates $\{ \bfW^{(\ell,t)} \}_{\ell,t=0}^{L,T}$ converge to $\bfW^{[p]}$ with $p$ satisfies \eqref{eqn: p_0} as 
    % \begin{equation}\label{eqn: ap_convergence}
    %     \begin{split}
    %         \lim_{\substack{\ell\to \infty\\ t\to \infty}} \| \W[\ell,t]-\overline{\bfW}(p^*) \|_F \le \frac{1}{1-(1+p^*K^{-1})\w[\varepsilon]}\cdot\Big(\frac{1-p^*}{K}  + {\mu\sqrt{K}\cdot|p^*-\hat{\lambda}|}\Big)\cdot \| \bfW^* - \bfW^{(0,0)} \|_F
    %     \end{split}
    % \end{equation}
    \begin{equation}\label{eqn: ap_convergence}
        \begin{split}
    &\lim_{T\to \infty}\| \bfW^{(\ell, T)} -\Wp \|_2\\
    \le& \Revise{\frac{1}{1-\tilde{\varepsilon}} \cdot \Big( {1-p^*} +\mu\sqrt{K}\big|(\hat{\lambda}-p^*)\big| \Big)\cdot\|\W[0,0]-\bfW^* \|_2 
    +\frac{\tilde{\varepsilon} }{(1-\tilde{\varepsilon})}\cdot\|\W[\ell,0]-\Wp \|_2,}
    \end{split}
    \end{equation}
    with probability at least $1-q^{-d}$.
\end{theorem}

\begin{proof}[Proof of Theorem \ref{Thm: p_main_thm}]
     From Algorithm \ref{Algorithm: Alg1}, in the $\ell$-th outer loop, we have 
    \begin{equation}\label{eqn: Thm1_temp1}
    \begin{split}
       \W[\ell, t+1] 
       =&  \W[\ell, t] -\eta \nabla\hat{f}_{\mathcal{D}_t,\widetilde{\mathcal{D}}_t}
       (\W[\ell, t])+\beta (\W[\ell, t] - \W[\ell, t-1])\\
       = & \W[\ell, t] -\eta \nabla{f}(\W[\ell, t])+\beta (\W[\ell, t] - \W[\ell, t-1])\\
       &+ \eta \cdot \Big( \nabla f(\W[\ell, t]) - \nabla \hat{f}_{\mathcal{D}_t,\widetilde{\mathcal{D}}_t}(\W[\ell, t]) \Big)
    \end{split}
    \end{equation}
    Since $\nabla f$ is a smooth function and $\Wp$ is a local (global) optimal to $f$, then we have 
    \Revise{\begin{equation}\label{eqn: Thm1_temp2}
        \begin{split}
            \nabla{f}(\W[\ell, t])
            =& \nabla{f}(\W[\ell, t]) - \nabla{f}(\Wp)\\
            =& \int_{0}^1 \nabla^2 f\Big(\bfW^{(\ell,t)} + u \cdot(\bfW^{(\ell,t)}-\Wp)\Big) du\cdot (\W[\ell, t]-\Wp),
        \end{split}
    \end{equation}
    where the last equality comes from Lemma \ref{Lemma: MVT}.}
    
    Similar to the proof of Theorem \ref{Thm: sufficient_number}, we have 
    \begin{equation}
        \| \bfW^{(\ell, t+1)} -\Wp \|_2 \le \|\bfA(\beta) \|_2 \cdot \|\bfW^{(\ell, t)}-\Wp \|_2  + \eta \cdot \|\nabla f(\W[\ell, t]) - \nabla \hat{f}_{\mathcal{D}_t,\widetilde{\mathcal{D}}_t}(\W[\ell, t]) \|_2.
    \end{equation}
    From Lemma \ref{Lemma: p_first_order_derivative}, we have 
    \begin{equation}
        \begin{split}
                &\|\nabla f(\W[\ell, t]) - \nabla \hat{f}(\W[\ell, t]) \|_2\\
            \lesssim& \frac{\lambda\delta^2}{K} \sqrt{\frac{d\log q}{N_t}} \cdot \| \W[\ell, t] - \bfW^*\| + \frac{\w[\lambda]\de^2}{K} \sqrt{\frac{d\log q}{M_t}} \cdot \| \W[\ell, t] -\W[\ell,0] \|_2\\
       & + \frac{\big| \lambda\delta^2 \cdot (\bfW^{(0,0)} -\Wp) -\w[\lambda]\de^2\cdot (\bfW^* - \Wp)  \big|}{K} \\
        \end{split}
    \end{equation}
    When $\ell = 0$, following the similar steps from \eqref{eqn:Heavy_ball_quaratic} to \eqref{eqn: beta},  we have 
    \begin{equation}
    \begin{split}
    &\|\nabla f(\W[\ell, t]) - \nabla \hat{f}(\W[\ell, t]) \|_2\\
        \lesssim & \frac{\lambda\delta^2}{K} \sqrt{\frac{d\log q}{N_t}} \cdot \| \W[\ell, t] - \Wp\| + \frac{\w[\lambda]\de^2}{K} \sqrt{\frac{d\log q}{M_t}} \cdot \| \W[\ell, t] -\Wp \|_2\\
      & + \frac{\lambda\delta^2}{K} \sqrt{\frac{d\log q}{N_t}} \cdot \| \bfW^* - \Wp\| + \frac{\w[\lambda]\de^2}{K} \sqrt{\frac{d\log q}{M_t}} \cdot \| \W[0,0] -\Wp \|_2\\
       & + \frac{\big| \lambda\delta^2 \cdot (1-p) -\w[\lambda]\de^2\cdot p  \big|}{K}\cdot\|\W[0,0]-\bfW^* \|_2
        \end{split}
    \end{equation}
    and
    \begin{equation}
    \begin{split}
        &\| \bfW^{(\ell, t+1)} -\Wp \|_2 \\
    \le& \Big( 1- \frac{1-\tilde{\varepsilon}}{\mu(\delta,\de)\sqrt{154\kappa^2\gamma K}} \Big) \cdot \|\W[\ell, t] -\Wp \|_2\\
    &+ \eta \cdot \Big( \frac{ \lambda \delta^2 (1-p) }{K} \sqrt{ \frac{d\log q}{N_t} }  + \frac{\big| \lambda \delta^2 \cdot(1-p)  -\w[\lambda]\de^2\cdot p  \big|}{K} \Big)\cdot\|\W[0,0]-\bfW^* \|_2\\
    &+\eta \cdot
    \frac{\tilde{\varepsilon} \w[\lambda]\de^2 \cdot p}{K}\cdot\sqrt{\frac{d\log q}{M_t}} \|\W[0,0]-\bfW^* \|_2.
    \end{split}
    \end{equation}
    Therefore, we have 
    \begin{equation}\label{eqn:p_outer_loop}
        \begin{split}
            &\lim_{T\to \infty}\| \bfW^{(\ell, T)} -\Wp \|_2\\
            \le&  \frac{\mu\sqrt{154\kappa^2\gamma K}}{1-\tilde{\varepsilon}} \cdot \eta \cdot
            \Big[ \Big(\frac{ \lambda \delta^2 (1-p) }{K} \sqrt{ \frac{d\log q}{N_t} }  + \frac{\big| \lambda\delta^2 \cdot(1-p)  -\w[\lambda]\de^2\cdot p  \big|}{K}\Big) \cdot\|\W[0,0]-\bfW^* \|_2\\
            &\qquad\qquad\qquad\qquad\qquad+
    \frac{\tilde{\varepsilon} \w[\lambda]\de^2 \cdot p}{K}\cdot\sqrt{\frac{d\log q}{M_t}} \cdot\|\W[0,0]-\bfW^* \|_2\Big]\\
    \le& 
    \frac{\mu\sqrt{154\kappa^2\gamma K}}{1-\tilde{\varepsilon}}\cdot \frac{{K}}{14 (\lambda\delta^2+\w[\lambda]\de^2 )}\cdot
    \Big[ \Big(\frac{ \lambda \delta^2 (1-p) }{K} \sqrt{ \frac{d\log q}{N_t} }  + \frac{\big| \lambda\delta^2 \cdot(1-p)  -\w[\lambda]\de^2\cdot p  \big|}{K}\Big)\\
    &\qquad\qquad\qquad\qquad\qquad \cdot\|\W[0,0]-\bfW^* \|_2 + 
    \frac{\tilde{\varepsilon} \w[\lambda]\de^2 \cdot p}{K}\cdot\sqrt{\frac{d\log q}{M_t}} \cdot\|\W[0,0]-\bfW^* \|_2\Big]\\
    \simeq & \Revise{\frac{1}{1-\tilde{\varepsilon}} \cdot \Big(  {1-p} +\sqrt{K}\cdot\big|(1-p)\mu\hat{\lambda} - p\mu(1-\hat{\lambda})\big| \Big)\cdot\|\W[0,0]-\bfW^* \|_2}\\
    &{+\frac{\tilde{\varepsilon} p}{(1-\tilde{\varepsilon})}\cdot\|\W[0,0]-\bfW^* \|_2}\\
    =&
    {\frac{1}{1-\tilde{\varepsilon}} \cdot \Big( {1-p} +\mu\sqrt{K}\big|\widehat{\lambda}-p\big| \Big)\cdot\|\W[0,0]-\bfW^* \|_2 
    +\frac{\tilde{\varepsilon} p}{(1-\tilde{\varepsilon})}\cdot\|\W[0,0]-\bfW^* \|_2},
    \end{split}
    \end{equation}
    where $\hat{\lambda} = \frac{\lambda\delta^2}{\lambda\delta^2 + \w[\lambda]\de^2}$.
    
    To guarantee the convergence in the outer loop, we require 
    \begin{equation}\label{eqn_temp: 2.1}
    \begin{split}
    &\lim_{T\to \infty}\|\W[\ell, T] -\Wp \|_2  \le \|\W[0,0]-\Wp \|_2 = p\|\W[0,0]-\bfW^* \|_2,\\
    \quad \text{and}\quad    &\lim_{T\to \infty}\| \bfW^{(\ell, T)} -\bfW^* \|_2 \le \|\W[0,0]-\bfW^* \|_2.
        \end{split}
    \end{equation}
    Since we have 
    \begin{equation}
        \begin{split}
        \| \bfW^{(\ell, T)} -\Wp \|_2  
        \le& \| \bfW^{(\ell, T)} - \bfW^* \|_2+ \| \bfW^*-\Wp \|_2 \\
        =& \| \bfW^{(\ell, T)} - \bfW^* \|_2 + (1-p)\cdot \| \bfW^*-\W[0,0] \|_2,
        \end{split}
    \end{equation}
    it is clear that \eqref{eqn_temp: 2.1} holds if and only if
    {\begin{equation}
        \frac{1}{1-\tilde{\varepsilon}} \cdot \Big( {1-p} + {\w[\varepsilon]p} +\mu\sqrt{K}\big|\hat{\lambda}-p\big| \Big) + 1-p \le 1.
    \end{equation}}
    To guarantee the iterates strictly converges to the desired point, we let 
    {\begin{equation}
        \frac{1}{1-\tilde{\varepsilon}} \cdot \Big( {1-p} + {\w[\varepsilon]p} +\mu\sqrt{K}\big|\hat{\lambda}-p\big| \Big) + 1-p \le 1 - \frac{1}{C}
    \end{equation}}
    for some larger constant $C$,
    which is equivalent to 
    {\begin{equation}\label{eqn_temp: 2.2}
        |p -\hat{\lambda}| \le\frac{2(1-\w[\varepsilon])p-1}{\mu\sqrt{K}}.
    \end{equation}}
    % when $K$ is sufficiently large.
    % Therefore, we have 
    % \begin{equation}\label{eqn_temp: 2.2}
    %     p \in \Big(\frac{\hat{\lambda}}{1+(1-\w[\varepsilon])\mu^{-1}K^{-1/2}}
    %     ,
    %      \frac{\hat{\lambda}}{1-(1-\w[\varepsilon])\mu^{-1}K^{-1/2}} \Big).
    % \end{equation}
    {To make the bound in \eqref{eqn_temp: 2.2}  meaningful, we need 
    \begin{equation}
        p\ge\frac{1}{2(1-\w[\varepsilon])}.
    \end{equation}}
    
    {When $\ell >1$, following similar steps in \eqref{eqn:p_outer_loop}, we have \begin{equation}\label{eqn:p_outer_loop_2}
        \begin{split}
            &\lim_{T\to \infty}\| \bfW^{(\ell, T)} -\Wp \|_2\\
    \le& \frac{1}{1-\tilde{\varepsilon}} \cdot \Big( {1-p} +\mu\sqrt{K}\big|(\hat{\lambda}-p)\big| \Big)\cdot\|\W[0,0]-\bfW^* \|_2 
    +\frac{\tilde{\varepsilon} p}{1-\tilde{\varepsilon}}\cdot\|\W[\ell,0]-\Wp \|_2,
    \end{split}
    \end{equation}
    Given \eqref{eqn_temp: 2.2} holds, from \eqref{eqn:p_outer_loop_2}, we have
    \begin{equation}
    \begin{split}
        &\lim_{L\to \infty, T\to \infty}\| \bfW^{(L, T)} -\Wp \|_2\\
        \le &  \frac{1}{1-\widetilde{\varepsilon}} \cdot\Big( {1-p} +\mu\sqrt{K}\big|\hat{\lambda}-p\big| \Big)\cdot\|\W[0,0]-\bfW^* \|_2\\
        \le& \frac{1}{1-\widetilde{\varepsilon}} \cdot \Big( {1-p} +\mu\sqrt{K}\big|\hat{\lambda}-p\big| \Big)\cdot\|\W[0,0]-\bfW^* \|_2.
    \end{split}
    \end{equation}}
\end{proof}

\section{Definition and relative proofs of $\rho$}
\label{sec: rho}
In this section, the formal definition of $\rho$ is included in Definition \ref{defi: rho}, and a corresponding claim about $\rho$ is summarized in Lemma \ref{lemma: rho_order}.  One can quickly check that \Revise{the} ReLU activation function satisfies the conditions in Lemma \ref{lemma: rho_order}.


The major idea in proving Lemma \ref{lemma: rho_order} is to show $H_r(\delta)$ and $J_r(\delta)$ in Definition \ref{defi: rho} are in the order of $\delta^r$ when $\delta$ is small. 
\begin{definition}\label{defi: rho}
    Let $H_r(\delta) = \mathbb{E}_{z\sim \mathcal{N}(0,\delta^2)}\big( \phi^{\prime}(\sigma_Kz)z^r \big)$ and  $J_r(\delta) = \mathbb{E}_{z\sim \mathcal{N}(0,\delta^2)}\big( \phi^{\prime 2}(\sigma_Kz)z^r \big)$. Then, $\rho=\rho(\delta)$ is defined as 
    \begin{equation}\label{eqn: rho}
        \rho(\delta)=\min\Big\{ J_0(\delta)-H_0^2( \delta) -H_1^2(\delta), J_2(\delta)-H_1^2( \delta) -H_2^2(\delta), H_0(\delta)\cdot H_2( \delta) -H_1^2(\delta)  \Big\},
    \end{equation}    
    where $\sigma_K$ is the minimal singular value of $\bfW^*$.
\end{definition}
\begin{lemma}[Order analysis of $\rho$]
\label{lemma: rho_order}
    If $\rho(\delta)>0$ for $\delta\in(0, \xi)$ for some positive constant $\xi$ and the sub-gradient of $\rho(\delta)$ at $0$ can be non-zero,  then $\rho(\delta)=\Theta(\delta^2)$ when $\delta\to 0^+$. \Revise{Typically, for ReLU activation function, $\mu$ in \eqref{eqn: definition_lambda} is a fixed constant for all $\delta, \de \leq 1$.}
\end{lemma}

\begin{proof}[ Proof of Lemma \ref{lemma: rho_order} ]
    From Definition \ref{defi: rho}, we know that 
    $H_r(\delta) = \mathbb{E}_{\bfz \sim \mathcal{N}(0,\delta^2)}\phi^{\prime}(\sigma_Kz)z^r$. 
    Suppose we have $H_r(\delta)=\Theta(\delta^r)$ and $J_r(\delta)=\Theta(\delta^r)$, then from \eqref{eqn: rho} we have 
    \begin{equation}
        \begin{split}
            &J_0(\delta)-H_0^2( \delta) -H_1^2(\delta) \in \Theta(1)-\Theta(\delta^2),\\
            &J_2(\delta)-H_1^2( \delta) -H_2^2(\delta) \in \Theta(\delta^2),\\
            &H_0(\delta)\cdot H_2( \delta) -H_1^2(\delta) \in \Theta(\delta^2)-\Theta(\delta^4).
        \end{split}
    \end{equation}
    Because $\rho$ is a continuous function with $\rho(z)>0$ for some $z>0$. Therefore, $\rho\neq J_0(\delta)-H_0^2( \delta) -H_1^2(\delta)$
    when $\delta \to 0^+$, otherwise $\rho(z)<0$ for any $z>0$. When $\delta\to 0^+$, both 
    $J_2(\delta)-H_1^2( \delta) -H_2^2(\delta)$ and $H_0(\delta)\cdot H_2( \delta) -H_1^2(\delta)$ are in the order of $\delta^2$, which indicates that $\mu$ is a fixed constant when both $\delta$ and $\de$ are close to $0$.
    In addition, $J_2(\delta)-H_1^2( \delta) -H_2^2(\delta)$ goes to $+\infty$ while both $J_0(\delta)-H_0^2( \delta) -H_1^2(\delta)$ and $H_0(\delta)\cdot H_2( \delta) -H_1^2(\delta)$ go to $-\infty$  when $\delta\to +\infty$. Therefore, with a large enough $\delta$, we have 
    \begin{equation}
        \Revise{\rho(\delta) \in \Theta(\delta^2)-\Theta(\delta^4) \text{ \quad or \quad } \Theta(1)-\Theta(\delta^2),}
    \end{equation}
    which indicates that \Revise{$\mu$ is a strictly decreasing function} when $\delta$ and $\de$ are large enough.
    
    Next, we provide the conditions that guarantee $H_r(\delta)=\Theta(\delta^r)$ hold, and the relative proof for $J_r(\delta)$ can be derived accordingly following the similar steps as well.
    From Definition \ref{defi: rho}, we have
    \begin{equation}
    \begin{split}
        \lim_{\delta \to 0^+} \frac{H_r(\delta)}{\delta^r} 
        =&\lim_{\delta \to 0^+} \int_{-\infty}^{+\infty} \phi^{\prime}(\sigma_K  z) \big(\frac{z}{\delta}\big)^r\frac{1}{\sqrt{2\pi}\delta}e^{-\frac{z^2}{\delta^2}}dz\\
        \stackrel{(a)}{=}&\lim_{\delta \to 0^+}\int_{-\infty}^{+\infty} \phi^{\prime}(\sigma_K \delta t) \frac{t^r}{\sqrt{2\pi}}e^{-t^2}dt \\
        =&\lim_{\delta \to 0^+} \int_{-\infty}^{0^-} \phi^{\prime}(\sigma_K \delta t) \frac{t^r}{\sqrt{2\pi}}e^{-t^2}dt 
        +\lim_{\delta \to 0^+}\int_{0^+}^{+\infty} \phi^{\prime}(\sigma_K \delta t) \frac{t^r}{\sqrt{2\pi}}e^{-t^2}dt \\
        =& \phi^{\prime}(0^-) \int_{-\infty}^{0^-}  \frac{t^r}{\sqrt{2\pi}}e^{-t^2}dt +\phi^{\prime}(0^+)\int_{0^+}^{+\infty}  \frac{t^r}{\sqrt{2\pi}}e^{-t^2}dt,
    \end{split}
    \end{equation}
    where equality $(a)$ holds by letting $t=\frac{z}{\delta}$.
    It is easy to verify that $$\int_{0^+}^{+\infty}  \frac{t^r}{\sqrt{2\pi}}e^{-t^2}dt=(-1)^r\int_{-\infty}^{0^-}  \frac{t^r}{\sqrt{2\pi}}e^{-t^2}dt,$$ and both are bounded for a fixed $r$.  Thus, as long as either $\phi^{\prime}(0^-)$ or $\phi^{\prime}(0^+)$ is non-zero, we have $H_r(\delta)=\Theta(\delta^r)$ when $\delta\to 0^+$.
    
    If $\phi$ has bounded gradient as $|\phi^{\prime}|\le C_{\phi}$ for some positive constant $C_{\phi}$. Then, we have 
        \begin{equation}
    \begin{split}
         \big|\frac{H_r(\delta)}{\delta^r}\big| 
        =&\Big|\int_{-\infty}^{+\infty} \phi^{\prime}(\sigma_K  z) \big(\frac{z}{\delta}\big)^r\frac{1}{\sqrt{2\pi}\delta}e^{-\frac{z^2}{\delta^2}}dz\Big|\\
        =&\Big|\int_{-\infty}^{+\infty} \phi^{\prime}(\sigma_K \delta t) \frac{t^r}{\sqrt{2\pi}}e^{-t^2}dt\Big| \\
        \le & C_{\phi}\cdot\Big|\int_{-\infty}^{+\infty}  \frac{t^r}{\sqrt{2\pi}}e^{-t^2}dt\Big|
    \end{split}
    \end{equation}
    Therefore, we have $H_r(\delta) = \mathcal{O}(\delta^r)$ for all $\delta>0$ when $\phi$ has bounded gradient.
    
    \Revise{Typiclly, for ReLU function, one can directly calculate that $H_r(\delta) = \delta^r$ for $\delta\in \mathbb{R}$, and $\rho(\delta) = C\delta^2$ when $\delta\le 1$ for some constant $C=0.091$. Then, it is easy to check that $\mu$ is a constant when $\delta, \tilde{\delta}\le1$.}
\end{proof}

\section{Proof of preliminary lemmas}
\label{sec: proof of preliminary lemmas}
\subsection{Proof of Lemma \ref{Lemma: p_second_order_derivative bound}} \label{sec: Proof: second_order_derivative}
The eigenvalues of $\nabla^2 f(\cdot;p)$ at any fixed point $\bfW$ can be bounded in the form of \eqref{eqn: thm1_main} by Weyl's inequality (Lemma \ref{Lemma: weyl}). Therefore, the primary technical challenge lies in bounding $\| \nabla^2 f (\bfW;p) - \nabla^2 f (\Wp;p) \|_2$, which is summarized in Lemma \ref{Lemma: p_Second_order_distance}. \Revise{Lemma \ref{Lemma: Zhong} provides the exact calulation of the lower bound of  $\mathbb{E}_{\bfx}\Big(\sum_{j=1}^K \bfal_j^T\bfx \phi^{\prime}(\bfw_j^{[p]T}\bfx) \Big)^2$ when $\bfx$ belongs to Gaussian distribution with zero mean, which is used in proving the lower bound of the Hessian matrix in \eqref{eqn: lower}.}
\begin{lemma}\label{Lemma: p_Second_order_distance}
   Let $f(\bfW;p)$ be the population risk function defined in \eqref{eqn: p_population_risk_function} with $p$ and $\bfW$ satisfying \eqref{eqn: p_initial}. Then, we have 
   \begin{equation}
       \| \nabla^2 f(\Wp;p)- \nabla^2 f(\bfW;p) \|_2 \lesssim \frac{\lambda\delta^2+(1-\lambda)\de^2}{K}\cdot\frac{\|\Wp-\bfW\|_2}{\sigma_K}.
   \end{equation}

\end{lemma}
\Revise{
\begin{lemma}[Lemma D.6, \citep{ZSJB17}]\label{Lemma: Zhong}
For any $\{\bfw_j\}_{j=1}^K\in \mathbb{R}^d$, let $\bfal \in \mathbb{R}^{dK}$ be the unit vector defined in \eqref{eqn: alpha_definition}. When the $\phi$ is ReLU function, we have
   \begin{equation}
       \min_{\|\bfal\|_2=1}\mathbb{E}_{\bfx\sim \mathcal{N}(0,\sigma^2)}\Big(\sum_{j=1}^K \bfal_j^T\bfx \phi^{\prime}(\bfw_j^{T}\bfx) \Big)^2 \gtrsim \rho(\sigma),
   \end{equation}
    where $\rho(\sigma)$ is defined in Definition \ref{defi: rho}.
\end{lemma}}
\begin{proof}[Proof of Lemma \ref{Lemma: p_second_order_derivative bound}]
    Let $\lambda_{\max}(\bfW)$ and $\lambda_{\min}(\bfW)$ denote the largest and smallest eigenvalues of $\nabla^2 f(\bfW;p)$ at point $\bfW$, respectively. Then, from Lemma \ref{Lemma: weyl}, we have 
    \begin{equation}\label{eqn: thm1_main}
    \begin{gathered}
        \lambda_{\max}(\bfW) \le \lambda_{\max}(\Wp) + \| \nabla^2 f (\bfW;p) - \nabla^2 f (\Wp;p) \|_2,\\
        \lambda_{\min}(\bfW) \ge \lambda_{\min}(\Wp) \Revise{ - } \| \nabla^2 f (\bfW;p) - \nabla^2 f (\Wp;p) \|_2.
    \end{gathered}
    \end{equation}
    Then, we provide the lower bound of the Hessian matrix of the population function at $\Wp$. \Revise{For any $\bfal\in\mathbb{R}^{dK}$ defined in \eqref{eqn: alpha_definition} with $\|\bfal\|_2 =1$,} we have 
    \begin{equation}\label{eqn: lower}
    \begin{split}
        &\min_{\|\boldsymbol{\alpha}\|_2=1} \bfal^T \nabla^2 f(\Wp;p) \bfal\\
        =& \frac{1}{K^2} \min_{\|\bfal\|_2=1 } \Big[\lambda \mathbb{E}_{\bfx}\Big(\sum_{j=1}^K \bfal_j^T\bfx \phi^{\prime}(\bfw_j^{[p]T}\bfx) \Big)^2
        +\widetilde{\lambda} \mathbb{E}_{\widetilde{\bfx}}\Big(\sum_{j=1}^K \bfal_j^T\w[\bfx] \phi^{\prime}(\bfw_j^{[p]T}\w[\bfx]) \Big)^2
        \Big] \\
        \ge &\frac{1}{K^2} \min_{\|\bfal\|_2=1 } \lambda \mathbb{E}_{\bfx}\Big(\sum_{j=1}^K \bfal_j^T\bfx \phi^{\prime}(\bfw_j^{[p]T}\bfx) \Big)^2
        +\min_{\|\bfal\|_2=1 }\widetilde{\lambda} \mathbb{E}_{\widetilde{\bfx}}\Big(\sum_{j=1}^K \bfal_j^T\w[\bfx] \phi^{\prime}(\bfw_j^{[p]T}\w[\bfx]) \Big)^2\\
        \ge & \frac{\lambda\rho(\delta) + \w[\lambda]\rho(\de)}{11\kappa^2\gamma K^2},
        \end{split}
    \end{equation}
    where the last inequality comes from Lemma \ref{Lemma: Zhong}. 
    
    Next, the upper bound can be bounded as 
    \begin{equation}
        \begin{split}
            &\max_{\|\boldsymbol{\alpha}\|_2=1} \bfal^T \nabla^2 f(\Wp;p) \bfal\\
        =& \frac{1}{K^2} \max_{\|\bfal\|_2=1 } \Big[\lambda \mathbb{E}_{\bfx}\Big(\sum_{j=1}^K \bfal_j^T\bfx \phi^{\prime}(\bfw_j^{[p]T}\bfx) \Big)^2
        +\widetilde{\lambda} \mathbb{E}_{\widetilde{\bfx}}\Big(\sum_{j=1}^K \bfal_j^T\w[\bfx] \phi^{\prime}(\bfw_j^{[p]T}\w[\bfx]) \Big)^2
        \Big] \\
        \le &\frac{1}{K^2} \max_{\|\bfal\|_2=1 } \lambda \mathbb{E}_{\bfx}\Big(\sum_{j=1}^K \bfal_j^T\bfx \phi^{\prime}(\bfw_j^{[p]T}\bfx) \Big)^2
        +\max_{\|\bfal\|_2=1 }\widetilde{\lambda} \mathbb{E}_{\widetilde{\bfx}}\Big(\sum_{j=1}^K \bfal_j^T\w[\bfx] \phi^{\prime}(\bfw_j^{[p]T}\w[\bfx]) \Big)^2.\\
        %  \le &\frac{1}{K^2} \max_{\|\bfal\|_2=1 } \lambda\sum_{j=1}^K \mathbb{E}_{\bfx}\Big( \bfal_j^T\bfx \phi^{\prime}(\bfw_j^{[p]T}\bfx) \Big)^2
        %  +\max_{\|\bfal\|_2=1 }\widetilde{\lambda}\sum_{j=1}^K \mathbb{E}_{\widetilde{\bfx}}\Big( \bfal_j^T\w[\bfx] \phi^{\prime}(\bfw_j^{[p]T}\w[\bfx]) \Big)^2\\
        %  \le& \frac{6(\lambda\delta^2+\w[\lambda]\de^2)}{K}.
        \end{split}
    \end{equation}
    \Revise{For $\mathbb{E}_{\bfx}\Big(\sum_{j=1}^K \bfal_j^T\bfx \phi^{\prime}(\bfw_j^{[p]T}\bfx) \Big)^2$, we have 
    \begin{equation}
        \begin{split}
            &\mathbb{E}_{\bfx}\Big(\sum_{j=1}^K \bfal_j^T\bfx \phi^{\prime}(\bfw_j^{[p]T}\bfx) \Big)^2\\
            =& \mathbb{E}_{\bfx}\sum_{j_1=1}^K \sum_{j_2=1}^K \bfal_{j_1}^T\bfx \phi^{\prime}(\bfw_{j_1}^{[p]T}\bfx) \bfal_{j_2}^T\bfx \phi^{\prime}(\bfw_{j_2}^{[p]T}\bfx)\\
            =&\sum_{j_1=1}^K \sum_{j_2=1}^K \mathbb{E}_{\bfx} \bfal_{j_1}^T\bfx \phi^{\prime}(\bfw_{j_1}^{[p]T}\bfx) \bfal_{j_2}^T\bfx \phi^{\prime}(\bfw_{j_2}^{[p]T}\bfx)\\
            \le & \sum_{j_1=1}^K \sum_{j_2=1}^K 
            \Big[\mathbb{E}_{\bfx} (\bfal_{j_1}^T\bfx)^4 \mathbb{E}_{\bfx} (\phi^{\prime}(\bfw_{j_1}^{[p]T}\bfx))^4
            \mathbb{E}_{\bfx} (\bfal_{j_2}^T\bfx)^4 \mathbb{E}_{\bfx} (\phi^{\prime}(\bfw_{j_2}^{[p]T}\bfx))^4\Big]^{1/4}\\
            \le& \sum_{j_1=1}^K \sum_{j_2=1}^K 3\delta^2 \|\bfal_{j_1}\|_2 \|\bfal_{j_2}\|_2\\
            \le& 6\delta^2 \sum_{j_1=1}^K \sum_{j_2=1}^K \frac{1}{2}(\|\bfal_{j_1}\|_2^2+ \|\bfal_{j_2}\|_2^2)\\
            =&6K\delta^2
        \end{split}
    \end{equation}
    Therefore, we have 
        \begin{equation}
        \begin{split}
            &\max_{\|\boldsymbol{\alpha}\|_2=1} \bfal^T \nabla^2 f(\Wp;p) \bfal\\
        % =& \frac{1}{K^2} \max_{\|\bfal\|_2=1 } \Big[\lambda \mathbb{E}_{\bfx}\Big(\sum_{j=1}^K \bfal_j^T\bfx \phi^{\prime}(\bfw_j^{[p]T}\bfx) \Big)^2
        % +\widetilde{\lambda} \mathbb{E}_{\widetilde{\bfx}}\Big(\sum_{j=1}^K \bfal_j^T\w[\bfx] \phi^{\prime}(\bfw_j^{[p]T}\w[\bfx]) \Big)^2
        % \Big] \\
         \le &\frac{1}{K^2} \max_{\|\bfal\|_2=1 } \lambda \mathbb{E}_{\bfx}\Big(\sum_{j=1}^K \bfal_j^T\bfx \phi^{\prime}(\bfw_j^{[p]T}\bfx) \Big)^2
         +\max_{\|\bfal\|_2=1 }\widetilde{\lambda} \mathbb{E}_{\widetilde{\bfx}}\Big(\sum_{j=1}^K \bfal_j^T\w[\bfx] \phi^{\prime}(\bfw_j^{[p]T}\w[\bfx]) \Big)^2\\
        % %  \le &\frac{1}{K^2} \max_{\|\bfal\|_2=1 } \lambda\sum_{j=1}^K \mathbb{E}_{\bfx}\Big( \bfal_j^T\bfx \phi^{\prime}(\bfw_j^{[p]T}\bfx) \Big)^2
        %  +\max_{\|\bfal\|_2=1 }\widetilde{\lambda}\sum_{j=1}^K \mathbb{E}_{\widetilde{\bfx}}\Big( \bfal_j^T\w[\bfx] \phi^{\prime}(\bfw_j^{[p]T}\w[\bfx]) \Big)^2\\
        \le& \frac{6(\lambda\delta^2+\w[\lambda]\de^2)}{K}.
        \end{split}
    \end{equation}
    }Then, given \eqref{eqn: p_initial}, we have 
    \begin{equation}\label{eqn: thm11_temp}
        \|\W[0,0] - \Wp \|_F = p\|\W[0,0]-\bfW^* \|_F \lesssim \frac{\sigma_K}{\mu^2K}.
    \end{equation}
    Combining \eqref{eqn: thm11_temp} and Lemma \ref{Lemma: p_Second_order_distance}, we have 
    \begin{equation}\label{eqn: thm11_temp2}
        \| \nabla^2 f (\bfW;p) - \nabla^2 f (\Wp;p) \|_2\lesssim \frac{\lambda\rho(\delta) + \w[\lambda]\rho(\de)}{\Revise{132\kappa^2\gamma K^2}}.
    \end{equation}
    Therefore, \eqref{eqn: thm11_temp2} and \eqref{eqn: thm1_main} completes the whole proof.
\end{proof}

\subsection{Proof of Lemma \ref{Lemma: p_first_order_derivative}}
\label{sec: first_order_derivative}
\Revise{The task of bounding of the quantity} between $\|\nabla \hat{f} -\nabla f \|_2$ is dividing into bounding $I_1$, $I_2$, $I_3$ and $I_4$ as shown in \eqref{eqn: Lemma2_temp}. $I_1$ and $I_3$ represent the deviation of  the mean of several random variables to their expectation, which can be bounded through concentration inequality, i.e, Chernoff bound. $I_2$ and $I_4$ come from the inconsistency of the output label $y$ and pseudo label $\widetilde{y}$ in the empirical risk function in \eqref{eqn: empirical_risk_function} and population risk function in \eqref{eqn: p_population_risk_function}. The major challenge lies in characterizing the upper bound of $\bfI_2$ and $\bfI_4$ as the linear function of $\w[\bfW]-\Wp$ and $\Wp-\bfW^*$, which is summarized in \eqref{eqn:first_order_term3}.
\begin{proof}[Proof of Lemma \ref{Lemma: p_first_order_derivative}]
    From \eqref{eqn: empirical_risk_function}, we know that 
    \begin{equation}
        \begin{split}
        \frac{\partial \hat{f}}{\partial \bfw_k}(\bfW) 
        =& \frac{\lambda}{N}\sum_{n=1}^N \Big( \frac{1}{K}\sum_{j=1}^K\phi(\bfw_j^T\bfx_n) - y_n \Big)\bfx_n
         +\frac{1-\lambda}{M}\sum_{m=1}^M \Big( \frac{1}{K}\sum_{j=1}^K\phi(\bfw_j^T\w[\bfx]_m) - \w[y]_n \Big)\w[\bfx]_m\\
        =& \frac{\lambda}{K^2N}\sum_{n=1}^N \sum_{j=1}^K\Big( \phi(\bfw_j^T\bfx_n)-\phi(\bfw_j^{*T}\bfx_n) \Big)\bfx_n \\
         & + \frac{1-\lambda}{K^2M}\sum_{m=1}^M \sum_{j=1}^K\Big( \phi(\bfw_j^T\w[\bfx]_m)-\phi(\w[\bfw]_j^T\w[\bfx]_m) \Big)\w[\bfx]_m.
        \end{split}
    \end{equation}
    From \eqref{eqn: population_risk_function}, we know that
    \begin{equation}
        \begin{split}
        \frac{\partial \hat{f}}{\partial \bfw_k}(\bfW) 
        = \frac{\lambda}{K^2}\mathbb{E}_{\bfx} \sum_{j=1}^K\Big( \phi(\bfw_j^T\bfx)-\phi(\bfw_j^{*T}\bfx) \Big)\bfx
         + \frac{1-\lambda}{K^2}\mathbb{E}_{\w[\bfx]} \sum_{j=1}^K\Big( \phi(\bfw_j^T\w[\bfx])-\phi(\w[\bfw]_j^T\w[\bfx]) \Big)\w[\bfx].
        \end{split}
    \end{equation}
    Then, from \eqref{eqn: p_population_risk_function}, we have 
    \begin{equation}\label{eqn: Lemma2_temp}
        \begin{split}
            &\frac{\partial \hat{f} }{ \partial \bfw_k } (\bfW) - \frac{\partial {f} }{ \partial \bfw_k} (\bfW;p)\\
            = & \frac{\lambda}{K^2N} \sum_{j=1}^K \Big[ \sum_{n=1}^N\big( \phi(\bfw_j^T\bfx_n) - \phi(\bfw_j^{*T}\bfx_n)\big)\bfx_n - \mathbb{E}_{\bfx}\big( \phi(\bfw_j^T\bfx) -\phi(\bfw^{[p]T}_j\bfx) \big)\bfx 
            \Big]\\
             &+ \frac{1-\lambda}{K^2M} \sum_{j=1}^K \Big[ \sum_{m=1}^M\big( \phi(\bfw_j^T\w[\bfx]_m) - \phi(\w[\bfw]_j^T\w[\bfx]_m)\big)\w[\bfx]_m - \mathbb{E}_{\w[\bfx]}\big( \phi(\bfw_j^T\w[\bfx]) -\phi(\bfw^{[p]T}_j\w[\bfx]) \big)\w[\bfx] 
            \Big]\\
            = & \frac{\lambda}{K^2} \sum_{j=1}^K \Big[ \frac{1}{N}\sum_{n=1}^N\big( \phi(\bfw_j^T\bfx_n) - \phi(\bfw_j^{*T}\bfx_n)\big)\bfx_n - \mathbb{E}_{\bfx}\big( \phi(\bfw_j^T\bfx) -\phi(\bfw^{*T}_j\bfx) \big)\bfx 
            \Big]\\
            & +\frac{\lambda}{K^2}\sum_{j=1}^K \mathbb{E}_{\bfx}\Big[ \big( \phi(\bfw_j^{*T}\bfx) - \phi(\bfw^{[p]T}_j\bfx) \big)\bfx  \Big]\\
             & + \frac{1-\lambda}{K^2} \sum_{j=1}^K \Big[ \frac{1}{M}\sum_{m=1}^M\big( \phi(\bfw_j^T\w[\bfx]_m) - \phi(\w[\bfw]_j^T\w[\bfx]_m)\big)\w[\bfx]_m - \mathbb{E}_{\w[\bfx]}\big( \phi(\bfw_j^T\w[\bfx]) -\phi(\w[\bfw]^T_j\w[\bfx]) \big)\w[\bfx] 
            \Big]\\
            & + \frac{1-\lambda}{K^2}\sum_{j=1}^K \mathbb{E}_{\w[\bfx]}\Big[ \big( \phi(\w[\bfw]_j^T\w[\bfx]) - \phi(\bfw^{[p]T}_j(p)\w[\bfx]) \big)\w[\bfx]  \Big]\\
            :=& \bfI_1 + \bfI_2 + \bfI_3 +\bfI_4.
        \end{split}
    \end{equation}
    For any $\boldsymbol{\alpha}_j \in \mathbb{R}^{d}$ with $\| \boldsymbol{\alpha}_j \|_2 \le 1$, we define a random variable $Z(j) = \big( \phi(\bfw_j^T\bfx) - \phi(\bfw_j^{*T}\bfx)\big)\boldsymbol{\alpha}^T_j\bfx$ and $Z_n(j) = \big( \phi(\bfw_j^T\bfx_n) - \phi(\bfw_j^{*T}\bfx_n)\big)\boldsymbol{\alpha}^T_j\bfx_n$ as the realization of $Z(j)$ for $n=1,2\cdots, N$. Then, for any $p\in \mathbb{N}^+$, we have 
    \begin{equation}\label{eqn: temppp}
        \begin{split}
        \big(\mathbb{E}|Z|^p\big)^{1/p}
        =& \Big( \mathbb{E} |\phi(\bfw_j^T\bfx)-\phi(\bfw_j^{*T}\bfx)|^p \cdot |\boldsymbol{\alpha}_j^T\bfx|^p \Big)^{1/p}\\
        \le& \Big( \mathbb{E} |(\bfw_j-\bfw_j^*)^T\bfx|^p \cdot |\boldsymbol{\alpha}_j^T\bfx|^p \Big)^{1/p}\\
        \le& C \cdot \delta^2 \| \bfw_j - \bfw_j^* \|_2 \cdot p, 
        \end{split}
    \end{equation}
    where $C$ is a positive constant and the last inequality holds since $\bfx\sim \mathcal{N}(0, \delta^2)$. From Definition \ref{Def: sub-exponential}, we know that $Z$ belongs to sub-exponential distribution with $\|Z\|_{\psi_1}\lesssim \delta^2 \| \bfw_j - \bfw_j^* \|_2$.
    Therefore, by Chernoff inequality, we have 
    \begin{equation}
        \mathbb{P}\bigg\{ \Big| \frac{1}{N}\sum_{n=1}^N Z_n(j) -\mathbb{E}Z(j) \Big| < t \bigg\} \le 1- \frac{e^{-C(\delta^2\| \bfw_j - \bfw_j^* \|_2)^2\cdot Ns^2}}{e^{Nst}}
    \end{equation}
    for some positive constant $C$ and any $s\in\mathbb{R}$. 
    
    Let $t=\delta^2\|\bfw_j-\bfw_j^*\|_2\sqrt{\frac{d\log q}{N}}$ and $s = \frac{2}{C\delta^2\|\bfw_j-\bfw_j^*\|_2}\cdot t$ for some large constant $q>0$, we have
    \begin{equation}
        \begin{split}
                \Big| \frac{1}{N}\sum_{n=1}^N Z_n(j) -\mathbb{E}Z(j) \Big| \lesssim \delta^2\|\bfw_j-\bfw_j^*\|_2 \cdot \sqrt{\frac{d\log q}{N}}
        \end{split}
    \end{equation}
    with probability at least $1-q^{-d}$.
    From Lemma \ref{Lemma: spectral_norm_on_net}, we have 
    \begin{equation}\label{eqn:first_order_term1}
    \begin{split}
       &\Big\| \frac{1}{N}\sum_{n=1}^N\big( \phi(\bfw_j^T\bfx_n) - \phi(\bfw_j^{*T}\bfx_n)\big)\bfx_n - \mathbb{E}_{\bfx}\big( \phi(\bfw_j^T\bfx) -\phi(\bfw^{*T}_j\bfx) \big)\bfx\Big\|_2\\
       \le& 2 \delta^2\|\bfw_j-\bfw_j^*\|_2 
       \cdot \sqrt{\frac{d\log q}{N}}
    \end{split}
    \end{equation}
    with probability at least $1-(q/5)^{-d}$. Since $q$ is a large constant, we release the probability as $1-q^{-d}$ for simplification. 
    Similar to $Z$, we have  
    \begin{equation}\label{eqn:first_order_term2}
        \begin{split}
        &\Big\|\frac{1}{M}\sum_{m=1}^M\big( \phi(\bfw_j^T\w[\bfx]_m) - \phi(\w[\bfw]_j^T\w[\bfx]_m)\big)\w[\bfx]_m - \mathbb{E}_{\w[\bfx]}\big( \phi(\bfw_j^T\w[\bfx]) -\phi(\w[\bfw]^T_j\w[\bfx]) \big)\w[\bfx]\Big\|_2\\
        \lesssim& \de^2\|\bfw_j-\w[\bfw]_j\|_2 \cdot \sqrt{\frac{d\log q}{M}}
        \end{split}
    \end{equation}
    with probability at least $1-q^{-d}$.
    
    \begin{figure}[h]
  	\centering
  	\includegraphics[width=0.4\linewidth]{Figure/circle_1.pdf}
  	\caption{The subspace spanned by $\bfw_j^*$ and $\bfw_j^{[p]}$}
  	\label{fig:circle}
    \end{figure}
    
    For term $\mathbb{E}_{\bfx}\Big[ \big( \phi(\bfw_j^{*T}\bfx) - \phi(\bfw^{[p]T}_j\bfx) \big)\bfx  \Big]$, let us define the angle between $\bfw_j^*$ and $\bfw^{[p]}_j$ as $\theta_1$. Figure \ref{fig:circle} shows the subspace spanned by the vector $\bfw_j^*$ and $\w[\bfw]_j$. We divide the subspace by 4 pieces, where the gray region denotes area I, and the blue area denotes area II. Areas III and IV are the symmetries of II and I from the origin, respectively. Hence, we have 
    \begin{equation}
        \begin{split}
            &\mathbb{E}_{\bfx}\Big[ \big( \phi(\bfw_j^{*T}\bfx) - \phi(\bfw^{[p]T}_j\bfx) \big)\bfx  \Big]\\
            =&\mathbb{E}_{\bfx\in \text{ area I} }\Big[ \big( \phi(\bfw_j^{*T}\bfx) - \phi(\bfw^{[p]T}_j\bfx) \big)\bfx  \Big]
            +\mathbb{E}_{\bfx\in \text{ area II} }\Big[ \big( \phi(\bfw_j^{*T}\bfx) - \phi(\bfw^{[p]T}_j\bfx) \big)\bfx  \Big]\\
            &+\mathbb{E}_{\bfx\in \text{ area III} }\Big[ \big( \phi(\bfw_j^{*T}\bfx) - \phi(\bfw^{[p]T}_j\bfx) \big)\bfx  \Big]
            +\mathbb{E}_{\bfx\in \text{ area IV} }\Big[ \big( \phi(\bfw_j^{*T}\bfx) - \phi(\bfw^{[p]T}_j\bfx) \big)\bfx  \Big]\\
            =&\mathbb{E}_{\bfx\in \text{ area I} }\Big[ \big( \phi(\bfw_j^{*T}\bfx) - \phi(\bfw^{[p]T}_j\bfx) \big)\bfx  \Big]
            + \mathbb{E}_{\bfx\in \text{ area II} }\big[ \bfw^{*T}_j\w[\bfx]\w[\bfx] \big] 
            - \mathbb{E}_{\bfx\in \text{ area III} }\big[ \bfw^{[p]T}_j\bfx\bfx \big]\\
            =&\mathbb{E}_{\bfx\in \text{ area I} }\big[ (\bfw^{*}_j-\bfw^{[p]}_j)^T\bfx \bfx \big]
            + \mathbb{E}_{\bfx\in \text{ area II} }\big[ (\bfw^{*}_j-\bfw^{[p]}_j)^T\bfx \bfx \big] \\
            =&\frac{1}{2}\mathbb{E}_{\bfx}\big[ (\bfw^{*}_j-\bfw^{[p]}_j)^T\bfx \bfx \big]
        \end{split}
    \end{equation}
    Therefore, we have
    \begin{equation}\label{eqn:first_order_term3}
    \begin{split}
        &\bigg\|\frac{\lambda}{K^2}\mathbb{E}_{\bfx}\Big[ \big( \phi(\bfw_j^{*T}\bfx) - \phi(\bfw^{[p]T}_j\bfx) \big)\bfx  \Big] +  \frac{1-\lambda}{K^2}\mathbb{E}_{\w[\bfx]}\Big[ \big( \phi(\w[\bfw]_j^T\w[\bfx]) - \phi(\bfw^{[p]T}_j\w[\bfx]) \big)\w[\bfx]  \Big]\bigg\|_2\\
        =&\bigg\|\frac{\lambda}{2K^2}\mathbb{E}_{\bfx}\big[ (\bfw^{*}_j-\bfw^{[p]}_j)^T\bfx \bfx \big] + 
        \frac{1-\lambda}{2K^2}
        \mathbb{E}_{\w[\bfx]}\big[ (\w[\bfw]_j-\bfw^{[p]}_j)^T\bfx \bfx \big]\bigg\|_2\\
        =& \frac{\big\| \lambda\delta^2 \cdot \big(\w[\bfw]_j-\bfw^{[p]}_{j}\big) +(1-\lambda)\de^2 \cdot \big(\bfw_j^*-\bfw^{[p]}_{j}\big)  \big\|_2}{2K^2}.
    \end{split}
    \end{equation}
    % Therefore, we have 
    % \begin{equation}\label{eqn:first_order_term3}
    %     \begin{split}
    %         &\left|\boldsymbol{\alpha}_j^T\mathbb{E}_{\w[\bfx]}\Big[ \big( \phi(\w[\bfw]_j^T\w[\bfx]) - \phi(\bfw^{*T}_j\w[\bfx]) \big)\w[\bfx]  \Big]\right|\\
    %         \le & \left| \mathbb{E}_{\w[\bfx]\in \text{ area I} }\big[ (\w[\bfw]_j - \bfw^{*}_j)^T\w[\bfx] (\boldsymbol{\alpha}_j^T\w[\bfx]) \big]
    %         + \mathbb{E}_{\w[\bfx]\in \text{ area II} }\big[ (\bfw^{*}_j-\w[\bfw]_j)^T\w[\bfx]\boldsymbol({\alpha}_j^T\w[\bfx]) \big] \right|\\
    %         \le & \left| \mathbb{E}_{\w[\bfx]\in \text{ area I} }\big[ (\w[\bfw]_j - \bfw^{*}_j)^T\w[\bfx] (\boldsymbol{\alpha}_j^T\w[\bfx]) \big] \right|
    %         + \left| \mathbb{E}_{\w[\bfx]\in \text{ area II} }\big[ (\bfw^{*}_j-\w[\bfw]_j)^T\w[\bfx]\boldsymbol({\alpha}_j^T\w[\bfx]) \big] \right|\\
    %         = & \frac{\pi - \theta}{2\pi}\de^2\|\w[\bfw]_j - \bfw_j^*\|_2 \|\boldsymbol{\alpha}_j\|_2 + \frac{\theta}{2\pi}\de^2\|\w[\bfw]_j - \bfw_j^*\|_2\|\boldsymbol{\alpha}_j\|_2\\
    %         = & \frac{\de^2}{2}\|\w[\bfw]_j - \bfw_j^*\|_2 \|\boldsymbol{\alpha}_j\|_2.
    %     \end{split}
    % \end{equation}
    From \eqref{eqn:first_order_term1}, \eqref{eqn:first_order_term2} and \eqref{eqn:first_order_term3}, we have
        \begin{equation}
        \begin{split}
            &\Big\|\frac{\partial \hat{f} }{ \partial \bfw_k } (\bfW;p) - \frac{\partial {f} }{ \partial \bfw_k } (\bfW)\Big\|_2\\
            \le & \frac{\lambda}{K^2} \sum_{j=1}^K \Big\| \frac{1}{N}\sum_{n=1}^N\big( \phi(\bfw_j^T\bfx_n) - \phi(\bfw_j^{*T}\bfx_n)\big)\bfx_n - \mathbb{E}_{\bfx}\big( \phi(\bfw_j^T\bfx) -\phi(\bfw^{*T}_j\bfx) \big)\bfx 
            \Big\|_2\\
             & + \frac{1-\lambda}{K^2} \sum_{j=1}^K \Big\| \frac{1}{M}\sum_{m=1}^M\big( \phi(\bfw_j^T\w[\bfx]_m) - \phi(\w[\bfw]_j^T\w[\bfx]_m)\big)\w[\bfx]_m - \mathbb{E}_{\w[\bfx]}\big( \phi(\bfw_j^T\w[\bfx]) -\phi(\w[\bfw]^T_j\w[\bfx]) \big)\w[\bfx] 
            \Big\|_2\\
            & + \sum_{j=1}^K\bigg\|\frac{\lambda}{K^2}\mathbb{E}_{\bfx}\Big[ \big( \phi(\bfw_j^{*T}\bfx) - \phi(\bfw^{[p]T}_j\bfx) \big)\bfx  \Big] +  \frac{1-\lambda}{K^2}\mathbb{E}_{\w[\bfx]}\Big[ \big( \phi(\w[\bfw]_j^T\w[\bfx]) - \phi(\bfw^{[p]T}_j\w[\bfx]) \big)\w[\bfx]  \Big]\bigg\|_2\\
            \le &  \frac{\lambda}{K^{2}}\delta^2 \sqrt{\frac{d\log q}{N}}\cdot \sum_{j=1}^K\| \bfw_j -\bfw_j^* \|_2  + \frac{1- \lambda}{K^{2}}\cdot\de^2 \sqrt{\frac{d\log q}{M}} \cdot\sum_{j=1}^K\| \bfw_j - \w[\bfw]_j \|_2\\
            &+\frac{1}{2K^{2}} \cdot\sum_{j=1}^K\big\| \lambda\delta^2 \cdot \big(\w[\bfw]_j-\bfw^{[p]}_{j}\big) +\w[\lambda]\de^2 \cdot \big(\bfw_j^*-\bfw^{[p]}_{j}\big)  \big\|_2\\
            \le &\frac{\lambda}{K^{3/2}}\delta^2 \sqrt{\frac{d\log q}{N}}\cdot \| \bfW -\bfW^* \|_2  + \frac{1- \lambda}{K^{3/2}}\cdot\de^2 \sqrt{\frac{d\log q}{M}} \cdot\| \bfW - \w[\bfW] \|_2\\
            &+\frac{1}{2K^{3/2}} \big\| \lambda\delta^2 \cdot \big(\w[\bfW]-\Wp\big) +(1-\lambda)\de^2 \cdot \big(\bfW^*-\Wp\big)  \big\|_2
            % \le &  \frac{\lambda}{K^{3/2}}\delta^2 \sqrt{\frac{d\log q}{N}}\cdot \| \bfW -\bfW^* \|_2  + \frac{1- \lambda}{K^{3/2}}\cdot\de^2 \sqrt{\frac{d\log q}{M}} \cdot\| \bfW -\w[\bfW] \|_2\\ 
            % &+\frac{(1- \lambda)\de^2}{2K^{3/2}} \cdot\| \w[\bfW] -\bfW^* \|_2\\
            % \le & \Big(\frac{\lambda}{K^{3/2}}\delta^2 \sqrt{\frac{d\log q}{N}} + \frac{1- \lambda}{K^{3/2}}\cdot\de^2 \sqrt{\frac{d\log q}{M}}\Big)\cdot \| \bfW -\bfW^* \|_2\\  &+ \frac{(1- \lambda)\de^2}{K^{3/2}}\cdot\Big( \sqrt{\frac{d\log q}{M}} +\frac{1}{2}\Big) \cdot\| \w[\bfW] -\bfW^* \|_2\\
        \end{split}
    \end{equation}
    with probability at least $1-q^{-d}$.
    
    In conclusion, let $\boldsymbol{\alpha}\in \mathbb{R}^{Kd}$ and  $\boldsymbol{\alpha}_{j}\in \mathbb{R}^d$ with $\boldsymbol{\alpha} =[\boldsymbol{\alpha}_{1}^T, \boldsymbol{\alpha}_{2}^T, \cdots, \boldsymbol{\alpha}_{K}^T]^T$, we have 
    \begin{equation}
        \begin{split}
            \|\nabla f(\bfW) -\nabla \hat{f}(\bfW) \|_2
            = & \Big| \boldsymbol{\alpha}^T \big( \nabla f(\bfW) -\nabla \hat{f}(\bfW) \big)  \Big|\\
            \le & \sum_{k=1}^K\Big| \boldsymbol{\alpha}_k^T \big(\frac{\partial \hat{f} }{ \partial \bfw_k } (\bfW) - \frac{\partial {f} }{ \partial \bfw_k } (\bfW)\big) \Big|\\
            \lesssim & \sum_{k=1}^K\Big\|\frac{\partial \hat{f} }{ \partial \bfw_k } (\bfW) - \frac{\partial {f} }{ \partial \bfw_k } (\bfW)\Big\|_2\cdot \|\boldsymbol{\alpha}_k\|_2\\
            \lesssim &\frac{\lambda}{K}\delta^2 \sqrt{\frac{d\log q}{N}}\cdot \| \bfW -\bfW^* \|_2  + \frac{1- \lambda}{K}\cdot\de^2 \sqrt{\frac{d\log q}{M}} \cdot\| \bfW - \w[\bfW] \|_2\\
            &+\frac{1}{\Revise{2}K} \big\| \lambda\delta^2 \cdot \big(\w[\bfW]-\Wp\big) +(1-\lambda)\de^2 \cdot \big(\bfW^*-\Wp\big)  \big\|_2
        \end{split}
    \end{equation}
    with probability at least $1-q^{-d}$.
\end{proof}

\subsection{Proof of Lemma \ref{Lemma: p_Second_order_distance}}
The distance of the second order derivatives of the population risk function $f(\cdot; p)$ at point $\bfW$ and $\Wp$ can be converted into bounding  $\bfP_1$, $\bfP_2$, $\bfP_3$ and $\bfP_4$, which are defined in \eqref{eqn: Lemma11_main}. The major idea in proving $\bfP_1$ is to connect the error bound to the angle between $\bfW$ and $\Wp$. Similar ideas apply in bounding the other three items as well. 
\begin{proof}[Proof of Lemma \ref{Lemma: p_Second_order_distance}]
	From \eqref{eqn: p_population_risk_function}, we have 
	\begin{equation}
		\begin{split}
		\frac{\partial^2 f}{\partial {\bfw}_{j_1}\partial {\bfw}_{j_2}}(\Wp;p)
		=&\frac{\lambda}{K^2} \mathbb{E}_{\bfx} \phi^{\prime} (\bfw^{[p]T}_{j_1}\bfx) \phi^{\prime} (\bfw^{[p]T}_{j_2}\bfx) \bfx \bfx^T
		+\frac{1-\lambda}{K^2} \mathbb{E}_{\w[\bfx]} \phi^{\prime} (\bfw^{[p]T}_{j_1}\w[\bfx])\phi^{\prime} (\bfw^{[p]T}_{j_2}\w[\bfx]) \w[\bfx] \w[\bfx]^T,
		\end{split}
	\end{equation}
	\begin{equation}
	\begin{split}
	\text{and \quad}  \frac{\partial^2 f}{\partial {\bfw}_{j_1}\partial {\bfw}_{j_2}}(\bfW;p)
	=&\frac{\lambda}{K^2} \mathbb{E}_{\bfx} \phi^{\prime} ({\bfw}_{j_1}^T\bfx)\phi^{\prime} ({\bfw}_{j_2}^T\bfx) \bfx \bfx^T
	+\frac{1-\lambda}{K^2} \mathbb{E}_{\w[\bfx]} \phi^{\prime} ({\bfw}_{j_1}^T\w[\bfx])\phi^{\prime} ({\bfw}_{j_2}^T\w[\bfx]) \w[\bfx] \w[\bfx]^T,
	\end{split}
	\end{equation}
	where \Revise{${\bfw}^{[p]}_j$} is the $j$-th column of $\Wp$.
	Then, we have 
	\begin{equation}\label{eqn: Lemma11_main}
	\begin{split}
	&\frac{\partial^2 f}{\partial {\bfw}_{j_1}\partial {\bfw}_{j_2}}(\bfW^*)
	-
	\frac{\partial^2 f}{\partial {\bfw}_{j_1}\partial {\bfw}_{j_2}}(\bfW)\\
	=&\frac{\lambda}{K^2} \mathbb{E}_{\bfx} \Big[
	\Revise{\phi^{\prime} (\bfw^{[p]T}_{j_1}\bfx)}\phi^{\prime} (\bfw^{[p]T}_{j_2}\bfx)
	-
	\phi^{\prime} ({\bfw}_{j_1}^T\bfx)\phi^{\prime} ({\bfw}_{j_2}^T\bfx)\Big] \bfx \bfx^T\\
	&+\frac{1-\lambda}{K^2} \mathbb{E}_{\w[\bfx]} \Big[
	\phi^{\prime} (\bfw^{[p]T}_{j_1}\w[\bfx])\phi^{\prime} (\bfw^{[p]T}_{j_2}\w[\bfx])
	-
	\phi^{\prime} ({\bfw}_{j_1}^T\w[\bfx])\phi^{\prime} ({\bfw}_{j_2}^T\w[\bfx])\Big] \w[\bfx] \w[\bfx]^T\\
	=&\frac{\lambda}{K^2}\mathbb{E}_{\bfx} 
	\Big[ \phi^{\prime} (\bfw^{[p]T}_{j_1}\bfx)
	\big(\phi^{\prime} (\bfw^{[p]T}_{j_2}\bfx)
	- \phi^{\prime} ({\bfw}_{j_2}^T\bfx)
	\big)
	+
	\phi^{\prime} ({\bfw}_{j_2}^T\bfx)
	\big(\phi^{\prime} (\bfw^{[p]T}_{j_1}\bfx)
	- \phi^{\prime} ({\bfw}_{j_1}^T\bfx)
	\big)
	\Big]\bfx \bfx^T\\
	&+\frac{1-\lambda}{K^2}\mathbb{E}_{\w[\bfx]} 
	\Big[ \phi^{\prime} (\bfw^{[p]T}_{j_1}\w[\bfx])
	\big(\phi^{\prime} (\bfw^{[p]T}_{j_2}\w[\bfx])
	- \phi^{\prime} ({\bfw}_{j_2}^T\w[\bfx])
	\big)
	+
	\phi^{\prime} ({\bfw}_{j_2}^T\w[\bfx])
	\big(\phi^{\prime} (\bfw^{[p]T}_{j_1}\w[\bfx])
	- \phi^{\prime} ({\bfw}_{j_1}^T\w[\bfx])
	\big)
	\Big]\w[\bfx] \w[\bfx]^T\\
	=&\frac{\lambda}{K^2}\Big[
	\mathbb{E}_{\bfx} 
	\phi^{\prime} (\bfw^{[p]T}_{j_1}\bfx)
	\big(\phi^{\prime} (\bfw^{[p]T}_{j_2}\bfx)
	- \phi^{\prime} ({\bfw}_{j_2}^T\bfx)
	\big)\bfx \bfx^T
	+
	\mathbb{E}_{\bfx}
	\phi^{\prime} ({\bfw}_{j_2}^T\bfx)
	\big(\phi^{\prime} (\bfw^{[p]T}_{j_1}\bfx)
	- \phi^{\prime} ({\bfw}_{j_1}^T\bfx)
	\big)\bfx \bfx^T
	\Big]\\
	&+\frac{1-\lambda}{K^2}\Big[
	\mathbb{E}_{\w[\bfx]} 
	\phi^{\prime} (\bfw^{[p]T}_{j_1}\w[\bfx])
	\big(\phi^{\prime} (\bfw^{[p]T}_{j_2}\w[\bfx])
	- \phi^{\prime} ({\bfw}_{j_2}^T\w[\bfx])
	\big)\w[\bfx] \w[\bfx]^T
	+
	\mathbb{E}_{\w[\bfx]}
	\phi^{\prime} ({\bfw}_{j_2}^T\w[\bfx])
	\big(\phi^{\prime} (\bfw^{[p]T}_{j_1}\w[\bfx])
	- \phi^{\prime} ({\bfw}_{j_1}^T\w[\bfx])
	\big)\w[\bfx] \w[\bfx]^T
	\Big]\\
	:=& \frac{\lambda}{K^2} (\bfP_1 + \bfP_2) + \frac{1-\lambda}{K^2}(\bfP_3+\bfP_4).
	\end{split}
	\end{equation}
	For any $\bfa\in\mathbb{R}^{d}$ with \Revise{$\|\bfa\|_2=1$}, we have 
	\begin{equation}
	\begin{split}
	\bfa^T\bfP_1 \bfa 
	=&\mathbb{E}_{\bfx} 
	\phi^{\prime} (\bfw^{[p]T}_{j_1}\bfx)
	\big(\phi^{\prime} (\bfw^{[p]T}_{j_2}\bfx)
	- \phi^{\prime} ({\bfw}_{j_2}^T\bfx)
	\big) 
	(\bfa^T\bfx)^2\\	
% 	\le&\mathbb{E}_{\bfx} 
% 	\phi^{\prime} (\bfw^{*T}_{j_2}\bfx)
% 	\big(\phi^{\prime} (\bfw^{[p]T}_{j_2}\bfx)
% 	- \phi^{\prime} (\bfw_{j_2}^T\bfx)
% 	\big) 
% 	\cdot
% 	(\bfa^T\bfx)^2,	
	\end{split}
	\end{equation}
	 where $\bfa\in\mathbb{R}^d$.
	 Let $I =
    \phi^{\prime} (\bfw^{[p]T}_{j_1}\bfx)
    \big(\phi^{\prime} (\bfw^{[p]T}_{j_2}\bfx)
    - \phi^{\prime} (\bfw_{j_2}^T\bfx)
    \big) 
    \cdot
    (\bfa^T\bfx)^2$. 
    It is easy to verify there exists \Revise{a group of orthonormal vectors} such that $\mathcal{B}=\{\bfa, \bfb, \bfc, \bfa_4^{\perp}, \cdots, \bfa_d^{\perp}\}$ with $\{\bfa, \bfb, \bfc \}$ spans a subspace that contains $\bfa, \bfw_{j_2}$ and $\bfw_{j_2}^*$. Then, for any $\bfx$, we have a unique $\bfz=\begin{bmatrix}
		z_1,&z_2,&\cdots, & z_d
		\end{bmatrix}^T$ such that 
		\begin{equation*}
		\bfx = z_1\bfa + z_2 \bfb +z_3\bfc + \cdots + z_d\bfa^{\perp}_d.
		\end{equation*}
		Also, since $\bfx \sim \mathcal{N}(\boldsymbol{0}, \delta^2\bfI_d)$, we have $\bfz \sim \mathcal{N}(\boldsymbol{0}, \delta^2\bfI_d)$. Then, we have 
		\begin{equation*}
		\begin{split}
		I 
		=& \mathbb{E}_{z_1, z_2, z_3}|\phi^{\prime}\big(\bfw_{j_2}^T{\bfx}\big)-\phi^{\prime}\big({\bfw^{[p]T}_{j_2}}{\bfx}\big)|\cdot 
		|\bfa^T{\bfx}|^2\\
		=&\int|\phi^{\prime}\big(\bfw_{j_2}^T{\bfx}\big)-\phi^{\prime}\big({\bfw^{[p]T}_{j_2}}{\bfx}\big)|\cdot 
		|\bfa^T{\bfx}|^2 \cdot f_Z(z_1, z_2,z_3)dz_1 dz_2 dz_3,
		\end{split}
		\end{equation*}
		where ${\bfx}= z_1\bfa + z_2\bfb + z_3\bfc$ and $f_Z(z_1, z_2,z_3)$ is probability density function of $(z_1, z_2, z_3)$. Next, we consider spherical coordinates with $z_1= Rcos\phi_1 , z_2 = Rsin\phi_1sin\phi_2, \Revise{z_3= Rsin\phi_1cos\phi_2}$. Hence,
		\begin{equation}
		\begin{split}
		I
		=&\int|\phi^{\prime}\big(\bfw_{j_2}^T{\bfx}\big)-\phi^{\prime}\big(\bfw^{[p]T}_{j_2}{\bfx}\big)|\cdot |R\cos\phi_1|^2
		\cdot f_Z(R, \phi_1, \phi_2)R^2\sin \phi_1 dR d\phi_1 d \phi_2.
		\end{split}
		\end{equation}
		It is easy to verify that $\phi^{\prime}\big(\bfw_{j_2}^T{\bfx}\big)$ only depends on the direction of ${\bfx}$ and 
		\Revise{\begin{equation*}
		f_Z(R, \phi_1, \phi_2) = \frac{1}{(2\pi\delta^2)^{\frac{3}{2}}}e^{-\frac{z_1^2+z_2^2+z_3^2}{2\delta^2}}=\frac{1}{(2\pi\delta^2)^{\frac{3}{2}}}e^{-\frac{R^2}{2\delta^2}}
		\end{equation*}}
		only depends on $R$. Then, we have 
		\begin{equation}\label{eqn: ean111}
		\begin{split}
		&I(i_2, j_2)\\
		=&\int|\phi^{\prime}\big(\bfw_{j_2}^T({\bfx}/R)\big)-\phi^{\prime}\big({\bfw^{[p]T}_{j_2}}({\bfx}/R)\big)|
		\cdot |R\cos\phi_1|^2
		\cdot f_Z(R)R^2\sin \phi_1 dRd\phi_1d\phi_2\\
		=& \int_0^{\infty} R^4f_z(R)dR\int_{0}^{\pi}\int_{0}^{2\pi}|\cos \phi_1|^2\cdot \sin\phi_1
		\cdot|\phi^{\prime}\big(\bfw_{j_2}^T({\bfx}/R)\big)-\phi^{\prime}\big({\bfw^{[p]T}_{j_2}}({\bfx}/R)\big)|d\phi_1d\phi_2\\
		\stackrel{(a)}{\le} & \Revise{3\delta^2} \cdot \int_0^{\infty} R^2f_z(R)dR\int_{0}^{\pi}\int_{0}^{2\pi} \sin\phi_1
		\cdot|\phi^{\prime}\big(\bfw_{j_2}^T({\bfx}/R)\big)-\phi^{\prime}\big({\bfw^{[p]T}_{j_2}}({\bfx}/R)\big)|d\phi_1d\phi_2\\
		= &\Revise{3\delta^2}\cdot\mathbb{E}_{z_1, z_2, z_3}\big|\phi^{\prime}\big(\bfw_{j_2}^T{\bfx}\big)-\phi^{\prime}\big({\bfw^{[p]T}_{j_2}}{\bfx}\big)|\\
		\le & \Revise{3\delta^2}\cdot\mathbb{E}_{\bfx}\big|\phi^{\prime}\big(\bfw_{j_2}^T{\bfx}\big)-\phi^{\prime}\big({\bfw^{[p]T}_{j_2}}{\bfx}\big)|,
		\end{split}
		\end{equation}
    \Revise{where the inequality (a) is derived from the fact that $|cos\phi_1|\le 1$ and 
    \begin{equation}
    \begin{split}
        \int_{0}^{\infty} R^4 \frac{1}{(2\pi \delta^2)^{\frac{3}{2}}}e^{-\frac{R^2}{2\delta^2}}dR
         =&  \int_{0}^{\infty}  -\frac{R^3\delta^2}{(2\pi \delta^2)^{\frac{3}{2}}}d(e^{-\frac{R^2}{2\delta^2}})\\
         =&  \int_{0}^{\infty}e^{-\frac{R^2}{2\delta^2}} d\frac{R^3\delta^2}{(2\pi \delta^2)^{\frac{3}{2}}}\\
         =&3\delta^2\int_{0}^{\infty}R^2\frac{1}{(2\pi \delta^2)^{\frac{3}{2}}}e^{-\frac{R^2}{2\delta^2}}dR.
    \end{split}
    \end{equation}}

	Define a set $\mathcal{A}_1=\{\bfx| ({\bfw^{[p]T}_{j_2}}\bfx)(\bfw_{j_2}^T\bfx)<0 \}$. If $\bfx\in\mathcal{A}_1$, then ${\bfw^{[p]T}_{j_2}}\bfx$ and $\bfw_{j_2}^T\bfx$ have different signs, which means the value of $\phi^{\prime}(\bfw_{j_2}^T\bfx)$ and $\phi^{\prime}({\bfw^{[p]T}_{j_2}}\bfx)$ are different. This is equivalent to say that 
	\begin{equation}\label{eqn:I_1_sub1}
	|\phi^{\prime}(\bfw_{j_2}^T\bfx)-\phi^{\prime}({\bfw^{[p]T}_{j_2}}\bfx)|=
	\begin{cases}
	&1, \text{ if $\bfx\in\mathcal{A}_1$}\\
	&0, \text{ if $\bfx\in\mathcal{A}_1^c$}
	\end{cases}.
	\end{equation}
	Moreover, if $\bfx\in\mathcal{A}_1$, then we have 
	\begin{equation}
	\begin{split}
	|{\bfw^{[p]T}_{j_2}}\bfx|
	\le&|{\bfw^{[p]T}_{j_2}}\bfx-\bfw_{j_2}^T\bfx|
	\le\|{\bfw^{[p]}_{j_2}}-{\bfw_{j_2}}\|_2\cdot\|\bfx\|_2.
	\end{split}
	\end{equation}
	Let us define a set $\mathcal{A}_2$ such that
	\begin{equation}
	\begin{split}
	\mathcal{A}_2
	=&\Big\{\bfx\Big|\frac{|{\bfw^{[p]T}_{j_2}}\bfx|}{\|\bfw_{j_2}^*\|_2\|\bfx\|_2}\le\frac{\|{\bfw_{j_2}^*}-{\bfw_{j_2}}\|_2}{\|\bfw_{j_2}^*\|_2}   \Big\}
	=\Big\{\theta_{\bfx,\bfw_{j_2}^*}\Big||\cos\theta_{\bfx,\bfw^{[p]}_{j_2}}|\le\frac{\|{\bfw^{[p]}_{j_2}}-{\bfw_{j_2}}\|_2}{\|\bfw^{[p]}_{j_2}\|_2}   \Big\}.
	\end{split}
	\end{equation}	
	Hence, we have that
	\begin{equation}\label{eqn:I_1_sub2}
	\begin{split}
	\mathbb{E}_{\bfx}
	|\phi^{\prime}(\bfw_{j_2}^T\bfx)-\phi^{\prime}({\bfw^{[p]T}_{j_2}}\bfx)|^2
	=& \mathbb{E}_{\bfx}
	|\phi^{\prime}(\bfw_{j_2}^T\bfx)-\phi^{\prime}({\bfw^{[p]T}_{j_2}}\bfx)|\\
	=& \text{Prob}(\bfx\in\mathcal{A}_1)\\
	\le& \text{Prob}(\bfx\in\mathcal{A}_2).
	\end{split}
	\end{equation}
	Since $\bfx\sim \mathcal{N}({\bf0},\delta^2\|\bfa\|_2^2 \bfI)$, $\theta_{\bfx,\bfw^{[p]}_{j_2}}$ belongs to the uniform distribution on $[-\pi, \pi]$, we have
	\begin{equation}\label{eqn:I_1_sub3}
	\begin{split}
	\text{Prob}(\bfx\in\mathcal{A}_2)
	=\frac{\pi- \arccos\frac{\|{\bfw^{[p]}_{j_2}}-{\bfw_{j_2}}\|_2}{\|\bfw^{[p]}_{j_2}\|_2} }{\pi}
	\le&\frac{1}{\pi}\tan(\pi- \arccos\frac{\|{\bfw^{[p]}_{j_2}}-{\bfw_{j_2}}\|_2}{\|\bfw^{[p]}_{j_2}\|_2})\\
	=&\frac{1}{\pi}\cot(\arccos\frac{\|{\bfw^{[p]}_{j_2}}-{\bfw_{j_2}}\|_2}{\|\bfw^{[p]}_{j_2}\|_2})\\
	\le&\frac{2}{\pi}\frac{\|{\bfw^{[p]}_{j_2}}-{\bfw_{j_2}}\|_2}{\|\bfw^{[p]}_{j_2}\|_2}.
	\end{split}
	\end{equation}

	Hence,  \eqref{eqn: ean111} and \eqref{eqn:I_1_sub3} suggest that
	\begin{equation}\label{eqn:I_1_bound}
	I\le\frac{6\delta^2}{\pi}\frac{\|\bfw_{j_2} -\bfw^{[p]}_{j_2}\|_2}{\sigma_K} \cdot\|\bfa\|_2^2.
	\end{equation}
	The same bound that shown in \eqref{eqn:I_1_bound} holds for $\bfP_2$ as well.  
	
	$\bfP_3$ and $\bfP_4$ satisfy \eqref{eqn:I_1_bound} except for changing $\delta^2$ to $\de^2$.
	
	Therefore, we have 
	\begin{equation}
	    \begin{split}
	    &\| \nabla^2f(\Wp;p) - \nabla^2f(\bfW;p)\|_2\\
	    =&\max_{\|\boldsymbol{\alpha}\|_2\le 1} \Big|\boldsymbol{\alpha}^T(\nabla^2f(\Wp;p) - \nabla^2f(\bfW;p))\boldsymbol{\alpha}\Big|\\
	    \le&\sum_{j_1=1}^K\sum_{j_2=1}^K\Bigg|\boldsymbol{\alpha}_{j_1}^T\bigg(\frac{\partial^2 f}{\partial {\bfw}_{j_1}\partial {\bfw}_{j_2}}(\Wp;p)
	    -
	    \frac{\partial^2 f}{\partial {\bfw}_{j_1}\partial {\bfw}_{j_2}}(\bfW;p)\bigg)\boldsymbol{\alpha}_{j_2}\Bigg|\\
	    \le &\frac{1}{K^2}\sum_{j_1=1}^K\sum_{j_2=1}^K\Big(\lambda \|\bfP_1+\bfP_2\|_2 + (1-\lambda)\|\bfP_3+\bfP_4\|_2\Big)\|\boldsymbol{\alpha}_{j_1}\|_2 \|\boldsymbol{\alpha}_{j_2}\|_2\\
	    \le & \frac{1}{K^2}\sum_{j_1=1}^K\sum_{j_2=1}^K4(\lambda\delta^2+(1-\lambda)\de^2)\frac{\|\bfw^{[p]}_{j_2}-\bfw_{j_2}\|_2}{\sigma_K}\|\boldsymbol{\alpha}_{j_1}\|_2 \|\boldsymbol{\alpha}_{j_2}\|_2\\
	    \le & \frac{4}{K}\big(\lambda\delta^2+(1-\lambda)\de^2\big)\cdot\frac{\|\Wp-\bfW\|_2}{\sigma_K},
	    \end{split}
	\end{equation}
	where $\boldsymbol{\alpha}\in \mathbb{R}^{Kd}$ and  $\boldsymbol{\alpha}_{j}\in \mathbb{R}^d$ with $\boldsymbol{\alpha} =[\boldsymbol{\alpha}_{1}^T, \boldsymbol{\alpha}_{2}^T, \cdots, \boldsymbol{\alpha}_{K}^T]^T$.
\end{proof}

\Revise{
\section{Initialization via tensor method}\label{sec: initialization}
In this section, we briefly summarize the tensor initialization in \citep{ZSJB17} by studying the target function class as 
\begin{equation}\label{eqn: two_layer}
    y = \frac{1}{K}\sum_{j=1}^K v_j^* \phi(\bfw_j^{*T}\bfx),
\end{equation}
where $v_j^*\in R$.
Note that for ReLU function, we have $v_j^* \phi(\bfw_j^{*T}\bfx) = \text{sign}(v_j^*) \phi(|v_j^*|\bfw_j^{*T}\bfx)$. Without loss of generalization, we can assume $v_j^*\in \{+1, -1\}$. Additionally, it is clear that the function studied in \eqref{eqn: teacher_model} is the special case of \eqref{eqn: two_layer} when $v_j^*=1$ for all $j$. In addition, Theorem 5.6 in \citep{ZSJB17} show that the sign of $v_j^*$ can be directly recovered using tensor initialization, which indicates the the equivalence of \eqref{eqn: teacher_model} and \eqref{eqn: two_layer} when using tensor initialization.}



\Revise{We first define some high order momenta in the following 
way:
\begin{equation}\label{eqn: M_1}
\bfM_{1} = \mathbb{E}_{\bfx}\{y \bfx \}\in \mathbb{R}^{d},
\end{equation}
\begin{equation}\label{eqn: M_2}
\bfM_{2} = \mathbb{E}_{\bfx}\Big[y\big(\bfx\otimes \bfx-\delta^2\bfI\big)\Big]\in \mathbb{R}^{d\times d},
\end{equation}
\begin{equation}\label{eqn: M_3}
\bfM_{3} = \mathbb{E}_{\bfx}\Big[y\big(\bfx^{\otimes 3}- \bfx\widetilde{\otimes} \delta^2\bfI  \big)\Big]\in \mathbb{R}^{d\times d \times d},
\end{equation}
where $\mathbb{E}_{\bfx}$ is the expectation over $\bfx$ and $\bfz^{\otimes 3} := \bfz \otimes \bfz \otimes \bfz$. The operator $\widetilde{\otimes}$ is defined as    
\begin{equation}
\bfv\widetilde{\otimes} \bfZ=\sum_{i=1}^{d_2}(\bfv\otimes \bfz_i\otimes \bfz_i +\bfz_i\otimes \bfv\otimes \bfz_i + \bfz_i\otimes \bfz_i\otimes \bfv),
\end{equation} 
for any vector $\bfv\in \mathbb{R}^{d_1}$ and $\bfZ\in \mathbb{R}^{d_1\times d_2}$.}

\Revise{Following the same calculation formulas in the Claim 5.2 \citep{ZSJB17},  there exist some known constants $\psi_i, i =1, 2, 3$, such that
\begin{equation}\label{eqn: M_1_2}
\bfM_{1} = \sum_{j=1}^{K} \psi_1\cdot \|{\bfw}_{j}^*\|_2\cdot\overline{\bfw}_j^*,
\end{equation}
\begin{equation}\label{eqn: M_2_2}
\bfM_{2} = \sum_{j=1}^{K} \psi_2\cdot \|{\bfw}_{j}^*\|_2\cdot\overline{\bfw}_{j}^* \overline{\bfw}_{j}^{*T},
\end{equation}\label{eqn: M_3_2}
\begin{equation}\label{eqn:M_3_v2}
\bfM_{3} = \sum_{j=1}^{K} \psi_3\cdot \|{\bfw}_{j}^*\|_2\cdot\overline{\bfw}_{j}^{*\otimes3},
\end{equation} 
where $\overline{\bfw}^*_{j}={\bfw}_{j}^*/\|{\bfw}_{j}^*\|_2$ in \eqref{eqn: M_1}-\eqref{eqn: M_3} is the normalization of ${\bfw}_{j}^*$. Therefore, we can see that the information of $\{\bfw_j^*\}_{j=1}^K$ are separated as the direction of $\bfw_j$ and the magnitude of $\bfw_j$ in $M_1$, $M_2$ and $M_3$.}

\Revise{$\bfM_{1}$, $\bfM_{2}$ and $\bfM_{3}$ can be estimated through the samples $\big\{(\bfx_n, y_n)\big\}_{n=1}^{N}$, and let $\widehat{\bfM}_{1}$, $\widehat{\bfM}_{2}$, $\widehat{\bfM}_{3}$ denote the corresponding estimates. 
First, we will decompose the rank-$K$ tensor $\bfM_{3}$ and obtain the $\{\overline{\bfw}^*_{j}\}_{j=1}^K$. By applying the tensor decomposition method \citep{KCL15} to $\widehat{\bfM}_{3}$, the outputs, denoted by $\widehat{\overline{\bfw}}_{j}^*$, are the estimations of $\{\bfs_j\overline{\bfw}^*_{j}\}_{j=1}^K$, where $s_j$ is an unknown sign.
Second, we will estimate $s_j$, $\bfv_j^*$ and $\|\bfw_j^*\|_2$ through $\bfM_{1}$ and $\bfM_{2}$. Note that $\bfM_{2}$ does not contain the information of $\bfs_j$ because $\bfs_j^2$ is always $1$. Then, through solving the following two optimization problem:
\begin{equation}\label{eqn: int_op}
\begin{gathered}
\widehat{\boldsymbol{\alpha}}_1 = \arg\min_{\boldsymbol{\alpha}_1\in\mathbb{R}^K}:\quad  \Big|\widehat{\bfM}_{1} - \sum_{j=1}^{K}\psi_1 \alpha_{1,j} \widehat{\overline{\bfw}}^*_{j}\Big|,\\
\widehat{\boldsymbol{\alpha}}_2 = \arg\min_{\boldsymbol{\alpha}_2\in\mathbb{R}^K}:\quad  \Big|\widehat{\bfM}_{2} - \sum_{j=1}^{K}\psi_2 \alpha_{2,j} \widehat{\overline{\bfw}}^*_{j} {\widehat{\overline{\bfw}}_j^{*T}}\Big|,
\end{gathered}
\end{equation}
The estimation of $s_j$ can be given as 
$$\hat{s}_j = \text{sign}(\widehat{\alpha}_{1,j}/\widehat{\alpha}_{2,j}).$$ 
Also, we know that $|\widehat{\alpha}_{1,j}|$ is the estimation of 
$\|\bfw_j^*\|$ and 
$$\hat{v}_j = \text{sign}(\widehat{\alpha}_{1,j}/s_j)= \text{sign}(\widehat{\alpha}_{2,j}).$$
Thus, 
$\bfW^{(0)}$ is given as 
 $$\begin{bmatrix}
 \text{sign}(\widehat{\alpha}_{2,1})\widehat{\alpha}_{1,1}\widehat{\overline{\bfw}}^*_{1}, &\cdots,& \text{sign}(\widehat{\alpha}_{2,K})\widehat{\alpha}_{1,K}
 \widehat{\overline{\bfw}}^*_{K}
 \end{bmatrix}.$$}
% $\bfM_{1}$, $\bfM_{2}$ and $\bfM_{3}$ can be estimated through the samples $\big\{(\bfx_n, y_n)\big\}_{n=1}^{N}$, and let $\widehat{\bfM}_{1}$, $\widehat{\bfM}_{2}$, $\widehat{\bfM}_{3}$ denote the corresponding estimates. 
% First, we will decompose the rank-$k$ tensor $\bfM_{3}$ and obtain the $\{\overline{\bfw}^*_{j}\}_{j=1}^K$. By applying the tensor decomposition method \citep{KCL15} to $\widehat{\bfM}_{3}$, the outputs, denoted by $\{\widehat{\overline{\bfw}}_{j}^*\}_{j=1}^K$, are the estimations of $\{\overline{\bfw}^*_{j}\}_{j=1}^K$.
% Next, we will estimate $\|\bfw_j^*\|_2$ through solving the following optimization problem:
% \begin{equation}\label{eqn: int_op}
% \begin{gathered}
% \widehat{\boldsymbol{\alpha}} = \arg\min_{\boldsymbol{\alpha}\in\mathbb{R}^K}:\quad  \Big|\widehat{\bfM}_{1} - \sum_{j=1}^{K}\psi_1 \alpha_{j} \widehat{\overline{\bfw}}^*_{j}\Big|,\\
% % \widehat{\boldsymbol{\alpha}}_2 = \arg\min_{\boldsymbol{\alpha}_2\in\mathbb{R}^K}:\quad  \Big|\widehat{\bfM}_{i,2} - \sum_{j=1}^{K}\psi_2 \alpha_{2,j} \widehat{\overline{\bfw}}^*_{j} {\widehat{\overline{\bfw}}_j^{*T}}\Big|,
% \end{gathered}
% \end{equation}
%  From \eqref{eqn: M_1_2} and \eqref{eqn: int_op},
%  we know that $|\widehat{\alpha}_{j}|$ is the estimation of $\|\bfw_j^*\|_2$. Thus, 
% $\widehat{\bfw}$ is given as 
% $\big[
% |\widehat{\alpha}_{1}|\widehat{\overline{\bfw}}^*_{1}, \cdots, |\widehat{\alpha}_{j}|\widehat{\overline{\bfw}}^*_{j}, \cdots, |\widehat{\alpha}_{K}|\widehat{\overline{\bfw}}^*_{K}
% \big]$.


\floatname{algorithm}{Subroutine}
\setcounter{algorithm}{0}
\begin{algorithm}[h]
	\caption{Tensor Initialization Method}\label{Alg: initia_snn}
	\begin{algorithmic}[1]
		\State \textbf{Input:} labeled data $\mathcal{D}=\{(\bfx_n, y_n) \}_{n=1}^{N}$;
		\State Partition $\mathcal{D}$ into three disjoint subsets $\mathcal{D}_1$, $\mathcal{D}_2$, $\mathcal{D}_3$;
		\State Calculate $\widehat{\bfM}_{1}$, $\widehat{\bfM}_{2}$ {following \eqref{eqn: M_1}, \eqref{eqn: M_2}} using $\mathcal{D}_1$, $\mathcal{D}_2$, respectively;
		\State Obtain the estimate subspace $\widehat{\bfV}$ of $\widehat{\bfM}_{2}$;
		\State Calculate $\widehat{\bfM}_{3}(\widehat{\bfV},\widehat{\bfV},\widehat{\bfV})$  through $\mathcal{D}_3$;
		\State Obtain $\{ \widehat{\bfs}_j \}_{j=1}^K$ via {tensor decomposition method \citep{KCL15}} on $\widehat{\bfM}_{3}(\widehat{\bfV},\widehat{\bfV},\widehat{\bfV})$;
		\State Obtain $\widehat{\boldsymbol{\alpha}}_1$, $\widehat{\boldsymbol{\alpha}}_2$ by solving  optimization problem $\eqref{eqn: int_op}$;
		\State \textbf{Return:}  $\bfw^{(0)}_j=\text{sign}(\widehat{\alpha}_{2,j})\widehat{\alpha}_{1,j}\widehat{\bfV}\widehat{\bfu}_j$ and ${v}_j^{(0)}=\text{sign}(\widehat{{\alpha}}_{2,j}) $, {$j=1,...,K$.}
	\end{algorithmic}
\end{algorithm}

\Revise{To reduce the computational complexity of tensor decomposition, one can project $\widehat{\bfM}_{3}$ to a lower-dimensional tensor \citep{ZSJB17}. The idea is to first estimate the subspace spanned by $\{\bfw_{j}^* \}_{j=1}^{K}$, and let $\widehat{\bfV}$ denote the estimated subspace. 
Moreover, we have 
\begin{equation}\label{eqn: M_3_vv2}
\bfM_{3}(\widehat{\bfV},\widehat{\bfV},\widehat{\bfV}) = \mathbb{E}_{\bfx}\Big[y\big((\widehat{\bfV}^T\bfx)^{\otimes 3}- (\widehat{\bfV}^T\bfx)\widetilde{\otimes} \mathbb{E}_{\bfx}(\widehat{\bfV}^T\bfx)(\widehat{\bfV}^T\bfx)^T  \big)\Big]\in \mathbb{R}^{K\times K \times K},
\end{equation}
Then, one can decompose the estimate $\widehat{\bfM}_{3}(\widehat{\bfV}, \widehat{\bfV}, \widehat{\bfV})$ to obtain unit vectors $\{\hat{\bfs}_j \}_{j=1}^K \in \mathbb{R}^{K}$.
Since $\overline{\bfw}^*$ lies in the subspace $\bfV$, we have $\bfV\bfV^T\overline{\bfw}_j^*=\overline{\bfw}_j^*$. Then, $\widehat{\bfV}\hat{\bfs}_j$ is an estimate of $\overline{\bfw}_j^*$. 
The initialization process is summarized in Subroutine \ref{Alg: initia_snn}.
}

\Revise{
\section{Classification Problems}
The framework in this paper is extendable to binary classification problem. For binary classification problem, the output $y$ given input $\bfx$ is defined as 
\begin{equation}
    \text{Prob}\{ y= 1 \} = g(\bfW^*;\bfx)
\end{equation}
with some ground truth parameter $\bfW^*$. To guarantee the output is within $[0,1]$, the activation function is often used as sigmoid. For classification, the loss function is cross-entropy, and the objective function over labeled data $\mathcal{D}$ is defined as 
\begin{equation}
    f_{\mathcal{D}}(\bfW) = \frac{1}{N} \sum_{(\bfx_n,y_n)\in \mathcal{D}} -y_n\log g(\bfW;\bfx_n) - (1-y_n) \log (1-g(\bfW;\bfx_n)).    
\end{equation}
The expectation of objective function can be written as
\begin{equation}\label{eqn: class_prf}
    \begin{split}
    \mathbb{E}_{\mathcal{D}}f_{\mathcal{D}}(\bfW) 
    =& \mathbb{E}_{(\bfx,y)} -y\log(g(\bfW;\bfx_n)) - (1-y)\log(1-g(\bfW;\bfx))\\
    =&  \mathbb{E}_{\bfx}\mathbb{E}_{(y|\bfx)} -y\log(g(\bfW;\bfx_n)) - (1-y)\log(1-g(\bfW;\bfx))\\
    =& \mathbb{E}_{\bfx}\Big[ -g(\bfW^*;\bfx)\log(g(\bfW;\bfx_n)) - (1-g(\bfW^*;\bfx))\log(1-g(\bfW;\bfx_n))\Big]
    \end{split}
\end{equation}
Please note that \eqref{eqn: class_prf} is exactly the same as \eqref{eqn: population_risk_function} with $\lambda=1$ when the loss function is squared loss.}

\Revise{
For cross entropy loss function, the second order derivative of \eqref{eqn: class_prf} is calculated as 
\begin{equation}
\begin{split}
\frac{\partial f_{\mathcal{D}}(\bfW)}{\partial \bfw_j \partial \bfw_k} 
=\frac{1}{N}[\frac{y_n}{g^2(\bfW;\bfx)} + \frac{1-y_n}{(1-g(\bfW;\bfx))^2}]\cdot \phi'(\bfw_j^T\bfx)\phi'(\bfw_k^T\bfx)\bfx\bfx^T.
\end{split}
\end{equation}
when $j\neq k$.
Refer to (88) in \citep{FCL20} or (132) in \citep{ZWLC20_2}, we have 
\begin{equation}
\begin{split}
        \Big\|\frac{y_n(\phi'(\bfw_j^T\bfx)\phi'(\bfw_k^T\bfx))}{g^2(\bfW;\bfx)}\Big\|_2
    \le&\Big\|\frac{\phi'(\bfw_j^T\bfx)\phi'(\bfw_k^T\bfx)}{g^2(\bfW;\bfx)}\Big\|_2
    \le K^2. 
\end{split}
\end{equation}
Following similar steps in \eqref{eqn: temppp}, from Defintion \ref{Def: sub-exponential}, we know that $\alpha_j^T\frac{\partial f_{\mathcal{D}}(\bfW)}{\partial \bfw_j \partial \bfw_k}\alpha_k$ belongs to the sub-exponential distribution. Therefore, similiar results for objective function with cross-entropy loss can be established as well. One can check \citep{FCL20}  or \citep{ZWLC20_2} for details.}



\Revise{\section{One-hidden layer neural network with top layer weights}\label{sec: two_layer}}
\Revise{For a general one-hidden layer neural network, the output of the neural network is defined as 
\begin{equation}\label{eqn: two_layer_n}
    g(\bfW,\bfv;\bfx) = \frac{1}{K}\sum_{j=1}^K v_j \phi(\bfw_j^{T}\bfx),
\end{equation}
where $\bfv = [v_1, v_2, \cdots, v_K]\in R^K$. Then, the target function can be defined as 
\begin{equation}\label{eqn: two_layer_*}
    y = g(\bfW^*,\bfv^*;\bfx) = \frac{1}{K}\sum_{j=1}^K v_j^* \phi(\bfw_j^{*T}\bfx)
\end{equation}
for some unknown weights $\bfW^*$ and $\bfv^*$.}

\Revise{In the following paragraphs, we will provide a short description for the equivalence of \eqref{eqn: two_layer_*} and \eqref{eqn: teacher_model} in theoretical analysis.
Note that for ReLU functions, we have $v_j \phi(\bfw_j^{T}\bfx) = \text{sign}(v_j) \phi(|v_j|\bfw_j^{T}\bfx)$. Without loss of generalization, we can assume $v_j, v_j^*\in \{+1, -1\}$ for all $j\in[K]$\footnote{To see this, one can view $|v_j^*| \bfw^{*}_j$ as the new ground truth weights, and the goal for this paper is to recover the new ground truth weights.}. From Appendix \ref{sec: initialization}, we know that the sign of $v_j^*$ can exactly estimated through tensor initialization. There, we can focus on analysis the neural network in the form as 
\begin{equation}\label{eqn: two_layer_1}
    g(\bfW;\bfx) = \frac{1}{K}\sum_{j=1}^K v_j^* \phi(\bfw_j^{T}\bfx).
\end{equation}
Considering the objective function in \eqref{eqn: empirical_risk_function}  and population risk function in \eqref{eqn: p_population_risk_function}, we have 
\begin{equation}
\begin{split}
    &\Big\|\frac{\partial \hat{f} }{ \partial \bfw_k } (\bfW) - \frac{\partial {f} }{ \partial \bfw_k} (\bfW;p)\Big\|_2\\
    = & \Big\|\frac{\lambda}{K^2N} \sum_{j=1}^K v_j^*\Big[ \sum_{n=1}^N\big( \phi(\bfw_j^T\bfx_n) - \phi(\bfw_j^{*T}\bfx_n)\big)\bfx_n - \mathbb{E}_{\bfx}\big( \phi(\bfw_j^T\bfx) -\phi(\bfw^{[p]T}_j\bfx) \big)\bfx 
    \Big]\\
    &+ \frac{1-\lambda}{K^2M} v_j^*\sum_{j=1}^K \Big[ \sum_{m=1}^M\big( \phi(\bfw_j^T\w[\bfx]_m) - \phi(\w[\bfw]_j^T\w[\bfx]_m)\big)\w[\bfx]_m - \mathbb{E}_{\w[\bfx]}\big( \phi(\bfw_j^T\w[\bfx]) -\phi(\bfw^{[p]T}_j\w[\bfx]) \big)\w[\bfx] 
            \Big]\Big\|_2\\
    \le& \sum_{j=1}^K \cdot |v_j^*| \cdot \Big\|\frac{\lambda}{K^2N} \Big[ \sum_{n=1}^N\big( \phi(\bfw_j^T\bfx_n) - \phi(\bfw_j^{*T}\bfx_n)\big)\bfx_n - \mathbb{E}_{\bfx}\big( \phi(\bfw_j^T\bfx) -\phi(\bfw^{[p]T}_j\bfx) \big)\bfx 
    \Big]\\
    &+\frac{1-\lambda}{K^2M} \Big[ \sum_{m=1}^M\big( \phi(\bfw_j^T\w[\bfx]_m) - \phi(\w[\bfw]_j^T\w[\bfx]_m)\big)\w[\bfx]_m - \mathbb{E}_{\w[\bfx]}\big( \phi(\bfw_j^T\w[\bfx]) -\phi(\bfw^{[p]T}_j\w[\bfx]) \big)\w[\bfx] 
            \Big]\Big\|_2\\
    =& \sum_{j=1}^K \Big\| \frac{\lambda}{K^2N}\Big[ \sum_{n=1}^N\big( \phi(\bfw_j^T\bfx_n) - \phi(\bfw_j^{*T}\bfx_n)\big)\bfx_n - \mathbb{E}_{\bfx}\big( \phi(\bfw_j^T\bfx) -\phi(\bfw^{[p]T}_j\bfx) \big)\bfx 
    \Big]\\
    &+\frac{1-\lambda}{K^2M} \Big[ \sum_{m=1}^M\big( \phi(\bfw_j^T\w[\bfx]_m) - \phi(\w[\bfw]_j^T\w[\bfx]_m)\big)\w[\bfx]_m - \mathbb{E}_{\w[\bfx]}\big( \phi(\bfw_j^T\w[\bfx]) -\phi(\bfw^{[p]T}_j\w[\bfx]) \big)\w[\bfx] 
            \Big]\Big\|_2,\\
\end{split}
\end{equation}
which is exact the same as \eqref{eqn: Lemma2_temp}. Similar results can be derived for Lemma \ref{Lemma: p_Second_order_distance}. Therefore, the conclusions and proofs of Lemma \ref{Lemma: p_second_order_derivative bound} and Lemma \ref{Lemma: p_first_order_derivative} does not change at all.}

\Revise{Additionally, fixing the second-layer weights and only training the hidden layer is the state-of-the-art practice in analyzing two-layer neural networks \citep{ADHL19,ADHLW19,ALL19,SS18,LL18,BG17, OS18, ZYWG19}. Additionally, as indicated in \citep{SS18},  training a one-hidden-layer neural network  with all $v_j$ fixed as $1$ has intractable many spurious local minima, which indicates that training problem is not trivial.}


% \begin{proof}[Proof of Lemma \ref{Lemma: first_order_distance}]
%     From \eqref{eqn: empirical_risk_function}, we know that 
%     \begin{equation}
%         \begin{split}
%         \frac{\partial \hat{f}}{\partial \bfw_k}(\bfW) 
%         =& \frac{\lambda}{N}\sum_{n=1}^N \Big( \frac{1}{K}\sum_{j=1}^K\phi(\bfw_j^T\bfx_n) - y_n \Big)\bfx_n
%          +\frac{1-\lambda}{M}\sum_{m=1}^M \Big( \frac{1}{K}\sum_{j=1}^K\phi(\bfw_j^T\w[\bfx]_m) - \w[y]_n \Big)\w[\bfx]_m\\
%         =& \frac{\lambda}{K^2N}\sum_{n=1}^N \sum_{j=1}^K\Big( \phi(\bfw_j^T\bfx_n)-\phi(\bfw_j^{*T}\bfx_n) \Big)\bfx_n \\
%          & + \frac{1-\lambda}{K^2M}\sum_{m=1}^M \sum_{j=1}^K\Big( \phi(\bfw_j^T\w[\bfx]_m)-\phi(\w[\bfw]_j^T\w[\bfx]_m) \Big)\w[\bfx]_m.
%         \end{split}
%     \end{equation}
%     From \eqref{eqn: population_risk_function}, we know that
%     \begin{equation}
%         \begin{split}
%         \frac{\partial \hat{f}}{\partial \bfw_k}(\bfW) 
%         = \frac{\lambda}{K^2}\mathbb{E}_{\bfx} \sum_{j=1}^K\Big( \phi(\bfw_j^T\bfx)-\phi(\bfw_j^{*T}\bfx) \Big)\bfx
%          + \frac{1-\lambda}{K^2}\mathbb{E}_{\w[\bfx]} \sum_{j=1}^K\Big( \phi(\bfw_j^T\w[\bfx])-\phi(\w[\bfw]_j^T\w[\bfx]) \Big)\w[\bfx].
%         \end{split}
%     \end{equation}
%     Then, we have 
%     \begin{equation}
%         \begin{split}
%             &\frac{\partial \hat{f} }{ \partial \bfw_k } (\bfW) - \frac{\partial {f} }{ \partial \bfw_k} (\bfW)\\
%             = & \frac{\lambda}{K^2N} \sum_{j=1}^K \Big[ \sum_{n=1}^N\big( \phi(\bfw_j^T\bfx_n) - \phi(\bfw_j^{*T}\bfx_n)\big)\bfx_n - \mathbb{E}_{\bfx}\big( \phi(\bfw_j^T\bfx) -\phi(\bfw^{*T}_j\bfx) \big)\bfx 
%             \Big]\\
%              &+ \frac{1-\lambda}{K^2M} \sum_{j=1}^K \Big[ \sum_{m=1}^M\big( \phi(\bfw_j^T\w[\bfx]_m) - \phi(\w[\bfw]_j^T\w[\bfx]_m)\big)\w[\bfx]_m - \mathbb{E}_{\w[\bfx]}\big( \phi(\bfw_j^T\w[\bfx]) -\phi(\bfw^{*T}_j\w[\bfx]) \big)\w[\bfx] 
%             \Big]\\
%             = & \frac{\lambda}{K^2} \sum_{j=1}^K \Big[ \frac{1}{N}\sum_{n=1}^N\big( \phi(\bfw_j^T\bfx_n) - \phi(\bfw_j^{*T}\bfx_n)\big)\bfx_n - \mathbb{E}_{\bfx}\big( \phi(\bfw_j^T\bfx) -\phi(\bfw^{*T}_j\bfx) \big)\bfx 
%             \Big]\\
%              & + \frac{1-\lambda}{K^2} \sum_{j=1}^K \Big[ \frac{1}{M}\sum_{m=1}^M\big( \phi(\bfw_j^T\w[\bfx]_m) - \phi(\w[\bfw]_j^T\w[\bfx]_m)\big)\w[\bfx]_m - \mathbb{E}_{\w[\bfx]}\big( \phi(\bfw_j^T\w[\bfx]) -\phi(\w[\bfw]^T_j\w[\bfx]) \big)\w[\bfx] 
%             \Big]\\
%             & + \frac{1-\lambda}{K^2}\sum_{j=1}^K \mathbb{E}_{\w[\bfx]}\Big[ \big( \phi(\w[\bfw]_j^T\w[\bfx]) - \phi(\bfw^{*T}_j\w[\bfx]) \big)\w[\bfx]  \Big].
%         \end{split}
%     \end{equation}
%     For any $\boldsymbol{\alpha}_j \in \mathbb{R}^{d}$ with $\| \boldsymbol{\alpha}_j \|_2 \le 1$, we define a random variable $Z(j) = \big( \phi(\bfw_j^T\bfx) - \phi(\bfw_j^{*T}\bfx)\big)\boldsymbol{\alpha}^T_j\bfx$ and $Z_n(j) = \big( \phi(\bfw_j^T\bfx_n) - \phi(\bfw_j^{*T}\bfx_n)\big)\boldsymbol{\alpha}^T_j\bfx_n$ as the realization of $Z(j)$ for $n=1,2\cdots, N$. Then, for any $p\in \mathbb{N}^+$, we have 
%     \begin{equation}
%         \begin{split}
%         \big(\mathbb{E}|Z|^p\big)^{1/p}
%         =& \Big( \mathbb{E} |\phi(\bfw_j^T\bfx)-\phi(\bfw_j^{*T}\bfx)|^p \cdot |\boldsymbol{\alpha}_j^T\bfx|^p \Big)^{1/p}\\
%         \le& \Big( \mathbb{E} |(\bfw_j-\bfw_j^*)^T\bfx|^p \cdot |\boldsymbol{\alpha}_j^T\bfx|^p \Big)^{1/p}\\
%         \le& C \cdot \delta^2 \| \bfw_j - \bfw_j^* \|_2 \cdot p, 
%         \end{split}
%     \end{equation}
%     where $C$ is a positive constant and the last inequality holds since $\bfx\sim \mathcal{N}(0, \delta^2)$. From Definition \ref{Def: sub-exponential}, we know that $Z$ belongs to sub-exponential distribution with $\|Z\|_{\psi_1}\lesssim \delta^2 \| \bfw_j - \bfw_j^* \|_2$.
%     Therefore, by Chernoff inequality, we have 
%     \begin{equation}
%         \mathbb{P}\bigg\{ \Big| \frac{1}{N}\sum_{n=1}^N Z_n(j) -\mathbb{E}Z(j) \Big| < t \bigg\} \le 1- \frac{e^{-C(\delta^2\| \bfw_j - \bfw_j^* \|_2)^2\cdot Ns^2}}{e^{Nst}}
%     \end{equation}
%     for some positive constant $C$ and any $s\in\mathbb{R}$. 
    
%     Let $t=\delta^2\|\bfw_j-\bfw_j^*\|_2\sqrt{\frac{d\log q}{N}}$ and $s = \frac{2}{C\delta^2\|\bfw_j-\bfw_j^*\|_2}\cdot t$ for some large constant $q>0$, we have
%     \begin{equation}
%         \begin{split}
%                 \Big| \frac{1}{N}\sum_{n=1}^N Z_n(j) -\mathbb{E}Z(j) \Big| \lesssim \delta^2\|\bfw_j-\bfw_j^*\|_2 \cdot \sqrt{\frac{d\log q}{N}}
%         \end{split}
%     \end{equation}
%     with probability at least $1-q^{-d}$.
%     From Lemma \ref{Lemma: spectral_norm_on_net}, we have 
%     \begin{equation}\label{eqn:first_order_term1}
%     \begin{split}
%       &\Big\| \frac{1}{N}\sum_{n=1}^N\big( \phi(\bfw_j^T\bfx_n) - \phi(\bfw_j^{*T}\bfx_n)\big)\bfx_n - \mathbb{E}_{\bfx}\big( \phi(\bfw_j^T\bfx) -\phi(\bfw^{*T}_j\bfx) \big)\bfx\Big\|_2\\
%       \le& 2 \delta^2\|\bfw_j-\bfw_j^*\|_2 
%       \cdot \sqrt{\frac{d\log q}{N}}
%     \end{split}
%     \end{equation}
%     with probability at least $1-(q/5)^{-d}$. Since $q$ is a large constant, we release the probability as $1-q^{-d}$ for simplification. 
%     Similar to $Z$, we have  
%     \begin{equation}\label{eqn:first_order_term2}
%         \begin{split}
%         &\Big\|\frac{1}{M}\sum_{m=1}^M\big( \phi(\bfw_j^T\w[\bfx]_m) - \phi(\w[\bfw]_j^T\w[\bfx]_m)\big)\w[\bfx]_m - \mathbb{E}_{\w[\bfx]}\big( \phi(\bfw_j^T\w[\bfx]) -\phi(\w[\bfw]^T_j\w[\bfx]) \big)\w[\bfx]\Big\|_2\\
%         \lesssim& \de^2\|\bfw_j-\w[\bfw]_j\|_2 \cdot \sqrt{\frac{d\log q}{M}}
%         \end{split}
%     \end{equation}
%     with probability at least $1-q^{-d}$.
    
%     \begin{figure}[h]
%   	\centering
%   	\includegraphics[width=0.4\linewidth]{Figure/circle_w.pdf}
%   	\caption{The subspace spanned by $\bfw_j^*$ and $\w[\bfw]_j$}
%   	\label{fig:circle}
%     \end{figure}
%     For term $\mathbb{E}_{\w[\bfx]}\Big[ \big( \phi(\w[\bfw]_j^T\w[\bfx]) - \phi(\bfw^{*T}_j\w[\bfx]) \big)\w[\bfx]  \Big]$, let us define the angle between $\bfw_j^*$ and $\w[\bfw]_j$ as $\theta$. Figure \ref{fig:circle} shows the subspace spanned by the vector $\bfw_j^*$ and $\w[\bfw]_j$. We divide the subspace by 4 pieces, where the gray region denotes area I, and blue area denotes area II. Areas III and IV are the symmetries of II and I from the origin, respectively. Hence, we have 
%     \begin{equation}
%         \begin{split}
%             &\mathbb{E}_{\w[\bfx]}\Big[ \big( \phi(\w[\bfw]_j^T\w[\bfx]) - \phi(\bfw^{*T}_j\w[\bfx]) \big)\w[\bfx]  \Big]\\
%             =&\mathbb{E}_{\w[\bfx]\in \text{ area I} }\Big[ \big( \phi(\w[\bfw]_j^T\w[\bfx]) - \phi(\bfw^{*T}_j\w[\bfx]) \big)\w[\bfx]  \Big]
%             +\mathbb{E}_{\w[\bfx]\in \text{ area II} }\Big[ \big( \phi(\w[\bfw]_j^T\w[\bfx]) - \phi(\bfw^{*T}_j\w[\bfx]) \big)\w[\bfx]  \Big]\\
%             &+\mathbb{E}_{\w[\bfx]\in \text{ area III} }\Big[ \big( \phi(\w[\bfw]_j^T\w[\bfx]) - \phi(\bfw^{*T}_j\w[\bfx]) \big)\w[\bfx]  \Big]
%             +\mathbb{E}_{\w[\bfx]\in \text{ area IV} }\Big[ \big( \phi(\w[\bfw]_j^T\w[\bfx]) - \phi(\bfw^{*T}_j\w[\bfx]) \big)\w[\bfx]  \Big]\\
%             =&\mathbb{E}_{\w[\bfx]\in \text{ area I} }\big[ (\w[\bfw]_j - \bfw^{*}_j)^T\w[\bfx] \w[\bfx] \big]
%             + \mathbb{E}_{\w[\bfx]\in \text{ area II} }\big[ \bfw^{*T}_j\w[\bfx]\w[\bfx] \big] 
%             + \mathbb{E}_{\w[\bfx]\in \text{ area III} }\big[ \w[\bfw]^T_j\w[\bfx]\w[\bfx] \big]\\
%             =&\mathbb{E}_{\w[\bfx]\in \text{ area I} }\big[ (\w[\bfw]_j - \bfw^{*}_j)^T\w[\bfx] \w[\bfx] \big]
%             + \mathbb{E}_{\w[\bfx]\in \text{ area II} }\big[ (\bfw^{*}_j-\w[\bfw]_j)^T\w[\bfx]\w[\bfx] \big] \\
%         \end{split}
%     \end{equation}
%     Therefore, we have 
%     \begin{equation}\label{eqn:first_order_term3}
%         \begin{split}
%             &\left|\boldsymbol{\alpha}_j^T\mathbb{E}_{\w[\bfx]}\Big[ \big( \phi(\w[\bfw]_j^T\w[\bfx]) - \phi(\bfw^{*T}_j\w[\bfx]) \big)\w[\bfx]  \Big]\right|\\
%             \le & \left| \mathbb{E}_{\w[\bfx]\in \text{ area I} }\big[ (\w[\bfw]_j - \bfw^{*}_j)^T\w[\bfx] (\boldsymbol{\alpha}_j^T\w[\bfx]) \big]
%             + \mathbb{E}_{\w[\bfx]\in \text{ area II} }\big[ (\bfw^{*}_j-\w[\bfw]_j)^T\w[\bfx]\boldsymbol({\alpha}_j^T\w[\bfx]) \big] \right|\\
%             \le & \left| \mathbb{E}_{\w[\bfx]\in \text{ area I} }\big[ (\w[\bfw]_j - \bfw^{*}_j)^T\w[\bfx] (\boldsymbol{\alpha}_j^T\w[\bfx]) \big] \right|
%             + \left| \mathbb{E}_{\w[\bfx]\in \text{ area II} }\big[ (\bfw^{*}_j-\w[\bfw]_j)^T\w[\bfx]\boldsymbol({\alpha}_j^T\w[\bfx]) \big] \right|\\
%             = & \frac{\pi - \theta}{2\pi}\de^2\|\w[\bfw]_j - \bfw_j^*\|_2 \|\boldsymbol{\alpha}_j\|_2 + \frac{\theta}{2\pi}\de^2\|\w[\bfw]_j - \bfw_j^*\|_2\|\boldsymbol{\alpha}_j\|_2\\
%             = & \frac{\de^2}{2}\|\w[\bfw]_j - \bfw_j^*\|_2 \|\boldsymbol{\alpha}_j\|_2.
%         \end{split}
%     \end{equation}
%     From \eqref{eqn:first_order_term1}, \eqref{eqn:first_order_term2} and \eqref{eqn:first_order_term3}, we have
%         \begin{equation}
%         \begin{split}
%             &\Big\|\frac{\partial \hat{f} }{ \partial \bfw_k } (\bfW) - \frac{\partial {f} }{ \partial \bfw_k } (\bfW)\Big\|_2\\
%             \le & \frac{\lambda}{K^2} \sum_{j=1}^K \Big\| \frac{1}{N}\sum_{n=1}^N\big( \phi(\bfw_j^T\bfx_n) - \phi(\bfw_j^{*T}\bfx_n)\big)\bfx_n - \mathbb{E}_{\bfx}\big( \phi(\bfw_j^T\bfx) -\phi(\bfw^{*T}_j\bfx) \big)\bfx 
%             \Big\|_2\\
%              & + \frac{1-\lambda}{K^2} \sum_{j=1}^K \Big\| \frac{1}{M}\sum_{m=1}^M\big( \phi(\bfw_j^T\w[\bfx]_m) - \phi(\w[\bfw]_j^T\w[\bfx]_m)\big)\w[\bfx]_m - \mathbb{E}_{\w[\bfx]}\big( \phi(\bfw_j^T\w[\bfx]) -\phi(\w[\bfw]^T_j\w[\bfx]) \big)\w[\bfx] 
%             \Big\|_2\\
%             & + \frac{1-\lambda}{K^2}\sum_{j=1}^K \mathbb{E}_{\w[\bfx]}\Big\| \big( \phi(\w[\bfw]_j^T\w[\bfx]) - \phi(\bfw^{*T}_j\w[\bfx]) \big)\w[\bfx]  \Big\|_2\\
%             \le &  \frac{\lambda}{K^{2}}\delta^2 \sqrt{\frac{d\log q}{N}}\cdot \sum_{j=1}^K\| \bfw_j -\bfw_j^* \|_2  + \frac{1- \lambda}{K^{2}}\cdot\de^2 \sqrt{\frac{d\log q}{M}} \cdot\sum_{j=1}^K\| \bfw_j -\bfw_j^* \|_2\\
%             &+\frac{(1- \lambda)\de^2}{2K^{2}} \cdot\sum_{j=1}^K\| \bfw_j -\bfw_j^* \|_2\\
%             \le &  \frac{\lambda}{K^{3/2}}\delta^2 \sqrt{\frac{d\log q}{N}}\cdot \| \bfW -\bfW^* \|_2  + \frac{1- \lambda}{K^{3/2}}\cdot\de^2 \sqrt{\frac{d\log q}{M}} \cdot\| \bfW -\w[\bfW] \|_2\\ 
%             &+\frac{(1- \lambda)\de^2}{2K^{3/2}} \cdot\| \w[\bfW] -\bfW^* \|_2\\
%             \le & \Big(\frac{\lambda}{K^{3/2}}\delta^2 \sqrt{\frac{d\log q}{N}} + \frac{1- \lambda}{K^{3/2}}\cdot\de^2 \sqrt{\frac{d\log q}{M}}\Big)\cdot \| \bfW -\bfW^* \|_2\\  &+ \frac{(1- \lambda)\de^2}{K^{3/2}}\cdot\Big( \sqrt{\frac{d\log q}{M}} +\frac{1}{2}\Big) \cdot\| \w[\bfW] -\bfW^* \|_2\\
%         \end{split}
%     \end{equation}
%     with probability at least $1-q^{-d}$.
    
%     In conclusion, let $\boldsymbol{\alpha}\in \mathbb{R}^{Kd}$ and  $\boldsymbol{\alpha}_{j}\in \mathbb{R}^d$ with $\boldsymbol{\alpha} =[\boldsymbol{\alpha}_{1}^T, \boldsymbol{\alpha}_{2}^T, \cdots, \boldsymbol{\alpha}_{K}^T]^T$, we have 
%     \begin{equation}
%         \begin{split}
%             \|\nabla f(\bfW) -\nabla \hat{f}(\bfW) \|_2
%             = & \Big| \boldsymbol{\alpha}^T \big( \nabla f(\bfW) -\nabla \hat{f}(\bfW) \big)  \Big|\\
%             \le & \sum_{k=1}^K\Big| \boldsymbol{\alpha}_k^T \big(\frac{\partial \hat{f} }{ \partial \bfw_k } (\bfW) - \frac{\partial {f} }{ \partial \bfw_k } (\bfW)\big) \Big|\\
%             \lesssim & \sum_{k=1}^K\Big\|\frac{\partial \hat{f} }{ \partial \bfw_k } (\bfW) - \frac{\partial {f} }{ \partial \bfw_k } (\bfW)\Big\|_2\cdot \|\boldsymbol{\alpha}_k\|_2\\
%             \lesssim &\Big(\frac{\lambda\delta^2}{K} \sqrt{\frac{d\log q}{N}} + \frac{(1- \lambda)\de^2}{K} \sqrt{\frac{d\log q}{M}}\Big)\cdot \| \bfW -\bfW^* \|_2 \\
%             &+ \frac{(1- \lambda)\de^2}{K}\Big( \sqrt{\frac{d\log q}{M}}+\frac{1}{2} \Big)\cdot\|\w[\bfW]-\bfW^* \|_2
%         \end{split}
%     \end{equation}
%     with probability at least $1-q^{-d}$.
% \end{proof}

% \subsection{Error bound of the second order derivative functions of population and empirical risk function at $\bfW$}

% \begin{lemma}\label{Lemma: second_order_distance}
%   Let $f$ and $\hat{f}$ be the functions defined in \eqref{eqn: population_risk_function} and $\eqref{eqn: empirical_risk_function}$, respectively. Suppose the pseudo label is generated through \eqref{eqn: psedu_label} with weights $\widetilde{\bfW}$. Then, we have
%   \begin{equation}
%       \|\nabla^2 f(\bfW) -\nabla^2 \hat{f}(\bfW) \|_2 \lesssim 
%       \lambda\delta^2\sqrt{\frac{d\log q}{N}}
%             +(1-\lambda)\de^2\sqrt{\frac{d\log q}{M}}
%     \end{equation}
%     with probability at least $1-q^{-d}$.
% \end{lemma}
% \begin{proof}[Proof of Lemma \ref{Lemma: second_order_distance}]
%     From \eqref{eqn: empirical_risk_function}, we know
%     \begin{equation}
%         \begin{split}
%             \frac{\nabla^2 \hat{f} }{ \partial\bfw_j\partial \bfw_k } 
%             =& \frac{\lambda}{NK^2}\sum_{n=1}^N \phi^{\prime}( \bfw_j^T\bfx_n ) \phi^{\prime}( \bfw_k^T\bfx_n )\bfx_n\bfx_n^T\\
%             &+ \frac{1-\lambda}{MK^2}\sum_{m=1}^M \phi^{\prime}( \bfw_j^T\w[\bfx]_m ) \phi^{\prime}( \bfw_k^T\w[\bfx]_m )\w[\bfx]_m\w[\bfx]_m^T.\\
%         \end{split}
%     \end{equation}
%     From \eqref{eqn: population_risk_function}, we know
%     \begin{equation}
%         \begin{split}
%             \frac{\nabla^2 {f} }{ \partial\bfw_j\partial \bfw_k } 
%             =& \frac{\lambda}{K^2} \mathbb{E}_{\bfx}\phi^{\prime}( \bfw_j^T\bfx ) \phi^{\prime}( \bfw_k^T\bfx )\bfx\bfx^T\\
%             &+ \frac{1-\lambda}{K^2} \mathbb{E}_{\w[\bfx]}\phi^{\prime}( \bfw_j^T\w[\bfx] ) \phi^{\prime}( \bfw_k^T\w[\bfx] )\w[\bfx] \w[\bfx]^T.\\
%         \end{split}
%     \end{equation}
%     Then, we have 
%     \begin{equation}
%         \begin{split}
%             &\frac{\nabla^2 \hat{f} }{ \partial\bfw_j\partial \bfw_k } -\frac{\nabla^2 {f} }{ \partial\bfw_j\partial \bfw_k }\\
%             =&\frac{\lambda}{K^2} \Big(\frac{1}{N}\sum_{n=1}^N\phi^{\prime}( \bfw_j^T\bfx_n ) \phi^{\prime}( \bfw_k^T\bfx_n )\bfx_n\bfx_n^T-\mathbb{E}_{\bfx}\phi^{\prime}( \bfw_j^T\bfx ) \phi^{\prime}( \bfw_k^T\bfx )\bfx\bfx^T \Big)\\
%             &+ \frac{1-\lambda}{K^2} 
%             \Big( \frac{1}{M}\sum_{m=1}^M \phi^{\prime}( \bfw_j^T\w[\bfx]_m ) \phi^{\prime}( \bfw_k^T\w[\bfx]_m )\w[\bfx]_m\w[\bfx]_m^T - \mathbb{E}_{\w[\bfx]}\phi^{\prime}( \bfw_j^T\w[\bfx]) \phi^{\prime}( \bfw_k^T\w[\bfx] )\w[\bfx]\w[\bfx]^T  \Big)
%         \end{split}
%     \end{equation}
%     For any vectors $\boldsymbol{\alpha}_j, \boldsymbol{\alpha}_k \in \mathbb{R}^d$ with $\|\boldsymbol{\alpha}_j\|_2, \|\boldsymbol{\alpha}_k\|_2 \le 1$, we define a random variable $$Z(j,k) = \phi^{\prime}( \bfw_j^T\bfx ) \phi^{\prime}( \bfw_k^T\bfx )\boldsymbol{\alpha}_j^T\bfx\boldsymbol{\alpha}_k^T\bfx.$$ 
%     Then, we have 
%     \begin{equation}\label{eqn: second_order_z}
%         \begin{split}
%             \big( \mathbb{E}|Z|^p \big)^{1/p} 
%             = & \Big( \mathbb{E} |\phi^{\prime}( \bfw_j^T\bfx ) \phi^{\prime}( \bfw_k^T\bfx )\boldsymbol{\alpha}_j^T\bfx\boldsymbol{\alpha}_k^T\bfx|^p \Big)^{1/p}\\
%             \le & \Big(\mathbb{E}  |(\boldsymbol{\alpha}_j^T\bfx)(\boldsymbol{\alpha}_k^T\bfx)|^p \Big)^{1/p}\\
%             \lesssim& \delta^2\cdot p.
%         \end{split}
%     \end{equation}
%  Similar to \eqref{eqn: second_order_z}, we have
%     \begin{equation}\label{eqn: second_order_z2}
%         \begin{split}
%             \Big( \mathbb{E} |\phi^{\prime}( \bfw_j^T\w[\bfx] ) \phi^{\prime}( \bfw_k^T\w[\bfx] )\boldsymbol{\alpha}_j^T\w[\bfx]\boldsymbol{\alpha}_k^T\w[\bfx]|^p \Big)^{1/p}
%             \lesssim& \de^2\cdot p.
%         \end{split}
%     \end{equation}
%     Hence, from \eqref{eqn: second_order_z} and \eqref{eqn: second_order_z2}, we know that both $Z(j,k)$ and $\phi^{\prime}( \bfw_j^T\w[\bfx] ) \phi^{\prime}( \bfw_k^T\w[\bfx] )\boldsymbol{\alpha}_j^T\w[\bfx]\boldsymbol{\alpha}_k^T\w[\bfx]$ belong to the sub-exponential distribution.
%         Let $Z_n(j,k) = \phi^{\prime}( \bfw_j^T\bfx_n ) \phi^{\prime}( \bfw_k^T\bfx_n )\boldsymbol{\alpha}_j^T\bfx_n\boldsymbol{\alpha}_k^T\bfx_n$ be the realization of $Z(j,k)$ for $n=1, 2, \cdots, N$.
%     Then, by Chernoff bound, we have 
%   \begin{equation}
%         \mathbb{P}\bigg\{ \Big| \frac{1}{N}\sum_{n=1}^N Z_n(j,k) -\mathbb{E}Z(j,k) \Big| < t \bigg\} \le 1- \frac{e^{-C\delta^4\cdot Ns^2}}{e^{Nst}}
%     \end{equation}
%     for some positive constant $C$ and any $s\in\mathbb{R}$. 
    
%     Let $t=\delta^2\sqrt{\frac{d\log q}{N}}$ and $s = \frac{2}{C\delta^2}\cdot t$ for some large constant $q>0$, we have
%     \begin{equation}
%         \begin{split}
%                 \Big| \frac{1}{N}\sum_{n=1}^N Z_n(j) -\mathbb{E}Z(j) \Big| \lesssim \delta^2 \cdot \sqrt{\frac{d\log q}{N}}
%         \end{split}
%     \end{equation}
%     with probability at least $1-q^{-d}$.
%     From Lemma \ref{Lemma: spectral_norm_on_net}, we have 
%     \begin{equation}\label{eqn:second_order_term1}
%     \begin{split}
%       &\Big\| \frac{1}{N}\sum_{n=1}^N \phi^{\prime}( \bfw_j^T\bfx_n ) \phi^{\prime}( \bfw_k^T\bfx_n )\bfx_n\bfx_n - \mathbb{E}_{\bfx}\phi^{\prime}( \bfw_j^T\bfx ) \phi^{\prime}( \bfw_k^T\bfx )\bfx\bfx\Big\|_2
%       \lesssim 2 \delta^2 \sqrt{ \frac{d\log q}{N} }
%     \end{split}
%     \end{equation}
%     with probability at least $1-(q/5)^{-d}$. Since $q$ is a large constant, we release the probability as $1-q^{-d}$ for simplification.
    
%     Similar to \eqref{eqn:second_order_term1}, we have 
%     \begin{equation}\label{eqn:second_order_term1}
%     \begin{split}
%       &\Big\| 
%       \frac{1}{M}\sum_{m=1}^M \phi^{\prime}( \bfw_j^T\w[\bfx]_m ) \phi^{\prime}( \bfw_k^T\w[\bfx]_m )\w[\bfx]_m\w[\bfx]_m - \mathbb{E}_{\bfx}\phi^{\prime}( \bfw_j^T\w[\bfx] ) \phi^{\prime}( \bfw_k^T\w[\bfx] )\w[\bfx]\w[\bfx]
%       \Big\|_2
%       \lesssim 2 \de^2 \sqrt{\frac{d\log q}{M}}
%     \end{split}
%     \end{equation}
%     with probability at least $1-q^{-d}$.
    
%     In conclusion, we have
%     \begin{equation}
%         \begin{split}
%             &\| \nabla^2 \hat{f}(\bfW) -\nabla^2 {f}(\bfW) \|_2\\
%             \le&\sum_{j=1}^K\sum_{k=1}^K\Big\| \frac{\nabla^2 \hat{f} }{ \partial\bfw_j\partial \bfw_k } -\frac{\nabla^2 {f} }{ \partial\bfw_j\partial \bfw_k } \Big\|_2  \\
%             =&\frac{\lambda}{K^2}\sum_{j=1}^K\sum_{k=1}^K \Big\| \frac{1}{N}\sum_{n=1}^N\phi^{\prime}( \bfw_j^T\bfx_n ) \phi^{\prime}( \bfw_k^T\bfx_n )\bfx_n\bfx_n^T-\mathbb{E}_{\bfx}\phi^{\prime}( \bfw_j^T\bfx ) \phi^{\prime}( \bfw_k^T\bfx )\bfx\bfx^T \Big\|_2\\
%             &+ \frac{1-\lambda}{K^2}\sum_{j=1}^K\sum_{k=1}^K 
%             \Big\| \frac{1}{M}\sum_{m=1}^M \phi^{\prime}( \bfw_j^T\w[\bfx]_m ) \phi^{\prime}( \bfw_k^T\w[\bfx]_m )\w[\bfx]_m\w[\bfx]_m^T - \mathbb{E}_{\w[\bfx]}\phi^{\prime}( \bfw_j^T\w[\bfx]) \phi^{\prime}( \bfw_k^T\w[\bfx] )\w[\bfx]\w[\bfx]^T  \Big\|_2\\
%             \lesssim & \lambda\delta^2\sqrt{\frac{d\log q}{N}}
%             +(1-\lambda)\de^2\sqrt{\frac{d\log q}{M}}.
%         \end{split}
%     \end{equation}
% \end{proof}

% \subsection{Error bound of the second order derivative function at points $\bfW$ and $\bfW^*$}

% \begin{proof}[Proof of Lemma \ref{Lemma:Second_order_distance}]
% 	From \eqref{eqn: population_risk_function}, we have 
% 	\begin{equation}
% 		\begin{split}
% 		\frac{\partial^2 f}{\partial {\bfw}_{j_1}\partial {\bfw}_{j_2}}({\bfW}^*)
% 		=&\frac{\lambda}{K^2} \mathbb{E}_{\bfx} \phi^{\prime} ({\bfw}_{j_1}^{*T}\bfx)\phi^{\prime} ({\bfw}_{j_2}^{*T}\bfx) \bfx \bfx^T
% 		+\frac{1-\lambda}{K^2} \mathbb{E}_{\w[\bfx]} \phi^{\prime} ({\bfw}_{j_1}^{*T}\w[\bfx])\phi^{\prime} ({\bfw}_{j_2}^{*T}\w[\bfx]) \w[\bfx] \w[\bfx]^T,
% 		\end{split}
% 	\end{equation}
% 	and 
% 	\begin{equation}
% 	\begin{split}
% 	\frac{\partial^2 f}{\partial {\bfw}_{j_1}\partial {\bfw}_{j_2}}({\bfW})
% 	=&\frac{\lambda}{K^2} \mathbb{E}_{\bfx} \phi^{\prime} ({\bfw}_{j_1}^T\bfx)\phi^{\prime} ({\bfw}_{j_2}^T\bfx) \bfx \bfx^T
% 	+\frac{1-\lambda}{K^2} \mathbb{E}_{\w[\bfx]} \phi^{\prime} ({\bfw}_{j_1}^T\w[\bfx])\phi^{\prime} ({\bfw}_{j_2}^T\w[\bfx]) \w[\bfx] \w[\bfx]^T.
% 	\end{split}
% 	\end{equation}
% 	Then, we have 
% 	\begin{equation}
% 	\begin{split}
% 	&\frac{\partial^2 f}{\partial {\bfw}_{j_1}\partial {\bfw}_{j_2}}(\bfW^*)
% 	-
% 	\frac{\partial^2 f}{\partial {\bfw}_{j_1}\partial {\bfw}_{j_2}}(\bfW)\\
% 	=&\frac{\lambda}{K^2} \mathbb{E}_{\bfx} \Big[
% 	\phi^{\prime} ({\bfw}_{j_1}^{*T}\bfx)\phi^{\prime} ({\bfw}_{j_2}^{*T}\bfx)
% 	-
% 	\phi^{\prime} ({\bfw}_{j_1}^T\bfx)\phi^{\prime} ({\bfw}_{j_2}^T\bfx)\Big] \bfx \bfx^T\\
% 	&+\frac{1-\lambda}{K^2} \mathbb{E}_{\w[\bfx]} \Big[
% 	\phi^{\prime} ({\bfw}_{j_1}^{*T}\w[\bfx])\phi^{\prime} ({\bfw}_{j_2}^{*T}\w[\bfx])
% 	-
% 	\phi^{\prime} ({\bfw}_{j_1}^T\w[\bfx])\phi^{\prime} ({\bfw}_{j_2}^T\w[\bfx])\Big] \w[\bfx] \w[\bfx]^T\\
% 	=&\frac{\lambda}{K^2}\mathbb{E}_{\bfx} 
% 	\Big[ \phi^{\prime} ({\bfw}_{j_1}^{*T}\bfx)
% 	\big(\phi^{\prime} ({\bfw}_{j_2}^{*T}\bfx)
% 	- \phi^{\prime} ({\bfw}_{j_2}^T\bfx)
% 	\big)
% 	+
% 	\phi^{\prime} ({\bfw}_{j_2}^T\bfx)
% 	\big(\phi^{\prime} ({\bfw}_{j_1}^{*T}\bfx)
% 	- \phi^{\prime} ({\bfw}_{j_1}^T\bfx)
% 	\big)
% 	\Big]\bfx \bfx^T\\
% 	&+\frac{1-\lambda}{K^2}\mathbb{E}_{\w[\bfx]} 
% 	\Big[ \phi^{\prime} ({\bfw}_{j_1}^{*T}\w[\bfx])
% 	\big(\phi^{\prime} ({\bfw}_{j_2}^{*T}\w[\bfx])
% 	- \phi^{\prime} ({\bfw}_{j_2}^T\w[\bfx])
% 	\big)
% 	+
% 	\phi^{\prime} ({\bfw}_{j_2}^T\w[\bfx])
% 	\big(\phi^{\prime} ({\bfw}_{j_1}^{*T}\w[\bfx])
% 	- \phi^{\prime} ({\bfw}_{j_1}^T\w[\bfx])
% 	\big)
% 	\Big]\w[\bfx] \w[\bfx]^T\\
% 	=&\frac{\lambda}{K^2}\Big[
% 	\mathbb{E}_{\bfx} 
% 	\phi^{\prime} ({\bfw}_{j_1}^{*T}\bfx)
% 	\big(\phi^{\prime} ({\bfw}_{j_2}^{*T}\bfx)
% 	- \phi^{\prime} ({\bfw}_{j_2}^T\bfx)
% 	\big)\bfx \bfx^T
% 	+
% 	\mathbb{E}_{\bfx}
% 	\phi^{\prime} ({\bfw}_{j_2}^T\bfx)
% 	\big(\phi^{\prime} ({\bfw}_{j_1}^{*T}\bfx)
% 	- \phi^{\prime} ({\bfw}_{j_1}^T\bfx)
% 	\big)\bfx \bfx^T
% 	\Big]\\
% 	&+\frac{1-\lambda}{K^2}\Big[
% 	\mathbb{E}_{\w[\bfx]} 
% 	\phi^{\prime} ({\bfw}_{j_1}^{*T}\w[\bfx])
% 	\big(\phi^{\prime} ({\bfw}_{j_2}^{*T}\w[\bfx])
% 	- \phi^{\prime} ({\bfw}_{j_2}^T\w[\bfx])
% 	\big)\w[\bfx] \w[\bfx]^T
% 	+
% 	\mathbb{E}_{\w[\bfx]}
% 	\phi^{\prime} ({\bfw}_{j_2}^T\w[\bfx])
% 	\big(\phi^{\prime} ({\bfw}_{j_1}^{*T}\w[\bfx])
% 	- \phi^{\prime} ({\bfw}_{j_1}^T\w[\bfx])
% 	\big)\w[\bfx] \w[\bfx]^T
% 	\Big]\\
% 	:=& \frac{\lambda}{K^2} (\bfP_1 + \bfP_2) + \frac{1-\lambda}{K^2}(\bfP_3+\bfP_4).
% 	\end{split}
% 	\end{equation}
% 	For any $\bfa\in\mathbb{R}^{d}$, we have 
% 	\begin{equation}
% 	\begin{split}
% 	\bfa^T\bfP_1 \bfa 
% 	=&\mathbb{E}_{\bfx} 
% 	\phi^{\prime} ({\bfw}_{j_1}^{*T}\bfx)
% 	\big(\phi^{\prime} ({\bfw}_{j_2}^{*T}\bfx)
% 	- \phi^{\prime} ({\bfw}_{j_2}^T\bfx)
% 	\big) 
% 	(\bfa^T\bfx)^2\\	
% % 	\le&\mathbb{E}_{\bfx} 
% % 	\phi^{\prime} (\bfw^{*T}_{j_2}\bfx)
% % 	\big(\phi^{\prime} (\bfw_{j_2}^{*T}\bfx)
% % 	- \phi^{\prime} (\bfw_{j_2}^T\bfx)
% % 	\big) 
% % 	\cdot
% % 	(\bfa^T\bfx)^2,	
% 	\end{split}
% 	\end{equation}
% 	 where $\bfa\in\mathbb{R}^d$.
% 	 Let $I =
% \phi^{\prime} (\bfw^{[p]T}_{j_1}\bfx)
% \big(\phi^{\prime} (\bfw_{j_2}^{*T}\bfx)
% - \phi^{\prime} (\bfw_{j_2}^T\bfx)
% \big) 
% \cdot
% (\bfa^T\bfx)^2$. 
% 	 It is easy to verify there exists a basis such that $\mathcal{B}=\{\bfa, \bfb, \bfc, \bfa_4^{\perp}, \cdots, \bfa_d^{\perp}\}$ with $\{\bfa, \bfb, \bfc \}$ spans a subspace that contains $\bfa, \bfw_{j_2}$ and $\bfw_{j_2}^*$. Then, for any $\bfx$, we have a unique $\bfz=\begin{bmatrix}
% 		z_1,&z_2,&\cdots, & z_d
% 		\end{bmatrix}^T$ such that 
% 		\begin{equation*}
% 		\bfx = z_1\bfa + z_2 \bfb +z_3\bfc + \cdots + z_d\bfa^{\perp}_d.
% 		\end{equation*}
% 		Also, since $\bfx \sim \mathcal{N}(\boldsymbol{0}, \delta^2\bfI_d)$, we have $\bfz \sim \mathcal{N}(\boldsymbol{0}, \delta^2\|\bfa\|_2^2\bfI_d)$. Then, we have 
% 		\begin{equation*}
% 		\begin{split}
% 		I 
% 		=& \mathbb{E}_{z_1, z_2, z_3}|\phi^{\prime}\big(\bfw_{j_2}^T{\bfx}\big)-\phi^{\prime}\big({\bfw_{j_2}^{*T}}{\bfx}\big)|\cdot 
% 		|\bfa^T{\bfx}|^2\\
% 		=&\int|\phi^{\prime}\big(\bfw_{j_2}^T{\bfx}\big)-\phi^{\prime}\big({\bfw_{j_2}^{*T}}{\bfx}\big)|\cdot 
% 		|\bfa^T{\bfx}|^2 \cdot f_Z(z_1, z_2,z_3)dz_1 dz_2 dz_3,
% 		\end{split}
% 		\end{equation*}
% 		where ${\bfx}= z_1\bfa + z_2\bfb + z_3\bfc$ and $f_Z(z_1, z_2,z_3)$ is probability density function of $(z_1, z_2, z_3)$. Next, we consider spherical coordinates with $z_1= Rcos\phi_1 , z_2 = Rsin\phi_1sin\phi_2, z_3=z_2 = Rsin\phi_1cos\phi_2$. Hence,
% 		\begin{equation}
% 		\begin{split}
% 		I
% 		=&\int|\phi^{\prime}\big(\bfw_{j_2}^T{\bfx}\big)-\phi^{\prime}\big(\bfw_{j_2}^{*T}{\bfx}\big)|\cdot |R\cos\phi_1|^2
% 		\cdot f_Z(R, \phi_1, \phi_2)R^2\sin \phi_1 dR d\phi_1 d \phi_2.
% 		\end{split}
% 		\end{equation}
% 		It is easy to verify that $\phi^{\prime}\big(\bfw_{j_2}^T{\bfx}\big)$ only depends on the direction of ${\bfx}$ and 
% 		\begin{equation*}
% 		f_Z(R, \phi_1, \phi_2) = \frac{1}{(2\pi\delta^2)^{\frac{3}{2}}}e^{\frac{x_1^2+x_2^2+x_3^2}{2\delta^2}}=\frac{1}{(2\pi\delta^2)^{\frac{3}{2}}}e^{\frac{R^2}{2\delta^2}}
% 		\end{equation*}
% 		only depends on $R$. Then, we have 
% 		\begin{equation}\label{eqn: ean111}
% 		\begin{split}
% 		&I(i_2, j_2)\\
% 		=&\int|\phi^{\prime}\big(\bfw_{j_2}^T({\bfx}/R)\big)-\phi^{\prime}\big({\bfw_{j_2}^{*T}}({\bfx}/R)\big)|
% 		\cdot |R\cos\phi_1|^2
% 		\cdot f_Z(R)R^2\sin \phi_1 dRd\phi_1d\phi_2\\
% 		=& \int_0^{\infty} R^4f_z(R)dR\int_{0}^{\pi}\int_{0}^{2\pi}|\cos \phi_1|^2\cdot \sin\phi_1
% 		\cdot|\phi^{\prime}\big(\bfw_{j_2}^T({\bfx}/R)\big)-\phi^{\prime}\big({\bfw_{j_2}^{*T}}({\bfx}/R)\big)|d\phi_1d\phi_2\\
% 		\le& \sqrt{\frac{8}{\pi}} \int_0^{\infty} R^2f_z(R)dR\int_{0}^{\pi}\int_{0}^{2\pi} \sin\phi_1
% 		\cdot|\phi^{\prime}\big(\bfw_{j_2}^T({\bfx}/R)\big)-\phi^{\prime}\big({\bfw_{j_2}^{*T}}({\bfx}/R)\big)|d\phi_1d\phi_2\\
% 		=&\sqrt{\frac{8}{\pi}}\delta^2\|\bfa\|_2^2\cdot\mathbb{E}_{z_1, z_2, z_3}\big|\phi^{\prime}\big(\bfw_{j_2}^T{\bfx}\big)-\phi^{\prime}\big({\bfw_{j_2}^{*T}}{\bfx}\big)|\\
% 		\le&2\delta^2\|\bfa\|_2^2\cdot\mathbb{E}_{\bfx}\big|\phi^{\prime}\big(\bfw_{j_2}^T{\bfx}\big)-\phi^{\prime}\big({\bfw_{j_2}^{*T}}{\bfx}\big)|.
% 		\end{split}
% 		\end{equation}


% 	Define a set $\mathcal{A}_1=\{\bfx| ({\bfw_{j_2}^{*T}}\bfx)(\bfw_{j_2}^T\bfx)<0 \}$. If $\bfx\in\mathcal{A}_1$, then ${\bfw_{j_2}^{*T}}\bfx$ and $\bfw_{j_2}^T\bfx$ have different signs, which means the value of $\phi^{\prime}(\bfw_{j_2}^T\bfx)$ and $\phi^{\prime}({\bfw_{j_2}^{*T}}\bfx)$ are different. This is equivalent to say that 
% 	\begin{equation}\label{eqn:I_1_sub1}
% 	|\phi^{\prime}(\bfw_{j_2}^T\bfx)-\phi^{\prime}({\bfw_{j_2}^{*T}}\bfx)|=
% 	\begin{cases}
% 	&1, \text{ if $\bfx\in\mathcal{A}_1$}\\
% 	&0, \text{ if $\bfx\in\mathcal{A}_1^c$}
% 	\end{cases}.
% 	\end{equation}
% 	Moreover, if $\bfx\in\mathcal{A}_1$, then we have 
% 	\begin{equation}
% 	\begin{split}
% 	|{\bfw_{j_2}^{*T}}\bfx|
% 	\le&|{\bfw_{j_2}^{*T}}\bfx-\bfw_{j_2}^T\bfx|
% 	\le\|{\bfw_{j_2}^*}-{\bfw_{j_2}}\|_2\cdot\|\bfx\|_2.
% 	\end{split}
% 	\end{equation}
% 	Let us define a set $\mathcal{A}_2$ such that
% 	\begin{equation}
% 	\begin{split}
% 	\mathcal{A}_2
% 	=&\Big\{\bfx\Big|\frac{|{\bfw_{j_2}^{*T}}\bfx|}{\|\bfw_{j_2}^*\|_2\|\bfx\|_2}\le\frac{\|{\bfw_{j_2}^*}-{\bfw_{j_2}}\|_2}{\|\bfw_{j_2}^*\|_2}   \Big\}
% 	=\Big\{\theta_{\bfx,\bfw_{j_2}^*}\Big||\cos\theta_{\bfx,\bfw_{j_2}^*}|\le\frac{\|{\bfw_{j_2}^*}-{\bfw_{j_2}}\|_2}{\|\bfw_{j_2}^*\|_2}   \Big\}.
% 	\end{split}
% 	\end{equation}	
% 	Hence, we have that
% 	\begin{equation}\label{eqn:I_1_sub2}
% 	\begin{split}
% 	\mathbb{E}_{\bfx}
% 	|\phi^{\prime}(\bfw_{j_2}^T\bfx)-\phi^{\prime}({\bfw_{j_2}^{*T}}\bfx)|^2
% 	=& \mathbb{E}_{\bfx}
% 	|\phi^{\prime}(\bfw_{j_2}^T\bfx)-\phi^{\prime}({\bfw_{j_2}^{*T}}\bfx)|\\
% 	=& \text{Prob}(\bfx\in\mathcal{A}_1)\\
% 	\le& \text{Prob}(\bfx\in\mathcal{A}_2).
% 	\end{split}
% 	\end{equation}
% 	Since $\bfx\sim \mathcal{N}({\bf0},\delta^2\|\bfa\|_2^2 \bfI)$, $\theta_{\bfx,\bfw_{j_2}^*}$ belongs to the uniform distribution on $[-\pi, \pi]$, we have
% 	\begin{equation}\label{eqn:I_1_sub3}
% 	\begin{split}
% 	\text{Prob}(\bfx\in\mathcal{A}_2)
% 	=\frac{\pi- \arccos\frac{\|{\bfw_{j_2}^*}-{\bfw_{j_2}}\|_2}{\|\bfw_{j_2}^*\|_2} }{\pi}
% 	\le&\frac{1}{\pi}\tan(\pi- \arccos\frac{\|{\bfw_{j_2}^*}-{\bfw_{j_2}}\|_2}{\|\bfw_{j_2}^*\|_2})\\
% 	=&\frac{1}{\pi}\cot(\arccos\frac{\|{\bfw_{j_2}^*}-{\bfw_{j_2}}\|_2}{\|\bfw_{j_2}^*\|_2})\\
% 	\le&\frac{2}{\pi}\frac{\|{\bfw_{j_2}^*}-{\bfw_{j_2}}\|_2}{\|\bfw_{j_2}^*\|_2}.
% 	\end{split}
% 	\end{equation}

% 	Hence,  \eqref{eqn: ean111} and \eqref{eqn:I_1_sub3} suggest that
% 	\begin{equation}\label{eqn:I_1_bound}
% 	I\le\frac{6\delta^2}{\pi}\frac{\|\bfw_{j_2} -\bfw_{j_2}^*\|_2}{\sigma_K} \cdot\|\bfa\|_2^2.
% 	\end{equation}
% 	The same bound that shown in \eqref{eqn:I_1_bound} holds for $\bfP_2$ as well.  
	
% 	$\bfP_3$ and $\bfP_4$ satisfy \eqref{eqn:I_1_bound} except for changing $\delta^2$ to $\de^2$.
	
% 	Therefore, we have 
% 	\begin{equation}
% 	    \begin{split}
% 	    &\| \nabla^2f(\bfW^*) - \nabla^2f(\bfW)\|_2\\
% 	    =&\max_{\|\boldsymbol{\alpha}\|_2\le 1} \Big|\boldsymbol{\alpha}^T(\nabla^2f(\bfW^*) - \nabla^2f(\bfW))\boldsymbol{\alpha}\Big|\\
% 	    \le&\sum_{j_1=1}^K\sum_{j_2=1}^K\Bigg|\boldsymbol{\alpha}_{j_1}^T\bigg(\frac{\partial^2 f}{\partial {\bfw}_{j_1}\partial {\bfw}_{j_2}}(\bfW^*)
% 	    -
% 	    \frac{\partial^2 f}{\partial {\bfw}_{j_1}\partial {\bfw}_{j_2}}(\bfW)\bigg)\boldsymbol{\alpha}_{j_2}\Bigg|\\
% 	    \le &\frac{1}{K^2}\sum_{j_1=1}^K\sum_{j_2=1}^K\Big(\lambda \|\bfI_1+\bfI_2\|_2 + (1-\lambda)\|\bfI_3+\bfI_4\|_2\Big)\|\boldsymbol{\alpha}_{j_1}\|_2 \|\boldsymbol{\alpha}_{j_2}\|_2\\
% 	    \le & \frac{1}{K^2}\sum_{j_1=1}^K\sum_{j_2=1}^K4(\lambda\delta^2+(1-\lambda)\de^2)\frac{\|\bfw_{j_2}^*-\bfw_{j_2}\|_2}{\sigma_K}\|\boldsymbol{\alpha}_{j_1}\|_2 \|\boldsymbol{\alpha}_{j_2}\|_2\\
% 	    \le & \frac{4}{K}\big(\lambda\delta^2+(1-\lambda)\de^2\big)\cdot\frac{\|\bfW^*-\bfW\|_2}{\sigma_K},
% 	    \end{split}
% 	\end{equation}
% 	where $\boldsymbol{\alpha}\in \mathbb{R}^{Kd}$ and  $\boldsymbol{\alpha}_{j}\in \mathbb{R}^d$ with $\boldsymbol{\alpha} =[\boldsymbol{\alpha}_{1}^T, \boldsymbol{\alpha}_{2}^T, \cdots, \boldsymbol{\alpha}_{K}^T]^T$.
% \end{proof}





==> Self-training (6)/Theoretical_results.tex <==
\section{Theoretical results}\label{sec: theoretical}
%The major theorems are presented in this section. Theorem \ref{Thm: p_convergence} provides the convergence analysis in low labeled regime, while the results in moderate labeled data regime are  summarized in Theorem \ref{Thm: sufficient_number}. 
%To begin with,

% \SL{[Why start from the following definitions. It seems that you did not call this definition in comparision with supervised learning.]}


\paragraph{{Beyond supervised learning: Challenge of self-training.}}
The existing theoretical works such as  \citep{ZSJB17,ZWLC20_1,ZWLC20_2,ZWLC20_3} verify that for one-hidden-layer neural networks, if only labeled data are available, and $\bfx$ are drawn from the standard Gaussian distribution, then supervised learning by minimizing \eqref{eqn: empirical_risk_function} with $\lambda=1$ %using labeled data from standard Gaussian only (i.e., $M=0$ and $\delta=1$)
 can return a model with ground-truth weights $\bfW^*$ (up to column permutation), as long as  the number of labeled data $N$ is at least  \Revise{$N^*$, which  depends on $\kappa, K$ and $d$}. In contrast, this paper focuses %on analyzing the performance of iterative self-training algorithm 
on the \textbf{low labeled-data regime} when $N$ is less than $N^*$. %  the existing sample complexity requirement for supervised learning, and 
Specifically,
\begin{wrapfigure}{r}{0.47\linewidth}
    \centering
    \vspace{-1mm}
    \includegraphics[width=0.80
    \linewidth]{Figure/AGD.pdf}
    \vspace{-1mm}
     \caption{Adding unlabeled data in the empirical risk function drives its local minimum closer to $\bfW^*$, which minimizes the generalization function.}%%Landscape of the generalization function, and the objective functions with/without unlabeled data.}
    \label{fig: landscape_1}
\end{wrapfigure}
\begin{equation}\label{eqn: definition_N*}
  N^* /4< N \leq N^*. %   = c(\kappa)\mu^{*2}K^3d\log q.
\end{equation}%
 
Intuitively, if $N<N^*$, the landscape of the empirical risk of the labeled data becomes highly nonconvex, even in a neighborhood   of $\bfW^*$, thus, the existing analyses for supervised learning do not hold in this region.  With additional unlabeled data, the landscape of the weighted empirical risk becomes smoother near  $\bfW^*$. Moreover, as $M$ increases, and starting from a nearby initialization, the returned model $\W[L]$ by iterative self-training  can converge to a local minimum that is closer to $\bfW^*$ (see  illustration in Figure \ref{fig: landscape_1}). 

%Inspired by the intuition,
%For the formal analysis, 
%we quantify the distance of the learned model to $\bfW^*$ analytically as  a function of  the numbers of labeled and unlabeled samples (see the illustration in Figure \ref{fig: Thm2_region}).

Compared with supervised learning, the formal analyses of self-training need to handle new technical challenges from two aspects. First, the existing analyses of supervised learning exploit the fact that   the GF and the empirical risk have the same minimizer, i.e., $\bfW^*$. This property does not hold for self-training as $\bfW^*$ no longer minimizes the weighted empirical risk in (\ref{eqn: empirical_risk_function}). Second, the iterative manner of self-training complicates the analyses. Specifically, the empirical risk   in each iteration is different and depends on the model trained in the previous iteration through the pseudo labels.  %  and the  for the formal analyses include (1) the iterative manner of self-training 
%and 
%(2) the requirement of new tools in analyzing the minimization of the weighted empirical risk in (1). Specifically,  % utilizing generalization function to analysis the objective function no longer hold because of insufficient labeled data amount and additional unlabeled dataset.  

{In what follows, we   provide theoretical insights and the formal theorems. 
Some important quantities $\hat{\lambda}$ and $\mu$  are defined below 
\vspace{-1mm}
\begin{equation}\label{eqn: definition_lambda}
    \hat{\lambda} : =\frac{\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2},
    \text{\quad and \quad}
    \mu
    = \mu( \delta, \de) 
    := \sqrt{\frac{\lambda\delta^2+\w[\lambda]\de^2}{\lambda\rho(\delta)+\w[\lambda]\rho(\de)}},
    \vspace{-1mm}
\end{equation}
 where $\rho$ is a positive function defined in \eqref{eqn: rho}.
 %, similar to  %defined in 
 %\citep{ZSJB17}. 
% One can easily check that 
 $\hat{\lambda}$ is an increasing function of $\lambda$. Also,
 from  Lemma \ref{lemma: rho_order} (in Appendix),   $\rho(\delta)$ is in the order of $\delta^2$ when $\delta\leq 1$   for ReLU activation functions. Thus,   $\mu$ is a fixed constant, denoted by $\mu^*$, for all $\delta, \de \leq 1$. %, which is the focus here. 
 When $\delta$ and $\de$ are large,   $\mu$ increases as they increase.} \Revise{The formal definition of $N^*$ in \eqref{eqn: definition_N*} is $c(\kappa)\mu^{*2}K^3d\log q$, where $c(\kappa)$ is some polynomial function of $\kappa$ and can be viewed as constant.}%Here we consider $\delta$ and $\de$ are small, and thus $\mu$ is a fixed  constant. Additionally, 
% We use  

% The major challenge is to seek an analyzable function along with characterized bound with respect to both the objective function and generalization function.


\subsection{Informal key theoretical findings}

% \SL{[I feel that 3.1 should cover both 3.2 and 3.3. Then, it will be better to point out which finding belongs to which formal theory sub-section.]}
% We first summarize the significance of our results before formally presenting Theorems \ref{Thm: p_convergence} and \ref{Thm: sufficient_number}. 
 \begin{wrapfigure}{r}{0.49\textwidth}
    \centering
    \vspace{-10mm}
    \includegraphics[width=1.00\linewidth]{Figure/self_training.pdf}
    \vspace{-2mm}
    \caption{Illustration of the (1) ground truth $\bfW^*$, (2) iterations $\{ \W[\ell] \}_{\ell=0}^L$, (3) convergent point $\W[L]$, and (4) $\WL = \hat{\lambda}\bfW^*+(1-\hat{\lambda})\W[0]$.}
    \label{fig: Thm2_region}
    \vspace{-5mm}
\end{wrapfigure}
To the best of our knowledge,   Theorems \ref{Thm: p_convergence} and \ref{Thm: sufficient_number} provide the first  theoretical characterization of iterative self-training on nonlinear neural networks. Before formally presenting them, we summarize the highlights as follows. % with a quantitative analysis of the generalization performance of the learned model as a function of the number of labeled and unlabeled samples. In particular, the significance of our results is summarized below before formally presenting Theorems \ref{Thm: p_convergence} and \ref{Thm: sufficient_number}.

% \iffalse
% In this part, we explore the behaviors of the iterations returned by Algorithm \ref{Algorithm: Alg1} in low labeled-data regime ($N < N^*$), from the theoretical aspects. \tcr{From \eqref{eqn: definition_lambda}, one can easily check that $\hat{\lambda}$ is an increasing function of $\lambda$, and $\hat{\lambda}$ is exactly $\lambda$ when $\delta = \w[\delta]$. In low labeled-data regime as $N$ is small, the landscape of the loss function in \eqref{eqn: loss_1} may contain significantly many waves near the ground truth, while the landscape of \eqref{eqn: loss_2} has a considerable large size of flat and smooth convex region with a sufficiently large number of unlabeled data. In other words, the value of $\hat{\lambda}$ and $M$ can be used to adjust the landscape of the objective function in \eqref{eqn: empirical_risk_function_2}.} 
% \fi
% % Theorem 1 characterizes the performance of Algorithm \ref{Algorithm: Alg1} after the first loop, as shown in \eqref{eqn: thm1_convergence}, provide that conditions \eqref{eqn: thm1_condition1} and \eqref{eqn: p_main_sample_M} hold. Built upon the results in Theorem \ref{Thm: p_weak}, with further assumptions in \eqref{eqn: thm2_condition1} and \eqref{eqn: p}, we are able to provide theoretical analysis of the iterations returned by Algorithm \ref{Algorithm: Alg1} shown in \eqref{eqn: p_convergence} after any loops. Moreover, \eqref{eqn: p_convergence_*} in Corollary \ref{corollary: W*} suggests that the model returned by Algorithm \ref{Algorithm: Alg1} under the constraints in Theorem \ref{Thm: p_convergence} is better than the initial model in terms of the distance to the ground truth weights. 
% %In particular, the significance of these results can be interpreted from the following aspects:



% \begin{figure}[h]
%     \centering
%     \begin{minipage}{0.49\linewidth}
%     \centering
%   	\includegraphics[width=1.0\linewidth]{Figure/C_1.pdf}
%      \caption{Convergence of the iterations $\{\W[\ell] \}_{\ell=0}^T$.}
%     \label{fig: convergence_illustration}
%     \end{minipage}
%     ~
%     \begin{minipage}{0.45\linewidth}
%     \centering
%         \includegraphics[width=0.88\linewidth]{Figure/C_2.pdf}
%     \caption{Illustration of initial weights $\W[0]$, ground truth $\bfW^*$, convergent point $\W[L]$ and $\WL = \hat{\lambda}\bfW^*+(1-\hat{\lambda})\W[0]$.}
%     \label{fig: Thm2_region}
%     \end{minipage}
%     \vspace{-1mm}
% \end{figure}

 
\textbf{1. Linear convergence of the learned models.} % Convergence analysis of iterative self-training algorithm.} As indicated in Figure \ref{fig: convergence_illustration}, 
The learned models %the iterations $\{\bfW^{\ell} \}_{\ell=0}^L$ generated in the iterative self-training algorithm 
%in $L$ iterations 
converge linearly to a model close to $\bfW^*$. %(Figure \ref{fig: Thm2_region}). 
Thus, the iterative approach returns a model with better generalization than that by the single-shot method. Moreover,    the convergence rate is a constant term plus a term in the order of $1/\sqrt{M}$ (see $\Delta_1$ in Figure \ref{fig: Thm2_region}), indicating a faster convergence with more unlabeled data. %. Compared with single shot approach, iterative manner improves the test accuracy with an exponential decay at the cost of a linear growth in the training time.}

%\textbf{2. Characterization of learned model via iterative self-training algorithm in low labeled data regime.} 
\textbf{2. Returning a model with guaranteed generalization   in the low labeled-data regime.}  Even when the number of labeled data is much less than the required sample complexity to obtain $\bfW^*$ in supervised learning, we prove that with the help of unlabeled data, 
%With limited number of labeled data such that (\ref{eqn: definition_N*}) holds, % such that $N$ satisfies 
% \begin{equation}
%     {N^*}/{K^2} \le N  \le N^*,
% \end{equation} 
 %the learned model $\W[L]$ lies in
 the iterative self-training can return a model in 
 the neighborhood 
 of $\WL$, where $\WL$ is in the line segment of  $\W[0]$ ($\hat{\lambda}=0$) and ground truth $\bfW^*$ ($\hat{\lambda}=1$). % and  $\WL$ moves closer to  $\bfW^*$ as $\hat{\lambda}$  increases. 
% See the illustration of $\mathcal{E}_0$ in Figure \ref{fig: Thm2_region} for details.
Moreover, %Additionally, 
$\hat{\lambda}$ is upper bounded by $\sqrt{N/N^*}$. Thus $\W[L]$ moves closer to $\bfW^*$ as $N$ increases ($\mathcal{E}_0$ in Figure \ref{fig: Thm2_region}), indicating a better generalization performance with more labeled data. %the number of labeled data increases. }

 % (Theorem \ref{Thm: p_convergence}), and the relationships of $\w[L]$, $\WL$ and $\bfW^*$ are illustrated in Figure \ref{fig: Thm2_region} as well. $\WL$ is a convex combination of the initial weights $\W[0]$ and ground truth $\bfW^*$, and the distance between $\WL$ and the ground truth $\bfW^*$ becomes smaller with larger $\hat{\lambda}$. In addition, the value of $\hat{\lambda}$ is upper bounded by the number of labeled data $N$, therefore the convergent point moves closer to $\bfW^*$ if we increase the number of labeled data. Also, 


%\textbf{2. The learned model is improved over the initial model.} Starting from some initial teacher model, the learned model with sufficiently many unlabeled data are able to find a model with smaller distance to the ground truth, which suggests a smaller generalization error bound. 
%We emphasize some initial teacher model is because there exists some model that cannot be further improved given limited number of labeled data. For instance, the initial model is close enough to the ground truth such that it can match all the labeled data in $\mathcal{D}$ as well, then we cannot improve the initial model unless we are accessible to extra labeled data. 


%\textbf{3. Unlabeled data improves the generalization performance and convergence rate.}
\textbf{3. Guaranteed generalization improvement by unlabeled data.} %As illustrated by $\mathcal{E}_1$ in Figure \ref{fig: Thm2_region},
The distance between $\W[L]$ and $\WL$ ($\mathcal{E}_1$ in Figure \ref{fig: Thm2_region})
%$\|\W[L]-\WL\|_F$ 
scales in the order of $1/\sqrt{M}$. With a larger number of unlabeled data $M$, $\W[L]$ moves closer to $\WL$ and thus $\bfW^*$,  indicating an improved generalization performance %on data in $\mathcal{D}$ 
(Theorem \ref{Thm: p_convergence}).
When $N$ is close to $N^*$ but still smaller as defined in (\ref{eqn: main_sample}), %namely, $N^*> N>(1-\mu^{-1}K^{-1/2})^2N^*$, %but still smaller than $N^*$, 
 both $\W[L]$ and $\WL$ converge to $\bfW^*$, and thus the learned model achieves zero generalization error (Theorem \ref{Thm: sufficient_number}).  %Moreover, from Figure \ref{fig: Thm2_region},  the convergence rate is proportional to $1/\sqrt{M}$. Thus, the algorithm converges faster as $M$ increases.





\iffalse
As shown in Figure \ref{fig: Thm2_region}, the distance between the learned model $\W[L]$ and the ground truth $\bfW^*$ are upper bounded by $\mathcal{E}_2$ $(\| \W[L]-\WL \|_F)$ and  $\mathcal{E}_3$  $ (\|\WL - \bfW^* \|_F)$. In particular, $\mathcal{E}_3$ is a linear function of $1/\sqrt{M}$. Therefore, With larger number of unlabeled data $M$, the value of $\|\W[L]-\WL\|_F$ become smaller, and thus the upper bound of $\|\W[L] -\bfW^* \|_F$ decreases, which suggests an improved generalization error. Notably, with enough unlabeled data,
the learned model can still converge to the ground truth even if the  $N$ is slightly smaller than $N^*$ as $N=(1-\mu^{-1}K^{-1/2})^2 N^*$ (Theorem \ref{Thm: sufficient_number}).
However, except the cases in Theorem \ref{Thm: sufficient_number},  the distance between $\W[L]$ and $\WL$ cannot be arbitrarily small in general even with infinite number of unlabeled data, which is unlike increasing labeled data. 
Moreover, the convergence rate of the iterations $\{\W[\ell] \}_{\ell=0}^L$ is a linear function of ${1}/{\sqrt{M}}$ as well. If the number of unlabeled data is increases, the convergence rate becomes smaller (faster).
\fi
\iffalse
\textbf{1. Sample complexity analysis of labeled and unlabeled data.} 
% From \eqref{eqn: p_main_sample_M}, we can see that the number of unlabeled data needs to be at least in the order of $\mu^2(1-\hat{\lambda})^2K^3d\log q$ to provide analyzable performance. Specifically, The required number of samples is a linear function of $d$, which is the dimension of the input data dimension. In addition, \eqref{eqn: thm1_condition1} suggests that the largest possible value of $\hat{\lambda}$ depends on $\sqrt{N}$ linearly. With less labeled data (smaller $N$), we thus requires more number of unlabeled data to guarantee the analyzable performance (larger $M$).  However, to guarantee the learned model is improved over the initial model as shown in \eqref{eqn: p_convergence_*}, the number of labeled data cannot be arbitrarily small but satisfies the constraints shown in \eqref{eqn: thm2_condition1}. 
The number of unlabeled data needs to be at least in the order of $\mu^2(1-\hat{\lambda})^2K^3d\log q$ to provide analyzable performance. Specifically, The required number of unlabeled samples is a linear function of $d$, which is the dimension of the input data dimension. In addition, the largest possible value of $\hat{\lambda}$ depends on $\sqrt{N}$ linearly. With less labeled data (smaller $N$), we thus requires more number of unlabeled data to guarantee the analyzable performance (larger $M$).  However, to guarantee the learned model is improved over the initial model, the number of labeled data cannot be arbitrarily small but needs to be larger than $\mu^2Kd\log q$.



\textbf{2. Region of initial weights for improved learned model.} 
% From Figure \ref{fig: Thm2_region} (a), we can see that the convergent point is better than the initial point in terms of the distance to the ground truth if the initial weights lie in the region between the two vertical dash lines in the same color. 
%The constraint in \eqref{eqn: p}, along with the definition of $p$ in \eqref{eqn: definition_p}, implies that the learned model $\bfW^{(L)}$ is improved if the initial weights lie in a region near the ground truth $\bfW^*$ whose radius is both lower and upper bound by some function of $\hat{\lambda}$ and $M$. With the same number of labeled data, if we increase the number of unlabeled data (larger $M$), the lower bound decreases and upper bound increases, which indicates the region of initial weights for improved learned model enlarged (see the lines in red and blue in Figure \ref{fig: Thm2_region}(a)). In contrast, if we increase the value of $\hat{\lambda}$, both the lower and upper bound of the radius decreases, which indicates that the region of initial weights for improved learned model moves towards to the ground truth (see the lines in red and black in Figure \ref{fig: Thm2_region}(a)). 
From Figure \ref{fig: Thm2_region} (a), we can see that the convergent point is better than the initial point in terms of the distance to the ground truth if the initial weights lie in the region between the two vertical dash lines in the same color. 
Theorem \ref{Thm: p_convergence} indicates that the learned model $\bfW^{(L)}$ is improved if the initial weights lie in a region near the ground truth $\bfW^*$. With the same number of labeled data, if we increase the number of unlabeled data (larger $M$),  the region of initial weights for improved learned model enlarged (see the lines in red and blue in Figure \ref{fig: Thm2_region}(a)). Hence, to guarantee the improved learned model over the initial weights, the algorithm can tolerant a larger region of initial weights with a larger number of unlabeled data. In contrast, with the same number of labeled data, if we decrease the value of $\hat{\lambda}$,  the region of initial weights for improved learned model moves towards to the ground truth (see the lines in red and black in Figure \ref{fig: Thm2_region}(a)). Therefore, given a bad initial model whose weights are far away from the ground truth, we need to choose a small $\hat{\lambda}$ to guarantee the improved learned model over the initial weights.

\textbf{3. The performance of learned model $\bfW^{(L)}$.} 
%  From \eqref{eqn: p_convergence},
%  we know the learned model by Algorithm \ref{Algorithm: Alg1} converges linearly to a point that lies in the neighbor region of $\WL$, and the relationships of $\w[L]$, $\WL$ and $\bfW^*$ are illustrated in Figure \ref{fig: Thm2_region}(b) as well. $\WL$ is a convex combination of the initial weights $\W[0]$ and ground truth $\bfW^*$, and the distance between $\WL$ and the ground truth $\bfW^*$ becomes smaller with larger $\hat{\lambda}$. Note that the value of $\hat{\lambda}$ is upper bounded by the number of labeled data $N$, therefore the convergent point moves closer to $\bfW^*$ if we increase the number of labeled data. Also, with sufficiently large $N$, $\WL$ can be exactly as $\bfW^*$. 
%  Additionally, the distance between $\W[L]$ and $\WL$ is a function of the number of unlabeled data $M$. With larger $M$, the value of $\|\W[L]-\WL\|_F$, which is denoted as $\mathcal{E}_3$ in Figure \ref{fig: Thm2_region}(b), become smaller. However, unlike the labeled data, the distance between $\W[L]$ and $\WL$ cannot be arbitrarily small even with infinite number of unlabeled data.
 The learned model by Algorithm \ref{Algorithm: Alg1} converges linearly to a point that lies in the neighbor region of $\WL$, and the relationships of $\w[L]$, $\WL$ and $\bfW^*$ are illustrated in Figure \ref{fig: Thm2_region}(b) as well. $\WL$ is a convex combination of the initial weights $\W[0]$ and ground truth $\bfW^*$, and the distance between $\WL$ and the ground truth $\bfW^*$ becomes smaller with larger $\hat{\lambda}$. Note that the value of $\hat{\lambda}$ is upper bounded by the number of labeled data $N$, therefore the convergent point moves closer to $\bfW^*$ if we increase the number of labeled data. Also, with sufficiently large $N$, both $\W[L]$ and $\WL$ can be exactly as $\bfW^*$. 
 Additionally, the distance between $\W[L]$ and $\WL$ is a function of the number of unlabeled data $M$. With larger $M$, the value of $\|\W[L]-\WL\|_F$, which is denoted as $\mathcal{E}_3$ in Figure \ref{fig: Thm2_region}(b), become smaller. However, unlike the labeled data, the distance between $\W[L]$ and $\WL$ cannot be arbitrarily small even with infinite number of unlabeled data.
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.9\linewidth]{Figure/Thm2_region.pdf}
%     \caption{(a) The Landscape of the objective function with different $M$ and $\hat{\lambda}$; (b) The convergent point return by Algorithm \ref{Algorithm: Alg1}}
%     \label{fig: Thm2_region}
% \end{figure}
\fi



%\subsection{Formal theoretical results}
% Before presenting the main results, we first
% define some notations to simplify the theorems. 
% $\mu$ is defined as 
% \begin{equation}\label{eqn: mu}
%     \begin{split}
%           \mu
%         = \mu( \delta, \de) 
%         := \frac{\lambda\delta^2+\w[\lambda]\de^2}{\lambda\rho(\delta)+\w[\lambda]\rho(\de)},
%     \end{split}
% \end{equation}
% where $\rho$ is a positive function in \citep{ZSJB17}. Additionally, we use $c(\kappa)$ to denote some polynomial function value of $\kappa$, and $\kappa$ is the conditional number of the ground truth weights $\bfW^*$. With these notations, we specify the value of $N^*$ in \eqref{eqn: definition_N*} as 
% \begin{equation}\label{eqn: value_of_N*}
%     N^* = c(\kappa)\mu^2K^3d\log q,
% \end{equation}
% for some positive constant $q$, and the value in \eqref{eqn: value_of_N*} is the tightest bound among the existing theoretical results,  to the best of our knowledge, for supervised learning algorithms reaching zero generalization error.

\subsection{Formal theory in low labeled-data regime}

% \SL{[Organization flaw: You mention equations later equations too many times, but these equation have not been presented. I try to add `Takeaways' to address this flaw.]}

{\textit{Takeaways of Theorem\,1:}
Theorem 1 characterizes the convergence rate of the proposed algorithm and the accuracy of the learned model $\W[L]$ 
%through \eqref{eqn: p_convergence} and \eqref{eqn: p_convergence_*} 
in a low labeled-data regime. Specifically, the iterates converge linearly, and the learned model is close to  $\WL$ and guaranteed to outperform the initial model $\bfW^{(0)}$.} 

% \SL{[should this following paragraph go to after thr 1?]}



\begin{theorem}\label{Thm: p_convergence}
\Revise{Suppose the initialization  $\bfW^{(0)}$ and the number of labeled data  satisfy 
    \begin{equation}\label{eqn: definition_p}
        \| \bfW^{(0)} -\bfW^* \|_F \le  p^{-1}\cdot \frac{\|\bfW^*\|_F}{c(\kappa) \mu^2 K^{3/2}} \quad \text{with} \quad p\in \big(\frac{1}{2}, 1\big],
    \end{equation}
    % where $\bfW^{(0)}$ is an initial teacher model computed from labeled data only.
 %   Then, given the number of labeled data satisfies
    \begin{equation} \label{eqn:Nbound}
\hspace{-1in} \textrm{ and }\quad         \max\Big\{ \frac{1}{K}, p - \frac{2p-1}{\mu\sqrt{K}}\Big\}^2 \cdot N^* \le N \le N^*. 
    \end{equation}
If the value of $\hat{\lambda}$ in \eqref{eqn: definition_lambda} and unlabeled data amount $M$ satisfy
    \begin{equation}\label{eqn: thm1_condition1}
        \max\Big\{ \frac{1}{K}, p - \frac{2p-1}{\mu\sqrt{K}}\Big\}\le\hat{\lambda} \le \min \Big\{\sqrt{\frac{N}{N^*}}, p+ \frac{2p-1}{\mu\sqrt{K}}\Big\},
    \end{equation}
    \begin{equation}\label{eqn: thm1_condition2}
   \hspace{-1in}     \text{ and } \quad  M\ge (2p-1)^{-2} c(\kappa) \mu^2 \big( 1-  \hat{\lambda}\big)^2 K^3 d\log q.
    \end{equation}
    % Then, suppose the number of unlabeled data $M$ and the normalization factor $p$ and number of unlabeled data $M$ satisfy the following conditions
    % \iffalse
    % \begin{equation}\label{eqn: thm1_condition}
    %     \begin{gathered}
    %         {1}/{K}\le\hat{\lambda} \le \sqrt{{N}/{N^*}},\\
    %         M\ge  c(\kappa) \mu^2 \big( 1-  \hat{\lambda}\big)^2 K^3 d\log q,\\
    %         \hat{\lambda}-\Big(1-\Theta\big(\frac{1}{\sqrt{M}}\big)\Big)\cdot\frac{\hat{\lambda}}{\mu \sqrt{K}}
    %      < p < 
    %      \hat{\lambda}+\Big(1-\Theta\big(\frac{1}{\sqrt{M}}\big)\Big)\cdot\frac{\hat{\lambda}}{\mu \sqrt{K}}.
    %     \end{gathered}
    % \end{equation}
    % \fi
    % \begin{equation}\label{eqn: thm1_condition1}
    % \vspace{-1.5mm}
    %   {1}/{K}\le\hat{\lambda} \le \sqrt{{N}/{N^*}},
    % \end{equation}
    % \begin{equation}\label{eqn: thm1_condition2}
    % \vspace{-1.5mm}
    %     M\ge  c(\kappa) \mu^2 \big( 1-  \hat{\lambda}\big)^2 K^3 d\log q,
    % \end{equation}
    % \begin{equation}\label{eqn: thm1_condition3}
    % \vspace{-0.5mm}
    %      \hat{\lambda}-\Big(1-\Theta\big(\frac{1}{\sqrt{M}}\big)\Big)\cdot\frac{\hat{\lambda}}{\mu \sqrt{K}}
    %      < p < 
    %      \hat{\lambda}+\Big(1-\Theta\big(\frac{1}{\sqrt{M}}\big)\Big)\cdot\frac{\hat{\lambda}}{\mu \sqrt{K}}.
    % \end{equation}
    Then, when the number $T$ of SGD iterations  is large enough in each loop $\ell$, with probability at least $1-q^{-d}$,
     the iterates $\{ \bfW^{(\ell)} \}_{\ell=0}^{L}$ converge to $\WL$ as 
    \begin{equation}\label{eqn: p_convergence}
  %  \vspace{-1mm}
    %    \begin{split}
 \resizebox{.96\hsize}{!}{$\| \W[L]-\WL \|_F 
            \le \bigg(\Big(1+\Theta\big(\frac{\mu(1-\hat{\lambda})}{\sqrt{M}}\big)\Big)\cdot \hat{\lambda} \bigg)^L \cdot \| \bfW^{(0)}-\WL \|_2  +\Big(1+\Theta\big(\frac{\mu(1-\hat{\lambda})}{\sqrt{M}}\big)\Big) \cdot \| \bfW^* - \WL \|_F,$}%\\
    %&+\Big(1+\Theta\big(\frac{\mu(1-\hat{\lambda})}{\sqrt{M}}\big)\Big) \cdot \| \bfW^* - \WL \|_F,
      %  \end{split}
    \end{equation}
    where $\WL = \hat{\lambda}\bfW^* + (1-\hat{\lambda})\W[0]$. Typically, when the iteration number $L$ is sufficient large, we have
    \begin{equation}\label{eqn: p_convergence_*}
         \begin{split}
        \vspace{-1mm}
             \| \W[L]-\bfW^* \|_F 
            % \le \Big(1-\hat{\lambda} + \Theta(\frac{1}{\sqrt{M}})\frac{1}{K}\Big)\cdot \| \bfW^* - \bfW^{(0)} \|_F\\
            \le \Big(1+\Theta\big(\frac{\mu(1-\hat{\lambda})}{\sqrt{M}}\big)\Big) \cdot 2(1-\hat{\lambda})\cdot \| \bfW^* - \bfW^{(0)} \|_F.
         \end{split}
    \end{equation}}
    \vspace{-1mm}
\end{theorem}


The accuracy of the learned model $\W[L]$ with respect to $\bfW^*$ is characterized as
\eqref{eqn: p_convergence}, and the learning model is better than initial model as in
\eqref{eqn: p_convergence_*} if the following conditions hold.
First, the weights $\lambda$ in \eqref{eqn: empirical_risk_function} are properly chosen as in \eqref{eqn: thm1_condition1}. Second, the number of unlabeled data is sufficiently large as in \eqref{eqn: thm1_condition2}. 
% \Revise{Third, the selection of $\hat{\lambda}$ should match the initial model $\bfW^{(0)}$ in \eqref{eqn: thm1_condition3}.}


\Revise{
 \textbf{Selection of $\lambda$ in self-training algorithms}.   When $\hat{\lambda}$ increases, the required number of unlabeled data  is reduced from  \eqref{eqn: thm1_condition2}, and  the convergence point $\bfW^{(L)}$ becomes closer to $\bfW^*$ from \eqref{eqn: p_convergence_*}, which indicates a smaller generalization error. Thus, a large  $\hat{\lambda}$ within its feasible range \eqref{eqn: thm1_condition1} is desirable.  When the initial model $\bfW^{(0)}$  is closer to  $\bfW^*$ (corresponding to a larger $p$), and the number of labeled data $N$ increases, the upper bound in \eqref{eqn: thm1_condition1} increases, and thus, one can select a larger $\hat{\lambda}$.}

\Revise{
\textbf{The initial model $\bfW^{(0)}$}.  The 
tensor initialization from \citep{ZSJB17} can return  a  $\bfW^{(0)}$ that satisfies \eqref{eqn: definition_p} when the number of labeled data is $N = p^2N^*$ (see Lemma \ref{Thm: p_initialization} in Appendix). Combining with the requirement in \eqref{eqn:Nbound}, Theorem 1 applies to the case that $N$ is at least $N^*/4$.}

%and     First,  with a larger number of labeled data, the feasible range of $\hat{\lambda}$ become larger from \eqref{eqn: thm1_condition1}. Further, we can possibly choose a larger $\hat{\lambda}$. Thus, the required number of unlabeled data is reduced from \eqref{eqn: thm1_condition2}, and the convergence point $\bfW^{(L)}$ becomes closer to the ground truth from \eqref{eqn: p_convergence_*}, which indicates a smaller generalization error. Second, when $p$ is small, the feasible range of $\hat{\lambda}$ becomes large, and the requirement on initialization becomes less restrictive. However, $p$ has a lower bound from \eqref{eqn: definition_p} such that the initialization cannot be arbitrarily far away from $\bfW^*$. In particular, tensor initialization from \citep{ZSJB17} can return an initialization that satisfying \eqref{eqn: definition_p} with $N = p^2N^*$ (see Lemma \ref{Thm: p_initialization} in Appendix). In addition, for the best possible improvement, we need to set $\hat{\lambda}$ as in the order of the largest possible value of $p$, instead of  a smaller value. Finally, due to the complex influence of initialization, labeled and unlabeled data amount in the theorem,  we cannot derivate the best choice of $\hat{\lambda}$. Instead, a suitable choice of $\hat{\lambda}$ from \eqref{eqn: thm1_condition1} and \eqref{eqn: thm1_condition2} is in the order of $\frac{ \sqrt{N} }{ \sqrt{N}+\sqrt{M} }$. In practice, we see that \citep{CRSD19} picks $\lambda$ as $\frac{N}{N+M}$, which is also an increasing function of $N$ and a decreasing faction of $M$.}

%\Revise{
%(\textbf{Selection of $\lambda$ in self-training algorithms}.) It is easy to check that $\lambda$ is positively related with $\hat{\lambda}$ from \eqref{eqn: definition_lambda}. Typically, when $\delta =\de$, $\hat{\lambda}$ is exactly $\lambda$. Therefore, we will focus on the analysis of $\hat{\lambda}$. First,  with a larger number of labeled data, the feasible range of $\hat{\lambda}$ become larger from \eqref{eqn: thm1_condition1}. Further, we can possibly choose a larger $\hat{\lambda}$. Thus, the required number of unlabeled data is reduced from \eqref{eqn: thm1_condition2}, and the convergence point $\bfW^{(L)}$ becomes closer to the ground truth from \eqref{eqn: p_convergence_*}, which indicates a smaller generalization error. Second, when $p$ is small, the feasible range of $\hat{\lambda}$ becomes large, and the requirement on initialization becomes less restrictive. However, $p$ has a lower bound from \eqref{eqn: definition_p} such that the initialization cannot be arbitrarily far away from $\bfW^*$. In particular, tensor initialization from \citep{ZSJB17} can return an initialization that satisfying \eqref{eqn: definition_p} with $N = p^2N^*$ (see Lemma \ref{Thm: p_initialization} in Appendix). In addition, for the best possible improvement, we need to set $\hat{\lambda}$ as in the order of the largest possible value of $p$, instead of  a smaller value. Finally, due to the complex influence of initialization, labeled and unlabeled data amount in the theorem,  we cannot derivate the best choice of $\hat{\lambda}$. Instead, a suitable choice of $\hat{\lambda}$ from \eqref{eqn: thm1_condition1} and \eqref{eqn: thm1_condition2} is in the order of $\frac{ \sqrt{N} }{ \sqrt{N}+\sqrt{M} }$. In practice, we see that \citep{CRSD19} picks $\lambda$ as $\frac{N}{N+M}$, which is also an increasing function of $N$ and a decreasing faction of $M$.}
% In contrast, the condition on $p$ in \eqref{eqn: thm1_condition3} can be understood as the requirement on the parameter $\hat{\lambda}$. The value of $p$ depends on the inverse of the distance between the ground truth and initialization, and both the lower and upper bound of $p$ in \eqref{eqn: thm1_condition3} is a linear function of $\hat{\lambda}$. Therefore, with a bad initialization ($p$ is close to $0$), $\hat{\lambda}$ needs to be smaller such that \eqref{eqn: thm1_condition3} holds, and we also need a larger number of unlabeled data from \eqref{eqn: thm1_condition2}. Since the lower bound of $\hat{\lambda}$ does not depend on the labeled data amount $N$, Theorem 2 does not have any strong requirement depending on $N$ for the initialization. Nevertheless, as the upper bound of $\hat{\lambda}$ depends on $N$, the initialization has a lower bound. However, $\bfW^{(0)}$ cannot be  sufficiently close to $\bfW^*$, and unlabeled data do not help further, which is a trivial case in practice.}

% {The first two conditions in \eqref{eqn: thm1_condition1} and \eqref{eqn: thm1_condition2} are straight-forward, while
% the requirement on $\bfW^{(0)}$ through $p$ in \eqref{eqn: thm1_condition3} can be intuitively understood as follows.} The lower bound on $p$ means that $\bfW^{(0)}$ cannot be too faraway from $\bfW^*$. As  minimizing the weighed empirical risk in \eqref{eqn: empirical_risk_function} is a nonconvex problem, the analyses focus on the local convex region near  $\bfW^*$. The lower bound   is a  minor requirement,  as Lemma \ref{Thm: p_initialization} (in appendix) shows that $\bfW^{(0)}$ computed  from the labeled data using the tensor method  \citep{ZSJB17} satisfies the bound. The lower bound on $p$ means that $\bfW^{(0)}$ cannot be too close to $\bfW^*$ so that the learned model $\bfW^{(0)}$ improves upon $\W[L]$. Otherwise, $\bfW^{(0)}$ is already sufficiently close to $\bfW^*$, and unlabeled data do not help further. Similar requirements also appear in    \citep{WSCM20} (Assumption 4.1) that the initial model shall be neither too bad nor too good. Moreover, \eqref{eqn: thm1_condition3} is just a sufficient condition for analysis. In practice, $\W[L]$ outperforms the initial model for a wide range of $\bfW^{(0)}$, see, e.g., \citep{XLHL20,CRSD19}.

\iffalse
The requirement on $\bfW^{(0)}$ through $p$ in \eqref{eqn: thm1_condition} can be intuitively understood as follows. Compared with conventional training problem without unlabeled data, a sufficiently large $M$ improves the local landscape of the objective function in \eqref{eqn: empirical_risk_function} around $\bfW^*$ such as a local minimizer, if any, gets closer to $\bfW^*$ as $M$ increases. Thus, $\bfW^{(0)}$ needs to be in the neighborhood of  $\bfW^*$, i.e., $p$ has a  lower bound, so that the proposed algorithm converges to such a minimizer. The lower bound in \eqref{eqn: thm1_condition} is a  minor requirement,  as Lemma \ref{Thm: p_initialization} (in appendix) shows that $\bfW^{(0)}$ computed from the tensor method  \citep{ZSJB17} satisfies the bound.  The upper bound  in  \eqref{eqn: thm1_condition} may be counter-intuitive. That is because if $\bfW^{(0)}$ is already sufficiently close to $\bfW^*$,   $\W[L]$ can not necessarily be proved to be closer to $\bfW^*$. The upper bound addresses the technical caveat so that we focus on the situation when $\W[L]$ is better than $\bfW^{(0)}$. It is only a sufficient but not necessary condition. 
One can see a similar conclusion in \citep{WSCM20} as well. That is, from Assumption 4.1, the initial model needs to be good enough such that only a small fraction of pseudo labels are not correct. Additionally, the accuracy of the initial model cannot be arbitrarily small in order to guarantee that the learned model is improved over the initial model.
In practice, both our experiments in Section \ref{sec: empirical_results} and other existing works like \citep{XLHL20,CRSD19} show that $\W[L]$ outperforms the initial teacher model for a wide range of $\bfW^{(0)}$.
\fi

% When $\delta=1$ such that labeled data are generated from the standard Gaussian, $\mu$ is minimized for all $\tilde{\delta} \leq 1$ (see in Lemma \ref{lemma: rho_order}).  The required number of unlabeled data is also minimized under such a data distribution.



\subsection{Formal theory of achieving  zero generalization error}
\textit{Takeaways of Theorem\,2:} 
\Revise{Theorem \ref{Thm: sufficient_number} indicates the model returned by the proposed algorithm converges linearly to the ground truth $\bfW^*$. Thus the distance between the learned model and the ground truth can be arbitrarily small with the ability to achieve zero generalization error. The required sample complexity is reduced by a constant factor compared with supervised learning.}



\begin{theorem}\label{Thm: sufficient_number}
Consider the number of unlabeled data satisfies
   \begin{equation}\label{eqn: main_sample}
    \begin{split}
    \big(1 - {1}/{(\mu\sqrt{K})} \big)^2\cdot N^* \leq    N \leq    N^*,
    \end{split}
    \end{equation}
    we choose $\hat{\lambda}$ such that
    \begin{equation}\label{eqn: lambda_hat_s}
   1 - {1}/{(\mu\sqrt{K})} \leq     \hat{\lambda} \leq \sqrt{{N}/{N^*}}. 
    \end{equation}
Suppose the initial model $\bfW^{(0)}$  and the number of unlabeled data $M$ satisfy
\begin{equation}\label{eqn: Thm2_condition}
    \| \bfW^{(0)} -\bfW^* \|_F  \le \frac{\|\bfW^*\|_F}{c(\kappa)\mu^{2}K^{3/2}} \quad \text{and}\quad  M \geq c(\kappa)\mu^{2}(1-\hat{\lambda})^2 K^3 d\log q,
\end{equation}
    % \begin{equation}\label{eqn: Thm2_initial}
    %     \| \bfW^{(0)} -\bfW^* \|_F  \le \frac{\sigma_K}{c(\kappa)\mu^{2}K},
    % \end{equation}
    % \begin{equation}\label{eqn: main_M}
    %     M \geq c(\kappa)\mu^{2}(1-\hat{\lambda})^2 K^3 d\log q,
    % \end{equation}
    the iterates $\{ \bfW^{(\ell)} \}_{\ell=0}^{L}$ converge to the ground truth $\bfW^*$  as  follows,
    \begin{equation}\label{eqn: convergence}
    \vspace{-1mm}
         \| \W[L] -\bfW^* \|_F \le \Big[ \big(1+\frac{c(\kappa)\hat{\lambda}}{\sqrt{N}}+\frac{c(\kappa)(1-\hat{\lambda})}{\sqrt{M}}\big)\cdot\mu\sqrt{K}(1-\hat{\lambda}) \Big]^L 
        \cdot \| \W[0]-\bfW^* \|_F.
    \vspace{-1mm}
    \end{equation}
    % where 
    % \begin{equation}\label{eqn: convergence_rate}
    % \begin{split}
    %     &\nu_1(\beta^*) = 1- \Theta
    %     \Big(
    %     \frac{1-\Theta(\frac{\hat{\lambda}}{\sqrt{N}})-\Theta(\frac{1-\hat{\lambda}}{\sqrt{M}})}{\mu\sqrt{K}} 
    %     \Big),\\
    %     % \nu_2 = \Theta\Big( \frac{\w[\varepsilon]\mu}{\sqrt{K}}\Big) + \Theta\Big( \frac{\w[\lambda]\de^2}{\lambda\delta^2+\w[\lambda]\de^2} \Big).
    %     &\tcr{\nu_2 =  \Theta\Big(1+\Theta\big(\frac{\hat{\lambda}}{\sqrt{N}}\big)+\Theta\big(\frac{1-\hat{\lambda}}{\sqrt{M}}\big)\Big)\cdot\mu\sqrt{K}(1-\hat{\lambda}).}
    % \end{split}
    % \end{equation}
\end{theorem}


The models $\W[\ell]$'s  converge linearly  to the ground truth $\bfW^*$ as \eqref{eqn: convergence} when the number of labeled data 
satisfies \eqref{eqn: main_sample}. In contrast, supervised learning requires at least $N^*$ labeled samples to estimate $\bfW^*$ accurately without unlabeled data, which suggests self-training at least saves a constant fraction of labeled data.

\iffalse
\begin{theorem}\label{Thm: sufficient_number}
    Let $\hat{\lambda}$ be the value as
    \begin{equation}\label{eqn: lambda_hat_s}
        \hat{\lambda} \ge 1 - \frac{1}{\mu\sqrt{K}}. 
    \end{equation}
    Given any initial weights $\bfW^{(0)}$ that satisfies
    \begin{equation}\label{eqn: Thm2_initial}
        \| \bfW^{(0)} -\bfW^* \|_F  \le \frac{\sigma_K}{c(\kappa)\mu^{2}K}
    \end{equation}
    and the number of labeled that satisfies
    \begin{equation}\label{eqn: main_sample}
    \begin{split}
        N\ge \hat{\lambda}^2\cdot N^*,
    \end{split}
    \end{equation}
    Further, suppose the number of unlabeled data is sufficiently large as 
    \begin{equation}\label{eqn: main_M}
        M= c(\kappa)\mu^{2}(1-\hat{\lambda})^2 K^3 d\log q,
    \end{equation}
    the iterations $\{ \bfW^{(\ell)} \}_{\ell=0}^{L}$ converge to the ground truth as 
    \begin{equation}\label{eqn: convergence}
        \lim_{T\to \infty}\| \W[L] -\bfW^* \|_F \le \bigg[ \Big(1+\Theta\big(\frac{\hat{\lambda}}{\sqrt{N}}\big)+\Theta\big(\frac{1-\hat{\lambda}}{\sqrt{M}}\big)\Big)\cdot\mu\sqrt{K}(1-\hat{\lambda}) \bigg]^L 
        \cdot \| \W[0]-\bfW^* \|_F.
    \end{equation}
    % where 
    % \begin{equation}\label{eqn: convergence_rate}
    % \begin{split}
    %     &\nu_1(\beta^*) = 1- \Theta
    %     \Big(
    %     \frac{1-\Theta(\frac{\hat{\lambda}}{\sqrt{N}})-\Theta(\frac{1-\hat{\lambda}}{\sqrt{M}})}{\mu\sqrt{K}} 
    %     \Big),\\
    %     % \nu_2 = \Theta\Big( \frac{\w[\varepsilon]\mu}{\sqrt{K}}\Big) + \Theta\Big( \frac{\w[\lambda]\de^2}{\lambda\delta^2+\w[\lambda]\de^2} \Big).
    %     &\tcr{\nu_2 =  \Theta\Big(1+\Theta\big(\frac{\hat{\lambda}}{\sqrt{N}}\big)+\Theta\big(\frac{1-\hat{\lambda}}{\sqrt{M}}\big)\Big)\cdot\mu\sqrt{K}(1-\hat{\lambda}).}
    % \end{split}
    % \end{equation}
\end{theorem}

\textbf{Remark 2.1 (Saved sample complexity of labeled data):}
Suppose we do not have unlabeled data, which is equivalent to say that $\hat{\lambda} =1$, the required number of samples is exactly $N^*$. Then, the results in Theorem \ref{Thm: sufficient_number} reduce to the case of supervised learning.  When we have enough unlabeled data as shown in \eqref{eqn: main_M}, the sample complexity of $N$ for achieving zero generalization error can be reduced by a factor of $\hat{\lambda}$ at the cost of a slower convergence rate. Note that the smallest possible value of $\hat{\lambda}$ is $1-\mu^{-1}K^{-1/2}$, the smallest sample complexity for labeled data can be $(1-\mu^{-1}K^{-1/2})^2 N^*$.

\textbf{Remark 2.2 (Convergence rate):} 
From \eqref{eqn: convergence}, we know that convergence rates is in the order of $\big(1+\Theta(\frac{\hat{\lambda}}{\sqrt{N}})+\Theta(\frac{1-\hat{\lambda}}{\sqrt{M}})\big)\cdot\mu\sqrt{K}(1-\hat{\lambda})$. With the same $\hat{\lambda}$, the convergence rate
decreases, which indicates a faster convergence,  as a linear function of both $1/\sqrt{M}$ and $1/\sqrt{N}$.
Additionally, given the same $N$ and $M$, decreasing the value of $\hat{\lambda}$ will lead to  a slower convergence rate.
\fi


\subsection{The main proof idea}
Our proof  builds upon and extends one recent line of works on supervised learning such as \citep{ZSJB17,ZWLC20_2,ZWLC20_3,ZWLC21}. The standard framework of these works is first to show that the generalization function $I(g(\bfW))$ in \eqref{eqn: GF} is locally convex near $\bfW^*$, which is its global minimizer. Then, when $M=0$ and $N$ is sufficiently large, the empirical risk function using labeled data only can approximate  $I(g(\bfW))$ well  in the neighborhood of $\bfW^*$. Thus, if initialized in this local convex region, the iterations, returned by applying gradient descent approach on the empirical risk function, converge to $\bfW^*$ linearly.

The technical challenge here is that in self-training, when unlabeled data are paired with pseudo labels, $\bfW^*$ is no longer a global minimizer of the empirical risk $\hat{f}_{\mathcal{D},\widetilde{\mathcal{D}}}$ in \eqref{eqn: empirical_risk_function}, and $\hat{f}_{\mathcal{D},\widetilde{\mathcal{D}}}$ does not approach $I(g(\bfW))$ even when $M$ and $N$ increase to infinity. Our new idea is to design a population risk function $f(\bfW; \hat{\lambda})$ in \eqref{eqn: p_population_risk_function} (see appendix), which is a lower bound of $\hat{f}_{\mathcal{D},\widetilde{\mathcal{D}}}$ when $M$ and $N$ are infinity. $f(\bfW; \hat{\lambda})$ is locally convex around its minimizer $\WL$, and $\WL$ approaches $\bfW^*$ as $\hat{\lambda}$ increases. Then we show the iterates generated by $\hat{f}_{\mathcal{D},\widetilde{\mathcal{D}}}$ stay close to $f(\bfW; \hat{\lambda})$, and the returned model $\W[L]$ is close to $\WL$. New technical tools are developed to bound the distance between the functions $\hat{f}_{\mathcal{D},\widetilde{\mathcal{D}}}$ and $f(\bfW; \hat{\lambda})$.

\iffalse
The proofs follow the frameworks  built in \citep{ZSJB17} for supervised learning problems, major technical changes are made in this paper to generalize the analysis to the self-training algorithm. Due to the randomness of the realizations of the variables in $\mathcal{D}$ and $\widetilde{\mathcal{D}}$, one cannot directly characterize the landscape of the objective function (ERF) in \eqref{eqn: empirical_risk_function}. Instead, we first 
introduce and analyze the population risk function, which is defined as the expectation of certain transformed objective function as shown in \eqref{eqn: p_population_risk_function} and \eqref{eqn: population_risk_function} (see in appendix). Next, we utilize concentration theorem to  bound the distances between the population and objective functions. Then, the behaviors of the iterates on the objective function can be  described as the ones on the population risk function plus the distance between these two functions. 
\fi
% \begin{figure}[H]
%     \centering
% \begin{subfigure}{0.325\textwidth}
%   	\centering
%   	\includegraphics[width=0.90\linewidth]{Figure/AGD_part1.pdf}
%   	\caption{Unlabeled data}
%   	\label{fig: proof_1}
% \end{subfigure}
% \begin{subfigure}{0.33\textwidth}
%   	\centering
%   	\includegraphics[width=1.0\linewidth]{Figure/AGD_part2.pdf}
%   	\caption{Insufficient labeled data}
%   	\label{fig: proof_2}
% \end{subfigure}
% \begin{subfigure}{0.325\textwidth}
%   	\centering
%   	\includegraphics[width=1.0\linewidth]{Figure/AGD_part3.pdf}
%   	\caption{Sufficient labeled data}
%   	\label{fig: proof_2}
% \end{subfigure}
% \caption{The landscape of the empirical and population risk functions }
% \label{fig: proof}
% \end{figure}


\iffalse
\subsection{Comparison with existing theoretical results}
\tcr{To the best of our knowledge, there are limited number of 
of the theoretical results in the field of self-training \citep{CWKM20,RXYDL20, OG20, OADAR11, WSCM20}, however, none of them follow the line of model recovery as this paper. All the works among the works mentioned above, except \citep{WSCM20}, only study the linear model problems. Under the expansion and separation assumptions for labeled data,
\citep{WSCM20} proves that unlabeled data indeed improves the test accuracy. Compared with \citep{WSCM20}, this paper characterizes the  order dependence of the generalization error and convergence rate with the number of unlabeled data quantatively. Additionally, \citep{WSCM20} only provides the sample complexity analysis for unsupervised learning problems when
the labeled data have sufficiently large margins between different classes, and the sample complexity is a polynoimal function of the margins. While this paper considers regression problems and  presents the sample complexity bound for self-training methods, and the bound is a linear function of the input dimension, which is order-wise optimal as well.}

As the techniques used in this paper are built upon existing work
\citep{ZSJB17}, which is to solve supervised learning problems, we will make a further comparison with \citep{ZSJB17} as well. 
 In this paper, all the existing lemmas and techniques need to be modified or re-built in this paper for semi-supervised learning algorithms because the objective function is different from the one in \citep{ZSJB17} with unlabeled data. Additionally, as shown in Figure \ref{fig: landscape}, in low labeled-data regime ($N<N^*$), the landscape of the objective function contains many fake local minimum near the ground truth, and the initial point generated by the tensor initiation is not close enough to the ground truth, either. 
To better characterize the landscape of the objective function near the initial point, the population risk function is defined as \eqref{eqn: p_population_risk_function} with global optimal in $\overline{\bfW}(p)$, which is in between the ground truth and the initial point. In the end, the distance between the learned model $\bfW^{(L)}$ and the ground truth is characterized by bounding the distances of these two points to a third point $\overline{\bfW}(p)$. 
% As for the case of sufficient number of samples, the local convex region near the ground truth of the objective function becomes much larger, and we can find an initial point that lies near the local convex region through tensor initialization as well. Therefore, we can directly define the population risk function as the expectation of \eqref{eqn: empirical_risk_function} to characterize the behaviors of the iterations. In this case, ground truth $\bfW^*$ is the global optimal to both the objective and population risk functions, as shown in Figure \ref{fig: landscape}.    



% \begin{figure}[H]
%   	\centering
%   	\includegraphics[width=0.4\linewidth]{Figure/AGD_1.pdf}
%   	\caption{The landscape of the objective function for insufficient number of samples}
%   	\label{fig: proof_1}
% \end{figure}

% \begin{figure}[H]
%   	\centering
%   	\includegraphics[width=0.4\linewidth]{Figure/AGD_2.pdf}
%   	\caption{The landscape of the objective function for sufficient number of samples}
%   	\label{fig: proof_1}
% \end{figure}

\fi 

==> Self-training (6)/Thm1.tex <==
% Let us define $\overline{\bfW} = q\cdot \bfW^* + ( 1 - q )\cdot \bfW^{(0)}$, where $\W[0]$ denotes the initial point.
\iffalse
\begin{theorem}[Initialization]
\label{Thm: p_initialization}
     Assume  the number of samples of labeled data satisfies
     \begin{equation}\label{eqn: p_initial_sample}
         N = \Omega\big( p^2\mu^{4} K^3 d \log  q \big)
     \end{equation}
     for some large constant $q$ and $p\in[0,1]$, the tensor initialization method 
    outputs  ${\bfW}^{(0)}$  such that
    \begin{equation}\label{eqn: p_initialization}
        \| \bfW^{(0,0)} -\bfW^* \|_F  = \mathcal{O}\big(\frac{\sigma_K}{p\mu^{2}K}\big)
    \end{equation}
    with probability at least $1-q^{-d}$.
\end{theorem}
\begin{theorem}[Low labeled data regime]\label{Thm: p_convergence}
    Suppose $\W[0,0]$  satisfies \eqref{eqn: p_initialization}
    with
    \begin{equation}\label{eqn: p}
         \hat{\lambda}-\Theta\Big(\frac{1-M^{-{1}/{2}}}{\mu K^{1/2} }\Big) \cdot\hat{\lambda}
         \le p \le 
         \hat{\lambda}+\Theta\Big(\frac{1-M^{-{1}/{2}}}{\mu K^{1/2} }\Big) \cdot\hat{\lambda},
    \end{equation}
     where
    \begin{equation}\label{eqn: lambda_hat}
        \hat{\lambda} : =\frac{\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2}
        = \mathcal{O}\Big(\mu^{-1} \big(\frac{N}{K^3d \log q}\big)^{\frac{1}{2}}\Big),
    \end{equation}
    and 
    \begin{equation}\label{eqn: mu}
        \mu
        = \mu( \delta, \de) 
        = \frac{\lambda\delta^2+\w[\lambda]\de^2}{\lambda\rho(\delta)+\w[\lambda]\rho(\de)}.
    \end{equation}
    Then, if the number of samples in $\w[\mathcal{D}]$ further satisfies
    % \begin{equation}\label{eqn: p_main_sample}
    % \begin{split}
    %     &N= \Omega\Big( \varepsilon^{-2}\mu^{2}\big(\frac{\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2}\big)^2K^3 d\log q \Big),\\
    %     \end{split}
    % \end{equation}
    \begin{equation}\label{eqn: p_main_sample_M}
        \begin{split}
        M= \Omega \big(  \mu^2 \big( 1-  \hat{\lambda}\big)^2 K^3 d\log q \big),
        \end{split}
    \end{equation}
    the iterates $\{ \bfW^{(\ell,t)} \}_{\ell,t=1}^{L,T}$ converge to $\overline{\bfW}(\hat{\lambda})$ as 
    \begin{equation}\label{eqn: p_convergence}
        \begin{split}
            \| \W[L,T]-\overline{\bfW}(\hat{\lambda}) \|_F 
            \le& \bigg[\Big( 1-\frac{\Theta(1-M^{-{1}/{2}})}{\mu K^{1/2}} \Big)^T +\frac{\Theta(1-M^{-1/2})}{K} \bigg]^L \cdot \| \bfW^{(0,0)}-\overline{\bfW}(p) \|_2\\
            &+\Theta(1+M^{-{1}/{2}})\cdot \frac{1-\hat{\lambda}}{ K}\cdot \| \bfW^* - \bfW^{(0,0)} \|_F
        \end{split}
    \end{equation}
    % \begin{equation}\label{eqn: p_convergence}
    %     \begin{split}
    %         \lim_{\ell\to \infty, t\to \infty} 
    %         \| \W[\ell,t]-\overline{\bfW}(\hat{\lambda}) \|_F \le \Theta(1+M^{-{1}/{2}})\cdot \frac{1-\hat{\lambda}}{ K}\cdot \| \bfW^* - \bfW^{(0,0)} \|_F
    %     \end{split}
    % \end{equation}
    with probability at least $1-q^{-d}$, where $\overline{\bfW}(\hat{\lambda}) = \hat{\lambda}\bfW^* + (1-\hat{\lambda})\W[0,0]$.
\end{theorem}
\begin{corollary}\label{corollary: W*}
    Suppose $\hat{\lambda}$ can be $\Theta(\frac{1}{K})$ while all the conditions in Theorem \ref{Thm: p_convergence} still hold. Then, we have 
    \begin{equation}\label{eqn: p_convergence_*}
        \begin{split}
            \lim_{\ell\to \infty, t\to \infty} \| \W[\ell,t]-\bfW^* \|_F \le \Big(1-\Theta\big(\frac{1}{K^2}\big)\Big)\cdot \| \bfW^* - \bfW^{(0,0)} \|_F
        \end{split}
    \end{equation}
    with probability at least $1-q^{-d}$.
\end{corollary}
\fi
\begin{lemma}\label{lemma: rho_order}
    For ReLU activation function, we have $\rho(z) = \Theta(z^2)$ when $z$ is close to $0$, and $\rho(z) = \Omega(z^2)$ when $z>c$ for some large positive constant. Typically, $\max_{z>0} \rho(z) = 0.089$. 
\end{lemma}

Theorem \ref{Thm: p_convergence} indicates that  
the iterations converge to $\overline{\bfW}(\hat{\lambda})$, which is a weighted average of the ground truth $\bfW^*$ and the initial point $\WI$, up to an error bound that shown in the left-hand side of \eqref{eqn: p_convergence} provided two conditions hold. One condition is that the initial point $\WI$ is not far away from the ground truth up to a distance bounded by \eqref{eqn: p_initialization} with a large $p$ shown in \eqref{eqn: p}, and another one is that the number of unlabeled data $M$ is sufficiently large as shown in \eqref{eqn: p_main_sample_M}.
\\
\noindent
\textbf{Remark 1.1 (Parameter $\mu$):} From \eqref{eqn: mu}, we know $\mu$ is a function of $\delta$ and $\de$. From Lemma \ref{lemma: rho_order}, we know that $\rho(\delta)$ is in the order of $\delta^2$ when $\delta\to 0^+$ for any activation functions. Therefore, when $\delta$ and $\de$ are close to $0$, $\mu$ is a fixed constant. For Lipschitz continuous activation function, we have $\rho(\delta)<\mathcal{O}(\delta^2)$ when $\delta$ is sufficiently large. Hence, when $\delta$ and $\de$ are sufficiently large, increasing the value of $\de$ will lead to the increase of $\mu$, thus we need a higher requirement on the initial point from \eqref{eqn: p_initialization}, a larger $p$ from \eqref{eqn: p}, and a larger size of unlabeled data $M$ from \eqref{eqn: p_main_sample_M}.\\
\noindent
\textbf{Remark 1.2 (Parameter $p$):} From \eqref{eqn: p_initialization}, we know that $\|\WI - \bfW^*\|_F$ is a positive function of $p^{-1}$. If the lower bound of $p$ from \eqref{eqn: p} becomes smaller, then the algorithm can tolerate a larger range of initialization.  
\\
\noindent
\textbf{Remark 1.3 (Parameter $\hat{\lambda}$):} From \eqref{eqn: lambda_hat}, we know that the definition of $\hat{\lambda}$ is ${\lambda\delta^2}/{(\lambda\delta^2+\w[\lambda]\de^2)}$, and the value of $\hat{\lambda}$ should be less than $\mu^{-1}\sqrt{\frac{N}{K^3d\log q}}$. We can see that if we have a larger $N$, which means that the learning problems is accessible to a larger number of labeled data, the value of $\hat{\lambda}$ can be selected as a  larger number. With a larger $\hat{\lambda}$, the algorithm can tolerant a smaller number of unlabeled data from \eqref{eqn: p_main_sample_M} and $p$ from \eqref{eqn: p}, which thus suggests a less requirement on the initialization from \eqref{eqn: p_initialization}. Additionally, given a larger $\lambda$, the convergent point $\overline{\bfW}(\hat{\lambda})$ moves closer to the ground-truth $\bfW^*$, and the error bound between the convergence point and the iterates becomes smaller as well, which indicates that the iterates are closer to the ground-truth. \\
\noindent
\textbf{Remark 1.4 (parameter $M$):} When the number of labeled data $N$ is much less than $\mu^2K^3 d\log q$, where $\hat{\lambda}$ can only be as large as a small constant, then the number of unlabeled data needs to be at least in the order of $\mu^2 K^3 d \log q$ to guarantee the convergence from \eqref{eqn: p_main_sample_M}. 
In addition, suppose the training process is accessible to a larger size of unlabeled data $M$, the iterations converge faster to the convergent point from \eqref{eqn: p_convergence}.
Moreover, with a larger number of unlabeled data $M$, $p$ can achieve a smaller value while \eqref{eqn: p} still holds. Additionally, the error bound of the iteration $\W[\ell,t]$ and $\overline{\bfW}(\hat{\lambda})$ decreases as $M$ increases as well. 


\iffalse
\textbf{Remark 1.1 (Labeled data):} 
From \eqref{eqn: thm1_condition1}, we know that the $\hat{\lambda}$ bounded by $1/K$ and $\sqrt{N/N
^*}$ from below and above, respectively. To provide a meaningful bound, the number of labeled data needs to be at least $N^*/K^2$. 
In addition, since the value of $\hat{\lambda}$ should be less than $\sqrt{{N}/{N^*}}$,  the value of $\hat{\lambda}$ can be selected as a  larger number if we have a larger $N$. With a larger $\hat{\lambda}$, the algorithm can tolerant a smaller number of unlabeled data from \eqref{eqn: p_main_sample_M}. Moreover, given a larger $\hat{\lambda}$, the convergent point $\WL$ moves closer to the ground-truth $\bfW^*$, and the error bound between the convergence point and the iterates becomes smaller as well, which indicates that the iterates are closer to the ground-truth.
 
 
 
\textbf{Remark 1.2 (Unlabeled data):}
From \eqref{eqn: p_main_sample_M}, we can see that the number of unlabeled data needs to be at least in the order of $\mu^2(1-\hat{\lambda})^2K^3d\log q$ to provide analyzable performance.
In addition, suppose the training process is accessible to a larger size of unlabeled data $M$, the iterations converge faster to the convergent point from \eqref{eqn: p_convergence}.
Moreover, with a larger number of unlabeled data $M$, the range of $p$ to guarantee \eqref{eqn: p} enlarged, which indicates a larger range of initialization. Additionally, the error bound of the iteration $\W[\ell]$ and $\WL$ decreases as $M$ increases as well.

\textbf{Remark 1.3 (Initial weights):} From the definition of $p$ in \eqref{eqn: definition_p}, we know that $\|\W[0] - \bfW^*\|_F$ is a linear function of $p^{-1}$. 
Therefore, the constraint for $p$ in \eqref{eqn: p} is in fact the requirement of the initial weights $\W[0]$. From \eqref{eqn: p}, we know that the bounds of $p$ is the functions of $\hat{\lambda}$ and $M$. When the number of unlabeled data increases, the lower bound of $p$ becomes even smaller, and the upper bound becomes even larger, which indicates the range of selectable initial weights is enlarged as well. In contrast, given the same number of labeled data, if we choose a smaller $\hat{\lambda}$, then both the lower and upper bounds of $p$ decreases, which means that the region of selectable initial weights moves further away from the ground truth. It is equivalent to say that we need to select a small $\lambda$ such that $\hat{\lambda}$ is small as well to guarantee the learned model is improved over the initial model if the initialization is not good enough (far away from the ground truth weights $\bfW^*$). Moreover, the initialization can be found through tensor initialization, where the results are summarized in the following Lemma \ref{Thm: p_initialization}.
\begin{lemma}[Initialization]\label{Thm: p_initialization}
     Assuming the number of samples of labeled data satisfies
     \begin{equation}\label{eqn: p_initial_sample}
         N \ge  p^2 N^* 
     \end{equation}
     for some large constant $q$ and $p\in[0,1]$, the tensor initialization method 
    outputs  ${\bfW}^{(0)}$  such that
    \begin{equation}\label{eqn: p_initialization}
        \| \bfW^{(0)} -\bfW^* \|_F  \le \frac{\sigma_K}{p\cdot c(\kappa)\mu^{2}K}
    \end{equation}
    with probability at least $1-q^{-d}$.
\end{lemma}
\fi

\iffalse
\textbf{Remark 1.4 (Parameter $\mu$):} From \eqref{eqn: definition_lambda}, we know $\mu$ is a function of $\delta$ and $\de$. From the following Lemma \ref{lemma: rho_order} (in appendix), we know that $\rho(\delta)$ is in the order of $\delta^2$ when $\delta\to 0^+$ for ReLU activation functions. Therefore, when $\delta$ and $\de$ are close to $0$, $\mu$ is a fixed constant. Nonetheless, $\rho(\delta)$ is less than $\delta^2$ order-wisely when $\delta$ is sufficiently large. Hence, when $\delta$ and $\de$ are sufficiently large, increasing the value of $\de$ will lead to the increase of $\mu$, and thus we require a larger size of unlabeled data $M$ from \eqref{eqn: p_main_sample_M}. In this paper, we study the case that $\delta$ and $\de$ are relative small and fixed as constants.
\begin{lemma}\label{lemma: rho_order}
    For ReLU activation function, we have $\rho(z) = \Theta(z^2)$ when $z$ is close to $0$, and $\rho(z) = \Omega(z^2)$ when $z>c$ for some large positive constant. Typically, $\max_{z>0} \rho(z) = 0.089$. 
\end{lemma}

\fi

==> Self-training (6)/Thm1_old.tex <==
\section{Theoretical results: insufficient sample complexity}
% Let us define $\overline{\bfW} = q\cdot \bfW^* + ( 1 - q )\cdot \bfW^{(0)}$, where $\W[0]$ denotes the initial point.

\begin{theorem}[Initialization]
\label{Thm: p_initialization}
     Assume  the number of samples of labeled data satisfies
     \begin{equation}\label{eqn: p_initial_sample}
         N = \Omega\big( p^2\mu^{4} K^3 d \log  q \big)
     \end{equation}
     for some large constant $q$ and $p\in[0,1]$, the tensor initialization method 
    outputs  ${\bfW}^{(0)}$  such that
    \begin{equation}\label{eqn: p_initialization}
        \| \bfW^{(0)} -\bfW^* \|_F  = \mathcal{O}\big(\frac{\sigma_K}{p\mu^{2}K}\big)
    \end{equation}
    with probability at least $1-q^{-d}$, where $\overline{\bfW}(p) = p\cdot \bfW^* + ( 1 - p )\cdot \bfW^{(0)}$.
\end{theorem}
\begin{theorem}[Convergent point]\label{Thm: p_convergence}
    Let $\frac{\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2}=\Omega\big(\mu^{-1} (\frac{N}{K^3d \log q})^{\frac{1}{2}}\big)$.
     Suppose $\W[0]$ and $\overline{\bfW}(p)$ satisfy \eqref{eqn: p_initialization} 
     and the number of samples in $\w[\mathcal{D}]$ satisfy
    % \begin{equation}\label{eqn: p_main_sample}
    % \begin{split}
    %     &N= \Omega\Big( \varepsilon^{-2}\mu^{2}\big(\frac{\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2}\big)^2K^3 d\log q \Big),\\
    %     \end{split}
    % \end{equation}
    \begin{equation}\label{eqn: p_main_sample_M}
        \begin{split}
        M= \Omega \Big( \tilde{\varepsilon}^{-2} \big( \mu-  (\textstyle\frac{N}{K^3d \log q})^{\frac{1}{2}}\big)^2 K^3 d\log q \Big)
        \end{split}
    \end{equation}
    for some constant $\w[\varepsilon]\in (0, 1)$, where 
    \begin{equation}\label{eqn: mu}
        \mu
        = \mu( \delta, \de) 
        = \frac{\lambda\delta^2+\w[\lambda]\de^2}{\lambda\rho(\delta)+\w[\lambda]\rho(\de)}.
    \end{equation}
    Then, the iterates $\{ \bfW^{(t)} \}_{t=1}^{T}$ converge to the ground truth as 
    \begin{equation}\label{eqn: p_convergence}
        \begin{split}
            \| \W[T] -\overline{\bfW}(p) \|_F 
            \le& 
            \bigg[\Big(1- \Theta\big(\frac{1-\w[\varepsilon]}{\mu\sqrt{K}} 
            \big)\Big)^T + \w[\nu] \bigg]
            \| \W[0]-\overline{\bfW}(p) \|_F 
             + \nu \| \bfW^*-\overline{\bfW}(p) \|_F \\
            % & \| \W[0]-\overline{\bfW} \|_F
        \end{split}
    \end{equation}
    with probability at least $1-q^{-d}$, where
    \begin{equation}\label{eqn: nu}
        \nu = \frac{1}{1-\w[\varepsilon]}\cdot 
        \Big[
        \Theta\Big(\frac{\mu\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2}\Big) + \Theta\Big(\frac{1}{K}\Big)
        \Big],
    \end{equation}
    \begin{equation}\label{eqn: nu_tilde}
        \w[\nu] = \frac{1}{1-\w[\varepsilon]}\cdot 
        \Big[\Theta\Big(\frac{\mu\w[\lambda]\de^2}{\lambda\delta^2+\w[\lambda]\de^2}\Big)+\frac{\w[\varepsilon]}{K} \Big].
    \end{equation}
\end{theorem}
\begin{lemma}[Order analysis of $\rho$]
\label{lemma: rho_order}
    If $\rho(z)>0$ for $z\in(0, \xi)$ for some positive constant $\xi$ and the sub-gradient of $\rho(z)$ at $0$ can be non-zero,  then $\rho(z)=\Theta(z^r)$ when $z\to 0^+$.
\end{lemma}
\noindent
\textbf{Remark 1.1 (Influence of $\mu$):} From \eqref{eqn: mu}, we know $\mu$ is a function of $\delta$ and $\de$. From Lemma \ref{lemma: rho_order}, we know that $\rho(\delta)$ is in the order of $\delta^2$ when $\delta\to 0^+$ for any activation functions. Therefore, when $\delta$ and $\de$ are close to $0$, $\mu$ is a fixed constant. For Lipschitz continuous activation function, we have $\rho(\delta)<\mathcal{O}(\delta^2)$ when $\delta$ is sufficiently large. Hence, when $\delta$ and $\de$ are sufficiently large, increasing the value of $\de$ will lead to the increase of $\mu$, thus we need higher requirement on the initial point from \eqref{eqn: p_initialization} and slower convergence rate from \eqref{eqn: nu} and \eqref{eqn: nu_tilde} in terms of $\mu$. 

\noindent
\tcr{\textbf{Remark 1.2 (Influence of $M$):} 
When $N\ll K^3d$, the factor $\mu -\sqrt{\frac{N}{K^3d}}$ in \eqref{eqn: p_main_sample_M} is larger than $0$ and close to $\mu$. Therefore, with fixed $N$ and $N\ll K^3d$, to gaurantee \eqref{eqn: p_main_sample_M} hold, we need to increase $\w[\varepsilon]$ when $M$ decrease. From \eqref{eqn: nu_tilde}, we know that both $\nu$ and $\w[\nu]$ will increase accordingly, and thus the error term in  \eqref{eqn: p_convergence} will increase as well. Conversely, if we increase $M$, we can obtain smaller error bound, which means that
$\W[T]$ is closer to $\overline{\bfW}(p)$ and $\bfW^*$.}


\noindent
\tcr{\textbf{Remark 1.3 (Parameter $p$):} From \eqref{eqn: p_initialization} and \eqref{eqn: p_convergence}, we know that the best convergent point, where in terms of the distance to $\bfW^*$, returned by gradient descent method is $\overline{\bfW}(p_{\max})$, where $p_{\max}$ is the maximum value of $p$ while \eqref{eqn: p_initial_sample} still holds.
When $N = \Omega(\mu^4K^3d\log q)$, $p$ can be as large as $1$, which suggests that $\overline{\bfW}$ can be $\bfW^*$. However, when $N$ is small, we have $p_{\max}=\Theta(\mu^{-2}(\frac{N}{K^3d})^{\frac{1}{2}})$. Given a fixed initial point $\bfW^{(0)}$, The achievable weights with the smallest distance to $\bfW^*$ are $\overline{\bfW}(p_{\max})$. Also, with larger $N$, $\overline{\bfW}(p_{\max})$ is closer to $\bfW^*$.
}

\noindent
\tcr{\textbf{Remark 1.4 (Convergence analysis):} Suppose we have a good initial point, such that $p$ can be as large as $1$, which means that $\overline{\bfW}(p_{\max})$ can be $\bfW^*$ from Remark 1.3. However, with a small $N$ such that $N\ll K^3d$,  the iterates cannot guarantee to be arbitrarily close to $\overline{\bfW}(p_{\max})$, either. 
First, $\w[\nu]$ needs to be at least less than $1$ to gaurantee the outer loop can converge from \eqref{eqn: p_convergence}. Then, 
we know that $\frac{\w[\lambda]\de^2}{\lambda\delta^2+\w[\lambda]\de^2}$ needs to be smaller than $\Theta(\mu^{-1})$ from \eqref{eqn: nu_tilde}. However, it is equivalent to require $\frac{\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2}$ in the order of $1- \mathcal{O}(\mu^{-1})$, which contracts the statement in Theorem \ref{Thm: p_convergence} given $N\ll {K^3d}$. The details about analysis with $N=\Omega({K^3d})$ will be discussed in the following paragraphs.
}

\iffalse
\noindent
\tcr{\textbf{Remark 1.1 (Influence of $M$):} Since $\varepsilon$ can only be as large as a constant, it is clear that $\frac{\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2} = \mathcal{O}\big(\mu\sqrt{\frac{N}{K^3d}}\big)$ from \eqref{eqn: p_main_sample}, and $\frac{\w[\lambda]\de^2}{\lambda\delta^2+\w[\lambda]\de^2}$ needs to be in the order of $1-\mathcal{O}\big(\mu\sqrt{\frac{N}{K^3d}}\big)$. 
When $N\ll K^3d$, we know that $1-\mathcal{O}\big(\mu\sqrt{\frac{N}{K^3d}}\big)$ is lower-bounded and close to $1$. Therefore, with fixed $N$, if $M$ decreases, $\w[\varepsilon]$  will increase while $\w[\lambda]$ needs to stay the same. From \eqref{eqn: nu_tilde}, we know that $\w[\nu]$ will increase accordingly, and thus the error term in  \eqref{eqn: p_convergence} will increase as well. Conversely, if we increase $M$, we can obtain smaller error bound, and $\W[T]$ is closer to $\overline{\bfW}(p)$ and $\bfW^*$.}


\noindent
\tcr{\textbf{Remark (Parameter $p$):} From \eqref{eqn: p_initialization} and \eqref{eqn: p_convergence}, we know that the best convergent point, where in terms of the distance to $\bfW^*$, returned by gradient descent method is $\overline{\bfW}(p_{\max})$, where $p_{\max}$ is the maximum value of $p$ while \eqref{eqn: p_initial_sample} still holds.
When $N = \Omega(\mu^{-4}K^3d\log q)$, $p$ can be as large as $1$, which suggests that $\overline{\bfW}$ can be $\bfW^*$. However, when $N$ is small, we have $p_{\max}=\Theta(\mu^2\sqrt{\frac{N}{K^3d}})$. Given a fixed initial point $\bfW^{(0)}$, The achievable weights with the smallest distance to $\bfW^*$ are $\overline{\bfW}(p_{\max})$. Also, with larger $N$, $\overline{\bfW}(p_{\max})$ is closer to $\bfW^*$.
However, even we have a good initial point, such that $p$ can be $1$. With small $N$,  the iterates cannot guarantee to be arbitrarily close to $\overline{\bfW}(p_{\max})$, either. 
To guarantee that $\w[\nu]$ is less than $1$ and thus the outer loop can converge, we know that $\frac{\w[\lambda]\de^2}{\lambda\delta^2+\w[\lambda]\de^2}$ needs to be smaller than $\Theta(\mu)$ from \eqref{eqn: p_main_sample} and  \eqref{eqn: p_convergence}. However, it is equivalent to require $\frac{\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2}$ in the order of $1- \mathcal{\mu}$, which is a constant and $N$ still needs to be in the order of $K^3d\log q$.
}
\fi

==> Self-training (6)/Thm1_wrong.tex <==
\newpage
\section{Theoretical results: insufficient sample complexity}
\begin{theorem}
    
    Suppose the initial point $\W[0, 0]$ satisfies 
    \begin{equation}\label{eqn: p_initial_point}
        \|\bfW^* -\W[0,0] \| = \mathcal{O}\big( \frac{\mu^2\sigma_K}{p^2 K} \big)  \text{ for some $p\in(0,1]$}.
    \end{equation}
    Then, if the following conditions 
    \begin{equation}\label{eqn: p_condition1}
    \nu_1\cdot(1-p)+\w[\nu]_1\cdot p < 1,    
    \end{equation}
    \begin{equation}\label{eqn: p_main_sample}
    \begin{split}
        &N= \Omega\Big( \varepsilon^{-2}\mu^{-2}\big(\frac{\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2}\big)^2K^3 d\log q \Big),\\
        \end{split}
    \end{equation}
    \begin{equation}\label{eqn: p_main_sample_M}
        \begin{split}
        \text{and}&\quad 
        M= \Omega\Big(\tilde{\varepsilon}^{-2}\mu^{-2}\big(\frac{\w[\lambda]\de^2}{\lambda\delta^2+\w[\lambda]\de^2}\big)^2 K^3 d\log q\Big).
        \end{split}
    \end{equation}
    hold
    for some constant $\varepsilon$, $\w[\varepsilon]\in (0, \frac{1}{2})$,
    we have
    \begin{equation}
        \lim_{\ell\to \infty, t\to \infty} \| \W[\ell,t]-\overline{\bfW}(p) \|_F \le \frac{1}{1-\varepsilon-\w[\varepsilon]}\cdot \frac{\nu_1 (1-p)}{\nu_1 (1-p) + \w[\nu]_1 p } \|\bfW^* -\W[0,0]\|_F
    \end{equation}
    with probability at least $1-q^{-d}$, 
    where
    \begin{equation}\label{eqn: mu}
        \mu
        = \mu( \delta, \de) 
        = \frac{\lambda\rho(\delta)+\w[\lambda]\rho(\de)}{\lambda\delta^2+\w[\lambda]\de^2},
    \end{equation}
    \begin{equation}\label{eqn: nu1}
        \nu_1 = \Theta\Big(\frac{\lambda\delta^2}{\mu(\lambda\delta^2+\w[\lambda]\de^2)}\Big) + \frac{\varepsilon}{ K},
    \end{equation}
    \begin{equation}\label{eqn: nu1_tilde}
        \text{and \quad} \w[\nu]_1 = \Theta\Big(\frac{\w[\lambda]\de^2}{\mu(\lambda\delta^2+\w[\lambda]\de^2)}\Big) + \frac{\w[\varepsilon]}{ K}.
    \end{equation}
\end{theorem}

\noindent
\textbf{Remark 1 (Conditions for \eqref{eqn: p_condition1}):} Since $\varepsilon$ can only be as large as a constant, it is clear that $\frac{\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2} = \mathcal{O}\big(\mu\sqrt{\frac{N}{K^3d}}\big)$ from \eqref{eqn: p_main_sample}. When $N\ll K^3d$, we know $\frac{\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2}$ is a small positive constant, and $\frac{\w[\lambda]\de^2}{\lambda\delta^2+\w[\lambda]\de^2}$ is close to $1$. Therefore, we have $\w[\nu]_1\in\Theta(\mu^{-1})$, and $p$ needs to be less than $\mu$ in order to guarantee $\w[\nu]_1 p $ is small and thus \eqref{eqn: p_condition1} holds. Therefore, even we are given a good initial point such that $p$ can be $1$ in \eqref{eqn: p_initial_point}, without enough samples in $\mathcal{D}$, we cannot guarantee the algorithm converges to $\overline{\bfW}(1)$, which is actually the ground truth $\bfW^*$, but $\overline{\bfW}(\mu)$ at best (w.r.t the distance to the ground truth).

\noindent
\textbf{Remark 2 (Influence of $M$):} 

==> Self-training (6)/Thm2.tex <==
\begin{theorem}\label{Thm: sufficient_number}
    Suppose $\bfW^{(0)}$ satisfies \eqref{eqn: p_initialization} with $p=1$ and the number of samples in $\mathcal{D}$ and $\w[\mathcal{D}]$ satisfy
    \begin{equation}\label{eqn:main_sample}
    \begin{split}
        &N= \Omega\big( \mu^{2}\hat{\lambda}^2K^3 d\log q \big),
        \quad
        \text{and}\quad 
        M= \Omega\big(\mu^{2}(1-\hat{\lambda})^2 K^3 d\log q\big).
        \end{split}
    \end{equation}
     where
    \begin{equation}\label{eqn: lambda_hat_s}
        \hat{\lambda} : =\frac{\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2}
        = 1 - \mathcal{O}\big(\frac{1}{\mu\sqrt{K}}\big). 
    \end{equation}
    Then, the iterates $\{ \bfW^{(\ell,t)} \}_{\ell=1, t=1}^{L, T}$ converge to the ground truth as 
    \begin{equation}\label{eqn: convergence}
        \| \W[L,T] -\bfW^* \|_F \le \big( \nu_1^T(\beta) + \nu_2 \big)^L 
        \| \W[0,0]-\bfW^* \|_F,
    \end{equation}
    where 
    \begin{equation}\label{eqn: convergence_rate}
    \begin{split}
        &\nu_1(\beta^*) = 1- \Theta
        \Big(
        \frac{1-\Theta(\frac{\hat{\lambda}}{\sqrt{N}})-\Theta(\frac{1-\hat{\lambda}}{\sqrt{M}})}{\mu\sqrt{K}} 
        \Big),\\
        % \nu_2 = \Theta\Big( \frac{\w[\varepsilon]\mu}{\sqrt{K}}\Big) + \Theta\Big( \frac{\w[\lambda]\de^2}{\lambda\delta^2+\w[\lambda]\de^2} \Big).
        &\tcr{\nu_2 =  \Theta\Big(1+\Theta\big(\frac{\hat{\lambda}}{\sqrt{N}}\big)+\Theta\big(\frac{1-\hat{\lambda}}{\sqrt{M}}\big)\Big)\cdot\mu\sqrt{K}(1-\hat{\lambda}).}
    \end{split}
    \end{equation}
\end{theorem}

Theorem \ref{Thm: sufficient_number} indicates that the iterates returned by Algorithm \ref{Algorithm: Alg1} converge to the ground truth $\bfW^*$ with exponential decay as long as the number of samples satisfy \eqref{eqn:main_sample} with $\hat{\lambda}$ meeting \eqref{eqn: lambda_hat_s}. The linear convergence rates of the inner loop and outer loop are denoted as $\nu_1$ and $\nu_2$ as shown in \eqref{eqn: convergence_rate}.
\\
\noindent
\textbf{Remark 2.1 (Parameter $N$):}
Suppose we do not have unlabeled data, which is equivalent to say that $\hat{\lambda} =1$, the required number of samples are in the order of $\mu^{2}K^3d \log q$.  Therefore, the sample complexity of $N$ can be reduced by a factor of $\hat{\lambda}$ at the cost of a slower convergence rate, where $\nu_1$ in \eqref{eqn: convergence_rate} has an additional factor of $\frac{1-\hat{\lambda}}{\sqrt{M}}$ and $\nu_2$ is non-zero as $\hat{\lambda}$ is less than $1$ compared with training without unlabeled data.  

\noindent
\textbf{Remark 2.2 (Convergence rate $\nu_1$ and $\nu_2$):} 
From \eqref{eqn: convergence_rate}, we know that both the convergence rates decrease, which indicates a faster convergence rate, if either $N$ or $M$ increases. While if  $\mu$ increases, both the values of $\nu_1$ and $\nu_2$ will increase, which suggests a slower convergence rate.
Additionally, given $N$ and $M$ are in the same order as shown in \eqref{eqn:main_sample}, only $\nu_2$ depends on $\hat{\lambda}$ and is a negative function of $\hat{\lambda}$. Therefore, if we increase the value of $\hat{\lambda}$, algorithms will enjoy a faster convergence rate, however, which also suggests a larger number of labeled data $N$. 
 
\iffalse
\noindent
\textbf{Remark 2.1 (Range of $\lambda$):} From \eqref{eqn: convergence}, we know that $\nu_2$ needs to be less than $1$ in order to guarantee the convergence to $\bfW^*$. Therefore, $\w[\lambda]=\mathcal{O}(\mu^{-1}K^{-1/2})$ and $\lambda=1-\mathcal{O}(\mu^{-1}K^{-1/2} )$.

\noindent
\textbf{Remark 2.2 (Influence of $M$ and $N$):}  Suppose we do not have unlabeled data, which is equivalent to say that $\w[\lambda] =0$, the required number of samples are in the order of $\varepsilon^{-2}\mu^{-2}K^3d \log q$ with $\varepsilon\in(0,1)$. When we are accessible to infinite number of unlabeled samples, where $\w[\varepsilon]$ can be arbitrary close to $0$, the sample complexity of $N$ is reduced by a factor of $\big(\frac{\lambda\delta^2}{\lambda\delta^2 + \w[\lambda] \de^2}\big)^2$ with $\varepsilon\in(0,1)$. From another point of view, with fixed $\de$, $\varepsilon$ and $\w[\varepsilon]$ are in the order of $\frac{1}{\sqrt{N}}$ and $\frac{1}{\sqrt{M}}$. Thus, increase the value of $M$  or $N$ will lead to the decrease of $\nu_1$ and $\nu_2$ and thus faster convergence rate.



\noindent
\textbf{Remark 2.3 (Influence of $\de$):} The value of $\de$ will directly control the values of $\varepsilon$, $\w[\varepsilon]$ and $\nu$, and thus the sample complexity and convergence rate are affected. When $\de$ and $\delta$ are fixed or relative small,  $\mu$ is a fixed constant. 
With fixed finite number of samples $M$ and $N$, $\varepsilon$ and $\w[\varepsilon]$ are in the order of  $\frac{\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2}$ and $\frac{\w[\lambda]\de^2}{\lambda\delta^2+\w[\lambda]\de^2}$, respectively. Hence, changing the value of $\de$ will not affect the sum of $\varepsilon$ and $\w[\varepsilon]$, and the convergence rate of the inner loop $\nu_1$ stays the same as well. On contrast, the value of $\nu_2$ decreases as $\de$ decreases, thus the convergence rate of the outer loop, which is $\nu_1^T+\nu_2$, will become faster if we decrease the value of $\de$. However, $T$ is usually a relatively small number in training \tcr{(citation)}, and thus the value of $\nu_1$ plays a more important role in determining the convergence rate of the outer loop. Thus, decreasing the value of $\de$ when $\de$ is already close to $0$ will only increase the convergence rate of the outer loop slightly. Moreover, suppose we have the infinite number of unlabeled data, that is $M$ is sufficiently large, and $\w[\varepsilon]$ can be arbitrarily close to $0$. Decreasing the value of $\de$ will lead to the higher requirement on the sample complexity of labeled data $N$ with $\varepsilon\in(0,1)$. 
\fi

==> Self-training (6)/Thm2_old.tex <==
\section{Theoretical results: sufficient number of samples}
\subsection{Local convex region}
\begin{equation}\label{eqn: initialization}
    \|\bfW-\bfW^*\|_F\lesssim \frac{\sigma_K}{\mu^2 K}
\end{equation}
\tcr{\begin{lemma}[Initialization]\label{Thm: initialization}
    Assume  the number of samples $N = \Omega\big( \mu^{4} K^3 d \log  q \big)$ for some large constant $q$, the tensor initialization method 
    outputs  $\bfW^{(0,0)}$  such that \eqref{eqn: initialization} holds, i.e., $\| \bfW^{(0,0)} -\bfW^* \|_F  = \mathcal{O}\big(\frac{\sigma_K}{\mu^2K}\big)$ with probability at least $1-q^{-d}$.
%	\end{equation}
\end{lemma}}


\subsection{Convergence analysis}
\begin{theorem}\label{Thm: sufficient_number}
    Suppose $\bfW^{(0)}$ satisfies \eqref{eqn: initialization} and the number of samples in $\mathcal{D}$ and $\w[\mathcal{D}]$ satisfy
    \begin{equation}\label{eqn:main_sample}
    \begin{split}
        &N= \Omega\big( \varepsilon^{-2}\mu^{2}\hat{\lambda}^2K^3 d\log q \big),\\
        \end{split}
    \end{equation}
    \tcr{\begin{equation}
        \begin{split}
        \text{and}&\quad 
        M= \Omega\big(\tilde{\varepsilon}^{-2}\mu^{2}(1-\hat{\lambda})^2 K^3 d\log q\big).
        \end{split}
    \end{equation}}
    for some constant $\varepsilon$, $\w[\varepsilon]>0$ with $\varepsilon+\w[\varepsilon]<1$.
    Then, the iterates $\{ \bfW^{(\ell,t)} \}_{\ell=1, t=1}^{L, T}$ converge to the ground truth as 
    \begin{equation}\label{eqn: convergence}
        \| \W[L,T] -\bfW^* \|_F \le \big( \nu_1^T(\beta) + \nu_2 \big)^L 
        \| \W[0,0]-\bfW^* \|_F,
    \end{equation}
    where 
    \begin{equation}
    \begin{split}
        &\nu_1(\beta^*) = 1- \Theta
        \Big(
        \frac{1-\varepsilon-\w[\varepsilon]}{\mu\sqrt{K}} 
        \Big),
        \text{and}\quad
        % \nu_2 = \Theta\Big( \frac{\w[\varepsilon]\mu}{\sqrt{K}}\Big) + \Theta\Big( \frac{\w[\lambda]\de^2}{\lambda\delta^2+\w[\lambda]\de^2} \Big).
        \tcr{\nu_2 =  \Theta\Big(\frac{\mu\sqrt{K} \hat{\lambda}}{1-\varepsilon-\tilde{\varepsilon}}\Big).}
    \end{split}
    \end{equation}
\end{theorem}
\noindent
\textbf{Remark 2.1 (Range of $\lambda$):} From \eqref{eqn: convergence}, we know that $\nu_2$ needs to be less than $1$ in order to guarantee the convergence to $\bfW^*$. Therefore, $\w[\lambda]=\mathcal{O}(\mu^{-1}K^{-1/2})$ and $\lambda=1-\mathcal{O}(\mu^{-1}K^{-1/2} )$.

\noindent
\textbf{Remark 2.2 (Influence of $M$ and $N$):}  Suppose we do not have unlabeled data, which is equivalent to say that $\w[\lambda] =0$, the required number of samples are in the order of $\varepsilon^{-2}\mu^{-2}K^3d \log q$ with $\varepsilon\in(0,1)$. When we are accessible to infinite number of unlabeled samples, where $\w[\varepsilon]$ can be arbitrary close to $0$, the sample complexity of $N$ is reduced by a factor of $\big(\frac{\lambda\delta^2}{\lambda\delta^2 + \w[\lambda] \de^2}\big)^2$ with $\varepsilon\in(0,1)$. From another point of view, with fixed $\de$, $\varepsilon$ and $\w[\varepsilon]$ are in the order of $\frac{1}{\sqrt{N}}$ and $\frac{1}{\sqrt{M}}$. Thus, increase the value of $M$  or $N$ will lead to the decrease of $\nu_1$ and $\nu_2$ and thus faster convergence rate.



\noindent
\textbf{Remark 2.3 (Influence of $\de$):} The value of $\de$ will directly control the values of $\varepsilon$, $\w[\varepsilon]$ and $\nu$, and thus the sample complexity and convergence rate are affected. When $\de$ and $\delta$ are fixed or relative small,  $\mu$ is a fixed constant. 
With fixed finite number of samples $M$ and $N$, $\varepsilon$ and $\w[\varepsilon]$ are in the order of  $\frac{\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2}$ and $\frac{\w[\lambda]\de^2}{\lambda\delta^2+\w[\lambda]\de^2}$, respectively. Hence, changing the value of $\de$ will not affect the sum of $\varepsilon$ and $\w[\varepsilon]$, and the convergence rate of the inner loop $\nu_1$ stays the same as well. On contrast, the value of $\nu_2$ decreases as $\de$ decreases, thus the convergence rate of the outer loop, which is $\nu_1^T+\nu_2$, will become faster if we decrease the value of $\de$. However, $T$ is usually a relatively small number in training \tcr{(citation)}, and thus the value of $\nu_1$ plays a more important role in determining the convergence rate of the outer loop. Thus, decreasing the value of $\de$ when $\de$ is already close to $0$ will only increase the convergence rate of the outer loop slightly. Moreover, suppose we have the infinite number of unlabeled data, that is $M$ is sufficiently large, and $\w[\varepsilon]$ can be arbitrarily close to $0$. Decreasing the value of $\de$ will lead to the higher requirement on the sample complexity of labeled data $N$ with $\varepsilon\in(0,1)$. 

==> Self-training (6)/algorithm.tex <==
\subsection{Algorithm}\label{sec: algorithm}
We consider an iterative self-training method such as \citep{Lee13}, which can be divided into   steps: 



\begin{enumerate}
    \item Initial $\ell =0$ and obtain a  model $\W[\ell]$, denoted as the teacher model,   using labeled data $\mathcal{D}$ only;
%\noindent   For $\ell = 0 , 1, \cdots, L-1$
    \item Use the teacher model    to calculate  pseudo labels $\w[y]_m$ of unlabeled data in $\w[\mathcal{D}]$. %=\{\w[\bfx]_m \}_{m=1}^M$. 
    \item Train the neural network by solving (\ref{eqn: empirical_risk_function}) %via minimizing the objective function as shown in \eqref{eqn: empirical_risk_function} 
    via $T$-step  mini-batch stochastic gradient descent method using disjoint subsets $\{\mathcal{D}_t\}_{t=0}^{T-1}$ and $\{\widetilde{\mathcal{D}}_t\}_{t=0}^{T-1}$. Let $\W[\ell]$ denote the obtained student model. 
    \item Use $\W[\ell]$ as the current teacher model. Let $\ell=\ell+1$ and go back to step 2.
\end{enumerate}
The pseudocode of the self-training method is summarized in Algorithm
\ref{Algorithm: Alg1}.
\begin{algorithm}[h]
	\caption{Mini-batch stochastic gradient Descent Algorithm}\label{Algorithm: Alg1}
	\begin{algorithmic}
		\State \textbf{Input:} labeled $\mathcal{D}=\{(\bfx_n, y_n) \}_{n=1}^{N}$,  
		 unlabeled data $\w[\mathcal{D}]=\{\widetilde{\bfx}_m \}_{m=1}^{M}$,
		gradient step size $\eta$;
		\State \textbf{Initialization:} preliminary teacher model with weights $\bfW^{(0)}$;
		\State \textbf{Partition:} divide $\mathcal{D}$ and $\widetilde{\mathcal{D}}$ into $T$ disjoint subsets $\{ \mathcal{D}_t \}_{t=0}^{T-1}$ and $\{\widetilde{\mathcal{D}}_t\}_{t = 0}^{T-1}$, respectively; \For{$\ell = 0 , 1, \cdots, L-1$}
		    \State 1. Use the estimated teacher model $\bfW^{(\ell)}$ to generate pseudo labels for $\{\widetilde{\bfx}_m\}_{m=1}^M$:
		    \State \qquad $y_m = g(\bfW^{(\ell)};\w[\bfx]_m)$ for $m =1, 2, \cdots, M$;
		    \State 2. Obtain the student model ${\bfW}$ through minimizing \eqref{eqn: empirical_risk_function} via  mini-batch stochastic gradient descent method using $\mathcal{D}_t$ and $\widetilde{\mathcal{D}}_t$;
		    \State 3. Update the new teacher model  as the obtained student model: \qquad $\bfW^{(\ell+1)} = \bfW$;
		 \EndFor
	\end{algorithmic}
\end{algorithm}


==> Self-training (6)/problem_formulation.tex <==
\section{Formalizing {Self-Training}: Notation, Formulation, and Algorithm}\label{sec: problem}

% \paragraph{Notations.} \SL{Introduction key definitions and notations here. A notation table would help a lot. }

% \paragraph{\SL{Problem formulation.}}

% \paragraph{\SL{Algorithmic framework of self-training.}}

\textbf{Problem formulation.} %We consider the labeled data $(\bfx,y)$ from distribution $P_{l}$ and unlabeled data $\widetilde{\bfx}$ from distribution $P_{u}$. \tcr{Consequently, a neural network $g(\bfW)$ with weights $\bfW$ is defined as a mapping from the input $\bfx$ (or $\w[\bfx]$) to the output $g(\bfW;\bfx)$ (or $g(\bfW;\w[\bfx])$).}
Given $N$ labeled data sampled from distribution $P_{l}$, denoted by $\mathcal{D} = \{ \bfx_n, y_n\}_{n=1}^N$, and $M$ unlabeled data drawn from distribution $P_{u}$, denoted by $\widetilde{\mathcal{D}} = \{ \widetilde{\bfx}_m \}_{m=1}^M$. The \Revise{aim} is to find a neural network model $g(\bfW)$, where $\bfW$ denotes the trainable weights, that minimizes the testing error on data sampled from $P_{l}$. % the iterative self-training approach aims to find a student model $g(\bfW_S)$ with small 
%test error on the data from $P_{l}$, which is also known as the generalization error.   
% At the end, important notations are summarized in Table \ref{table:problem_formulation} for the convenience of reading.
% \begin{table}[h]
%     \centering
%     \vspace{-3mm}
%     \begin{tabular}{p{0.8cm}|p{5.7cm}||p{1.2cm}|p{5.5cm}}
%     \hline
%     \hline
%     $\mathcal{D}/\w[\mathcal{D}]$ & labeled/unlabeled dataset    
%     & $N/M$ & number of labeled/unlabeled data\\
%     \hline
%     $(\bfx,y)$ & input of labeled data $\bfx$ and corresponding label $y$    
%     & $(\w[\bfx],\w[y])$ & input of unlabeled data $\w[\bfx]$ and calculated pseudo-label $\w[y]$\\
%     \hline
%     $d$ & dimension of the input
%     &$K$  & number of neurons in the hidden layer\\
%     \hline
%     $g(\bfW)$ & neural network $g$ with weights $\bfW$ in \eqref{eqn: teacher_model}
%     &$g(\bfW;\bfx)$  & output of $g(\bfW)$ w.r.t input $\bfx$\\
%     \hline
%     $f_{\mathcal{D},\w[\mathcal{D}]}$ & objective function in \eqref{eqn: empirical_risk_function}
%     &$I(g(\bfW))$  & the value of generalization error in \eqref{eqn: GF}\\
%     \hline
%     \hline
%     \end{tabular}
%     \vspace{-1mm}
%     \caption{Notations related to the problem formulation.}   
%     \label{table:problem_formulation}
%     \vspace{-3mm}
% \end{table}
%\fbox{\begin{minipage}{42em}
%		\begin{itemize}
%			\item (S1) Initialize {iteration} $\ell =0$ and obtain a model $\W[\ell]$ as the teacher  using labeled data $\mathcal{D}$ only;
%			%\noindent   For $\ell = 0 , 1, \cdots, L-1$
%			
%			\item (S2) Use the teacher model  to obtain  pseudo labels $\w[y]_m$ of unlabeled data in $\w[\mathcal{D}]$; %=\{\w[\bfx]_m \}_{m=1}^M$; 
%			
%			\item (S3) Train the neural network  by minimizing (\ref{eqn: empirical_risk_function}) %via minimizing the objective function as shown in \eqref{eqn: empirical_risk_function} 
%			via $T$-step  mini-batch gradient descent method using disjoint subsets $\{\mathcal{D}_t\}_{t=0}^{T-1}$ and $\{\widetilde{\mathcal{D}}_t\}_{t=0}^{T-1}$ of $\w[\mathcal{D}]$. Let $\W[\ell+1]$ denote the obtained student model; 
%			
%			\item (S4) Use $\W[\ell+1]$ as the current teacher model. Let $\ell \leftarrow \ell+1$ and go back to step (S2);
%			
%		\end{itemize}
%		
%\end{minipage}}
\begin{mybox}[colback=mygray]{\textcolor{black}{Table 1: Iterative Self-Training}}
{%\small 
(S1) Initialize {iteration} $\ell =0$ and obtain a model $\W[\ell]$ as the teacher  using labeled data $\mathcal{D}$ only;
%\noindent   For $\ell = 0 , 1, \cdots, L-1$
    
    (S2) Use the teacher model  to obtain  pseudo labels $\w[y]_m$ of unlabeled data in $\w[\mathcal{D}]$; %=\{\w[\bfx]_m \}_{m=1}^M$; 
    
    (S3) Train the neural network  by minimizing (\ref{eqn: empirical_risk_function}) %via minimizing the objective function as shown in \eqref{eqn: empirical_risk_function} 
    via $T$-step  mini-batch gradient descent method using disjoint subsets $\{\mathcal{D}_t\}_{t=0}^{T-1}$ and $\{\widetilde{\mathcal{D}}_t\}_{t=0}^{T-1}$ of $\w[\mathcal{D}]$. Let $\W[\ell+1]$ denote the obtained student model; 
    
    (S4) Use $\W[\ell+1]$ as the current teacher model. Let $\ell \leftarrow \ell+1$ and go back to step (S2);}
\end{mybox}

\textbf{Iterative self-training.} In each iteration, given the current teacher predictor $g(\W[\ell])$, % with weights $\W[\ell]$, 
the pseudo-labels for the unlabeled data in $\w[\mathcal{D}]$ are computed as $\tilde{y}_m = g(\W[\ell];\w[\bfx]_m)$. %Then, the weights of the student model $\W[\ell+1]$ is obtained via minimizing the objective function of the mixture of labeled and unlabeled data, denoted as
The method then minimizes  the weighted empirical risk  $\hat{f}_{\mathcal{D},\w[\mathcal{D}]}(\bfW)$
%\footnote{\Revise{The result is extendable to binary classification equipped with cross-entropy loss function. See Appendix for details.}}
of both labeled and unlabeled data through stochastic gradient descent, where
\begin{equation}\label{eqn: empirical_risk_function}
\vspace{-1mm}
    \hat{f}_{\mathcal{D},\w[\mathcal{D}]}(\bfW) = \frac{\lambda}{2N}\sum_{n=1}^N\big(y_n - g(\bfW;\bfx_n) \big)^2 + \frac{\w[\lambda]}{2M}\sum_{m=1}^M \big(\w[y]_m - g(\bfW;\w[\bfx]_m) \big)^2, 
\end{equation}
and $\lambda+\w[\lambda]= 1$. The learned student model $g(\W[\ell+1])$   is used as the teacher model in the next iteration. The initial model $g(\W[0])$ is learned from labeled data. 
%Finally, we replace the teacher model as the obtained student $\bfW_S$ and iterate the steps above multiple times. 
The formal algorithm is summarized as in Table 1.  %in the following block:




% \fcolorbox{black}{mygray}
% {\begin{minipage}{0.97\linewidth}
%     (S1) Initial $\ell =0$ and obtain a  model $\W[\ell]$, denoted as the teacher model,   using labeled data $\mathcal{D}$ only;
% %\noindent   For $\ell = 0 , 1, \cdots, L-1$
    
%     (S2) Use the teacher model    to calculate  pseudo labels $\w[y]_m$ of unlabeled data in $\w[\mathcal{D}]$; %=\{\w[\bfx]_m \}_{m=1}^M$; 
    
%     (S3) Train the neural network by solving (\ref{eqn: empirical_risk_function}) %via minimizing the objective function as shown in \eqref{eqn: empirical_risk_function} 
%     via $T$-step  mini-batch stochastic gradient descent method using disjoint subsets $\{\mathcal{D}_t\}_{t=0}^{T-1}$ and $\{\widetilde{\mathcal{D}}_t\}_{t=0}^{T-1}$. Let $\W[\ell+1]$ denote the obtained student model; 
    
%     (S4) Use $\W[\ell+1]$ as the current teacher model. Let $\ell=\ell+1$ and go back to step (S2);
% \end{minipage}}

\textbf{Model and assumptions.} %In this paper, %we study the case that the neural network $g$ can be presented by a 
This paper considers regression\footnote{\Revise{The results can be extended to binary classification with a cross-entropy loss function. Please see Appendix-I.}}, where $g$ is a one-hidden-layer fully connected neural network equipped with $K$ neurons. Namely, given the input $\bfx\in\mathbb{R}^d$ and weights $\bfW = [\bfw_1, \bfw_2, \cdots, \bfw_K]\in \mathbb{R}^{d\times K}$, we have
\vspace{-2mm}
\begin{equation}\label{eqn: teacher_model}
\vspace{-2mm}
    g(\bfW;\bfx) : = \frac{1}{K}\sum_{j=1}^K \phi(\bfw_j^{T}\bfx),
\end{equation}
where $\phi$ is the ReLU activation function\footnote{\Revise{Because  ReLU  is non-linear and non-smooth,  \eqref{eqn: empirical_risk_function} is  non-convex  and non-smooth, which poses analytical challenges. The results can be easily extended to smooth functions with bounded gradients, e.g., Sigmoid.}},  %  of the objective function are the major challenges in landscape analysis, which are directly derived from the fact that ReLU function is non-linear and non-smooth. In particular, the results can be reduced to smooth functions with bounded gradient, e.g., sigmoid, logistic.}},  
and $\phi(z) = \max\{ z, 0 \}$ for any input $z\in \R$. \Revise{Here, we fix the top layer weights as $1$ for simplicity, and   %one check its 
the equivalence  of such a simplification %to %the case that the top layer is not fixed 
is discussed in Appendix \ref{sec: two_layer}.}
%\tcb{Although this paper focuses on regression, the results can be directly extended to binary classification with cross-entropy loss function. Please see Appendix-I for details.}


Moreover, we assume an unknown ground-truth model with weights $\bfW^*$ that maps all the features to the corresponding labels drawn from $P_l$, i.e., $y = g(\bfW^*;\bfx)$, where $(\bfx, y)\sim P_l$. 
%In addition, the labeled data $(\bfx, y)$ from $P_l$ are assumed to be learned by some unknown ground truth weights $\bfW^*$ of the network $g$, namely, $y = g(\bfW^*;\bfx)$. Consequently, 
The generalization function (GF) with respect to $g(\bfW)$  is defined as 
\vspace{-1mm}
\begin{equation}\label{eqn: GF}
\vspace{-1mm}
    I\big(g(\bfW)\big) = \mathbb{E}_{(\bfx, y)\sim P_l }\big(y - g(\bfW;\bfx)\big)^2 = \mathbb{E}_{(\bfx, y)\sim P_l }\big( g(\bfW^*;\bfx) - g(\bfW;\bfx)\big)^2.
\end{equation}
%One can easily check that $g(\bfW^*)$ is the global optimal to the 
By definition $I\big(g(\bfW^*)\big)$ is zero. 
Clearly, $\bfW^*$ is not unique because any column permutation of $\bfW^*$, which corresponds to permuting neurons, represents the same function as $\bfW^*$ and minimizes GF
% \PY{(did we define GF?)} 
in \eqref{eqn: GF} too. To simplify the representation, we follow the convention and abuse the notation that %$\bfW^*$ stands for any equivalent permutation of the value of $\bfW^*$ and  
the distance from $\bfW$ to $\bfW^*$, denoted by  $\|\bfW-\bfW^*\|_F$, means the smallest distance from $\bfW$ to any permutation of $\bfW^*$.  Additionally, some important notations are summarized in Table \ref{table:problem_formulation}.
% \tcr{Here, we use the convention that $\bfW^*$ stands for any equalavent permutation of the value of $\bfW^*$ in the neural network $g$, and the distance to $\bfW^*$ is the smallest one among all the equalavent permutations.}
%Moreover, for activation functions with bounded gradient, such as linear, ReLU, sigmoid, and logistic, the generalization error is upper bounded by the distance of $\bfW$ and $\bfW^*$ with an extra constant factor.
% Let $\bfw_j^*\in\mathbb{R}^d$ denote the ground truth weights vector for the $j$-th neuron, and $\bfW^* = [\bfw_1^*, \bfw_2^*, \cdots, \bfw_K^*]\in \mathbb{R}^{d\times K}$. 
% Then, the labeled data in $\mathcal{D}$ satisfies 
% \begin{equation}\label{eqn: teacher_model}
%     y_n= g(\bfW^*;\bfx_n) : = \frac{1}{K}\sum_{k=1}^K \phi(\bfw_j^{*T}\bfx_n),
% \end{equation}
% where $\phi$ is the activation function.

We assume the inputs of both the labeled and unlabeled data belong to the zero mean Gaussian distribution,  % however, the variances can be different. 
i.e., $\bfx \sim\mathcal{N}(0, \delta^2\bfI_{d})$, and $\w[\bfx]\sim \mathcal{N}(0, \de^2\bfI_d)$.  
{The Gaussian assumption is motivated by the data whitening \citep{LBOM12} and batch normalization techniques \citep{IS15} that are commonly used in practice to improve learning performance. %On top of the motivation, 
Moreover, training one-hidden-layer neural network with multiple neurons is NP-Complete \citep{BR92} without any  assumption.}
%At the end, 
% \PY{(Need to add some sentences discussing why this assumption is needed (cite recent papers, and why extending it is difficult - we can use similar argument from our NeurIPS rebuttal))}
% Some important notations are summarized in Table \ref{table:problem_formulation}. % for the convenience of reading.
%The activation function $\phi$ is ReLU, where $\phi(z) = \max\{ z, 0 \}$ for any 
%input $z\in \R$. 
 
\textbf{The focus of this paper.} %This paper aims to answering the following questions: (1) characterization of the convergent point $\W[L]$ with respect to the initial teacher model $\bfW^{(0)}$ and the ground truth $\bfW^*$; (2) how unlabeled data affect the convergence and generalization of $\W[L]$.
This paper will analyze three aspects about self-training:  
(1) the generalization performance of $\W[L]$, the returned model by self-training after $L$ iterations, measured by $\|\W[L]-\bfW^*\|_F$\footnote{We use this metric because  $I\big(g(\bfW)\big)$ is shown to be linear in $\|\W[L]-\bfW^*\|_F$ numerically when $\W[L]$ is close to  $\bfW^*$, see Figure \ref{fig:GF_1M}.}; (2) \Revise{the influence of parameter $\lambda$ in \eqref{eqn: empirical_risk_function} on the training performance;} and (3) the impact of unlabeled data on the training and generalization performance.
\AtBeginEnvironment{tabular}{\small}
\setcounter{table}{1}
\begin{table}[h]
    \centering
    \vspace{-2mm}
    \caption{Some Important Notations}
    \vspace{-2mm}
    \begin{tabular}{c|p{11cm}}
    \hline
    \hline
    $\mathcal{D} =\{ \bfx_n, \bfy_n \}_{n=1}^N$ & Labeled dataset with $N$  number of samples;\\
    \hline
    $\widetilde{\mathcal{D}} =\{ \widetilde{\bfx}_m \}_{m=1}^M$ & Unlabeled dataset with $M$  number of samples;\\
    \hline
    $d$ & Dimension of the input $\bfx$ or $\widetilde{\bfx};$
    \\
    \hline
    $K$ & Number of neurons in the hidden layer;
    \\
    \hline
    $\kappa$ & Conditional number (the ratio of the largest and smallest singular values) of $\bfW^*$;
    \\
    \hline
    $\W[\ell]$ & Model returned by self-training after $\ell$ iterations; $\W[0]$ is the initial model;\\
    \hline
    $\bfW^*$ & Weights of the ground truth model;\\
    \hline
    $\WL$ & $\WL = \hat{\lambda} \bfW^* + (1-\hat{\lambda})\W[0]$;\\
    \hline
    \hline
    \end{tabular}
    \label{table:problem_formulation}
    \vspace{-4mm}
\end{table}

\iffalse
\textbf{Comparison with   supervised learning and the focus of this paper.}
As existing work for supervised learning problems \citep{ZSJB17} already verified that minimizing \eqref{eqn: empirical_risk_function} using labeled data only  with $\delta=1$ can obtain the ground truth $W^*$  when  $N \ge N^* = c(\kappa)\mu^{*2}K^3d\log q$ \footnote{$\mu^* = \mu(\delta ,\delta)$, and $\mu^*=\mu(\delta,\de)$ when $\de$ is smaller than $1$.} 
for some positive constant $q$.
    %for some $N^*$. Therefore, 
The focus of this paper is to analysis the performance of self-training algorithm in low labeled data regime,
\begin{equation}\label{eqn: definition_N*}
    N< N^* = c(\kappa)\mu^{*2}K^3d\log q.
\end{equation}
%\tcr{for some positive constant $q$, and the value in \eqref{eqn: definition_N*} is the tightest bound among the existing theoretical results,  to the best of our knowledge, for supervised learning algorithms reaching zero generalization error.}
Specifically, how unlabeled data   help to learn a proper model when $N$ is small.
%This paper focuses on studying the performance of self-training algorithm in low data regime ($N< N^*$) given some initial weight $\bfW^{(0)}$, and we provide the conditions of $\hat{\lambda}$ and $M$ for obtaining an improved learned model over the initial weights.}
\fi




% \textbf{Focus of this paper.} 
% The teacher model is not unique because any permutation of the neurons weights does not change the output. Therefore, we have 
% \begin{equation}
%     y_n=g(\bfW^*;\bfx_n)=g(\bfW^*\bfP;\bfx_n),
% \end{equation}
% where $\bfP\in\{0,1\}^{K\times K}$ represents any permutation matrix.




\iffalse
Given two groups of data $\mathcal{D}$ and $\w[\mathcal{D}]$, where $\mathcal{D}$ denotes the labeled data and $\widetilde{\mathcal{D}}$ denotes the unlabeled data, we study the self-training approach, which is a semi-supervised learning problem, in recovering the ground truth teacher model $g(\bfW^*)$, where $g$ represents   network structure and $\bfW^*$ is the ground truth parameters. 
Given \tcr{a preliminary teacher model} with weights $\bfW^{(0)}$, we use this teacher model to calculate pseudo labels for the unlabeled data in $\w[\mathcal{D}]=\{\w[\bfx]_m \}_{m=1}^M$. Then, the neural network optimization problem is trained via minimizing the objective function of the mixture of data in both $\mathcal{D}$ and $\w[\mathcal{D}]$.
Suppose the estimated pseudo labels are denoted as $\w[y]_m$ for input $\w[\bfx]_m\in\w[\mathcal{D}]$ and the labeled data is denoted as $\mathcal{D}=\{\bfx_n,y_n \}_{n=1}^N$, following the setup in \citep{Lee13}, the objective function, which is also named as the \textbf{\textit{empirical risk function}} (ERF), is defined as 
\begin{equation}\label{eqn: empirical_risk_function}
    \hat{f}_{\mathcal{D},\w[\mathcal{D}]}(\bfW) = \frac{\lambda}{2N}\sum_{n=1}^N\big(y_n - g(\bfW;\bfx_n) \big)^2 + \frac{\w[\lambda]}{2M}\sum_{m=1}^M \big(\w[y]_m - g(\bfW;\w[\bfx]_m) \big)^2, 
\end{equation}
where $\lambda+\w[\lambda]= 1$. Thus, the optimization problem in training the neural network is written as:
\begin{equation}\label{eqn:studnet}
    \min_{\bfW}: \quad  \hat{f}_{\mathcal{D},\w[\mathcal{D}]}(\bfW).
\end{equation}
The performance of the learned model $g$ with weights $\bfW$ is estimated through the \textbf{\textit{generalization function}} (GF) as shown below:
\begin{equation}\label{eqn: GF}
    I\big(g(\bfW)\big) = \mathbb{E}_{(\bfx, y)\sim \mathcal{D}}\big(y - g(\bfW;\bfx)\big)^2.
\end{equation}
 Note that $y=g(\bfW^*;\bfx)$ for labeled data in $\mathcal{D}$, one can easily check that $\bfW^*$ is the global optimal to the GF in \eqref{eqn: GF}. In addition, for activation functions with bounded gradient\footnote{To name a few, linear, ReLU, sigmoid and logistic activation functions.}, the generalization error is upper bounded by the distance of $\bfW$ and $\bfW^*$ with an extra constant factor.  
% Although such form of GF in \eqref{eqn: GF} is widely used numerically, the value of GF is hard to characterize during theoretical analysis. According to the recent study \cite{ZSJB17}, there is a relatively flat and large local convex region near the ground truth of the GF  when the input data belongs to Gaussian distribution. Therefore, the distance of weights $\bfW$ to  the ground truth $\bfW^*$ is an alternative to the GF in theoretical analysis. In addition, from Figure \ref{fig:GF}, we can see the value of GF is almost a linear function of the normalized distance between $\bfW$ and $\bfW^*$ for Gaussian synthetic data. Therefore, we use the distance of weights of the learned $\bfW$ and ground truth $\bfW^*$ to representation the generalization error instead of the standard definition for the convenience of theoretical analysis. 
\fi




\iffalse
\tcr{and thus $\bfW^*$ is one of the global optimal for the loss function
\begin{equation}\label{eqn: loss_1}
    L_{\mathcal{D}}(\bfW) = \frac{1}{N}\sum_{n=1}^N(y_n - g(\bfW;\bfx_n) )^2.
\end{equation}

and $\w[\bfW]$ is one of the global optimal for 
\begin{equation}\label{eqn: loss_2}
    \w[L]_{\w[\mathcal{D}]}(\bfW) = \frac{1}{M}\sum_{m=1}^M(\w[y]_m - g(\bfW;\w[\bfx]_m) )^2.
\end{equation}}
% Given an estimated teacher model $\widetilde{\bfW}$, the pseudo label is calculated as
% \begin{equation}\label{eqn: psedu_label}
%     \w[y]_m = g(\widetilde{\bfW};\w[\bfx]_m) = \frac{1}{K}\sum_{k=1}^K \phi(\widetilde{\bfw}_j^{T}\w[\bfx]_m),
% \end{equation}
% where $\widetilde{\bfw}_j$ is the $j$-th column of $\widetilde{\bfW}$. Therefore, $\bfW^*$ is one of the global optimal for the loss function
% \begin{equation}\label{eqn: loss_1}
%     L_{\mathcal{D}}(\bfW) = \frac{1}{N}\sum_{n=1}^N(y_n - g(\bfW;\bfx_n) )^2,
% \end{equation}
% while $\w[\bfW]$ is one of the global optimal for 
% \begin{equation}\label{eqn: loss_2}
%     \w[L]_{\w[\mathcal{D}]}(\bfW) = \frac{1}{M}\sum_{m=1}^M(\w[y]_m - g(\bfW;\w[\bfx]_m) )^2.
% \end{equation}
Moreover, the objective function in \eqref{eqn: empirical_risk_function} can be re-written as 
\begin{equation}\label{eqn: empirical_risk_function_2}
    \hat{f}_{\mathcal{D},\mathcal{D}}(\bfW) = {\lambda}L_{\mathcal{D}}(\bfW) + \w[\lambda]\w[L]_{\w[\mathcal{D}]}(\bfW).
\end{equation}
%\textbf{Definition of additional notations.}
\fi







==> Self-training (6)/proof_1.tex <==
\section{Proof of Theorem \ref{Thm: sufficient_number}}
\label{sec: sufficient_number}
With $p=1$ in \eqref{eqn: p_population_risk_function}, the \textit{population risk function} is reduced as 
\begin{equation}\label{eqn: population_risk_function}
    f(\bfW) =  \frac{\lambda}{2} \mathbb{E}_{\bfx} (y - g(\bfW;\bfx)) + \frac{\w[\lambda]}{2} \mathbb{E}_{\w[\bfx]} (\w[y]^* - g(\bfW;\w[\bfx])),
\end{equation}
where $y=g(\bfW^*;\bfx)$ with $\bfx\sim \mathcal{N}(0,\delta^2\bfI)$ and $\w[y]^* = g(\bfW^*;\w[\bfx])$ with $\w[\bfx]\sim \mathcal{N}(0,\de^2\bfI)$. In fact, \eqref{eqn: population_risk_function} can be viewed as the expectation of the \textit{empirical risk function} in \eqref{eqn: empirical_risk_function} given $\w[y]_m = g(\bfW^*;\w[\bfx]_m)$. Moreover, the ground-truth model $\bfW^*$ is the global optimal to \eqref{eqn: population_risk_function} as well. Lemmas \ref{lemma: population_second_order_derivative} and \ref{Lemma: first_order_distance} are the special case of Lemmas \ref{Lemma: p_second_order_derivative bound} and \ref{Lemma: p_first_order_derivative} with $p=1$. The proof of Theorem \ref{Thm: sufficient_number} is followed by the presentation of the two lemmas.

The main idea in proving Theorem \ref{Thm: sufficient_number} is to characterize the gradient descent term by \Revise{ the MVT in Lemma \ref{Lemma: MVT}} as shown in \eqref{eqn: Thm3_temp1} and \eqref{eqn: Thm3_temp2}. The IVT is not directly applied in the empirical risk function because of its non-smoothness. However, the population risk functions defined in \eqref{eqn: p_population_risk_function} and \eqref{eqn: population_risk_function}, which are the expectations over the Gaussian variables, are smooth. Then, as the distance $\|\nabla f (\bfW) - \nabla f(\bfW^*) \|_F$ is upper bounded by a linear function of $\|\bfW - \bfW^*\|_F$ as shown in \eqref{eqn:eta1}, we can establish the connection between $\|\W[\ell,t+1] -\bfW^* \|_F$  and $\|\W[\ell,t]-\bfW^*\|_F$ as shown in \eqref{eqn: induction_t}. \Revise{Finally}, by mathematical induction over $\ell$ and $t$, one can characterize $\|\W[L,0]-\bfW^*\|_F$ by $\| \W[0,0] -\bfW^* \|_F$ as shown in \eqref{eqn:outer_loop}, which completes the whole proof. 



\begin{lemma}[Lemma \ref{Lemma: p_second_order_derivative bound} with $p=1$]
\label{lemma: population_second_order_derivative}
    Let $f$ and $\hat{f}$ are the functions defined in \eqref{eqn: population_risk_function} and $\eqref{eqn: empirical_risk_function}$, respectively. Then, for any $\bfW$ that satisfies,
    \begin{equation}\label{eqn: initial_point}
        \|\bfW-\bfW^*\|_F \le \frac{\sigma_K}{\mu^2 K},
    \end{equation}
    we have 
    \begin{equation}
        \frac{\lambda\rho(\delta)+\w[\lambda]\rho(\de)}{\Revise{12}\kappa^2\gamma K^2} \preceq \nabla^2 {f}(\bfW) \preceq \frac{7(\lambda\delta^2+\w[\lambda]\de^2)}{K}.
    \end{equation}
\end{lemma}

% \begin{lemma}[Lemma \ref{Lemma: p_Second_order_distance} with $p=1$]\label{Lemma:Second_order_distance}
%   Let $f$ be the population risk function defined in \eqref{eqn: population_risk_function}. Then, for any $\bfW$ in \eqref{eqn: initial_point}, we have 
%   \begin{equation}
%       \| \nabla^2 f(\bfW^*)- \nabla^2 f(\bfW) \|_2 \lesssim \frac{\lambda\delta^2+(1-\lambda)\de^2}{K}\cdot\frac{\|\bfW^*-\bfW\|_2}{\sigma_K}. 
%   \end{equation}
% \end{lemma}

 \begin{lemma}[Lemma \ref{Lemma: p_first_order_derivative} with $p =1$]
 \label{Lemma: first_order_distance}
   Let $f$ and $\hat{f}$ be the functions defined in \eqref{eqn: population_risk_function} and \eqref{eqn: empirical_risk_function}, respectively. Suppose the pseudo label is generated through \eqref{eqn: psedu_label} with weights $\widetilde{\bfW}$. Then, we have
      \begin{equation}
   \begin{split}
        \|\nabla f(\bfW) -\nabla \hat{f}(\bfW) \|_2
        \lesssim&
       \Big(\frac{\lambda\delta^2}{K} \sqrt{\frac{d\log q}{N}} + \frac{(1- \lambda)\de^2}{K} \sqrt{\frac{d\log q}{M}}\Big)\cdot \| \bfW -\bfW^* \|_2\\
       & + \frac{(1- \lambda)\de^2}{K}\Big( \sqrt{\frac{d\log q}{M}}+\frac{1}{2} \Big)\cdot\|\w[\bfW]-\bfW^* \|_2
   \end{split}
    \end{equation}
    with probability at least $1-q^{-d}$.
\end{lemma}

\begin{proof}[Proof of Theorem \ref{Thm: sufficient_number}]
    From Algorithm \ref{Algorithm: Alg1}, in the $\ell$-th outer loop, we have 
    \begin{equation}\label{eqn: Thm3_temp1}
    \begin{split}
       \W[\ell, t+1] 
       = &  \W[\ell, t] -\eta \nabla\hat{f}_{\mathcal{D}_t, \widetilde{\mathcal{D}}_t}(\W[\ell, t])+\beta (\W[\ell, t] - \W[\ell, t-1])\\
       = & \W[\ell, t] -\eta \nabla{f}(\W[\ell, t])+\beta (\W[\ell, t] - \W[\ell, t-1])\\
       &+ \eta \cdot \big( \nabla f(\W[\ell, t]) - \nabla \hat{f}_{\mathcal{D}_t, \widetilde{\mathcal{D}}_t}(\W[\ell, t]) \big).
    \end{split}
    \end{equation}
    Since $\nabla f$ is a smooth function and $\bfW^*$ is a local (global) optimal to $f$, then we have 
    \begin{equation}\label{eqn: Thm3_temp2}
        \begin{split}
            \nabla{f}(\W[\ell, t])
            =& \nabla{f}(\W[\ell, t]) - \nabla{f}(\bfW^*)\\
            =&\Revise{\int_{0}^1 \nabla^2 f\Big(\bfW^{(\ell,t)} + u \cdot(\bfW^{(\ell,t)}-\bfW^*) \Big)du \cdot(\W[\ell, t]-\bfW^*)},
        \end{split}
    \end{equation}
    where the last equality comes from \Revise{MVT in Lemma \ref{Lemma: MVT}}. 
    \Revise{For notational convenience, we use $\bfH^{(\ell, t)}$ to denote the integration as
    \begin{equation}
        \bfH^{(\ell,t)} : = \int_{0}^1 \nabla^2 f\Big(\bfW^{(\ell,t)} + u \cdot(\bfW^{(\ell,t)}-\bfW^*) \Big)du.    
    \end{equation}}
    
    Then, we have 
    \begin{equation}\label{eqn: matrix_convergence}
        \begin{split}
         \begin{bmatrix}
        \W[\ell, t+1]-\bfW^*\\
        \W[\ell, t]-\bfW^*
        \end{bmatrix}
        =
        &\begin{bmatrix}
                \bfI -\eta\Revise{\bfH^{(\ell, t)}}& \beta \bfI\\
                \bfI & \boldsymbol{0}
        \end{bmatrix}
         \begin{bmatrix}
        \W[\ell, t]-\bfW^*\\
        \W[\ell, t-1]-\bfW^*
        \end{bmatrix}\\
            &+\eta \begin{bmatrix}
            \nabla f(\W[\ell, t]) - \nabla \hat{f}_{\mathcal{D}_t, \widetilde{\mathcal{D}}_t}(\W[\ell, t])\\
            \boldsymbol{0}
        \end{bmatrix}.
        \end{split}
        \end{equation}
    % Let $\bfA(\beta)= \begin{bmatrix}
    %             \bfI -\eta\nabla^2 f(\hat{\bfW}^{(\ell, t)})& \beta \bfI\\
    %             \bfI & \boldsymbol{0}
    %     \end{bmatrix}$, then \eqref{eqn: matrix_convergence} implies
    %     \begin{equation}\label{eqn: convergence_origin}
    %     \begin{split}
    %         \| \W[\ell, t+1]-\bfW^* \|_2 
    %         \le \|\bfA(\beta) \|_2 \| \W[\ell, t]-\bfW^* \|_2
    %         + \eta \cdot \|\nabla f(\W[\ell, t]) - \nabla \hat{f}(\W[\ell, t]\|_2
    %     \end{split}    
    %     \end{equation}
    \Revise{Let $\bfH^{(\ell, t)}=\bfS\mathbf{\Lambda}\bfS^{T}$ be the eigen-decomposition of $\bfH^{(\ell, t)}$.} Then, we define
\begin{equation}\label{eqn:Heavy_ball_eigen}
\begin{split}
{\bfA}(\beta)
: =&
\begin{bmatrix}
\bfS^T&\bf0\\
\bf0&\bfS^T
\end{bmatrix}
\bfA(\beta)
\begin{bmatrix}
\bfS&\bf0\\
\bf0&\bfS
\end{bmatrix}
=\begin{bmatrix}
\bfI-\eta\bf\Lambda+\beta\bfI &\beta\bfI\\
\bfI& 0
\end{bmatrix}.
\end{split}
\end{equation}
Since 
$\begin{bmatrix}
\bfS&\bf0\\
\bf0&\bfS
\end{bmatrix}\begin{bmatrix}
\bfS^T&\bf0\\
\bf0&\bfS^T
\end{bmatrix}
=\begin{bmatrix}
\bfI&\bf0\\
\bf0&\bfI
\end{bmatrix}$, we know $\bfA(\beta)$ and $\begin{bmatrix}
\bfI-\eta\bf\Lambda+\beta\bfI &\beta\bfI\\
\bfI& 0
\end{bmatrix}$
share the same eigenvalues. 
Let $\gamma^{(\bf\Lambda)}_i$ be the $i$-th eigenvalue of $\nabla^2f(\widehat{\bfw}^{(t)})$, then the corresponding $i$-th eigenvalue of \eqref{eqn:Heavy_ball_eigen}, denoted by $\gamma^{(\bfA)}_i$, satisfies 
\begin{equation}\label{eqn:Heavy_ball_quaratic}
(\gamma^{(\bfA)}_i(\beta))^2-(1-\eta \gamma^{(\bf\Lambda)}_i+\beta)\gamma^{(\bfA)}_i(\beta)+\beta=0.
\end{equation}
By simple calculation, we have 
\begin{equation}\label{eqn:heavy_ball_beta}
\begin{split}
|\gamma^{(\bfA)}_i(\beta)|
=\begin{cases}
\sqrt{\beta}, \qquad \text{if}\quad  \beta\ge \big(1-\sqrt{\eta\gamma^{(\bf\Lambda)}_i}\big)^2,\\
\frac{1}{2} \left| { (1-\eta \gamma^{(\bf\Lambda)}_i+\beta)+\sqrt{(1-\eta \gamma^{(\bf\Lambda)}_i+\beta)^2-4\beta}}\right| , \text{otherwise}.
\end{cases}
\end{split}
\end{equation}
Specifically, we have
\begin{equation}\label{eqn: Heavy_ball_result}
\gamma^{(\bfA)}_i(0)>\gamma^{(\bfA)}_i(\beta),\quad \text{for}\quad  \forall \beta\in\big(0, (1-{\eta \gamma^{(\bf\Lambda)}_i})^2\big),
\end{equation}
and  $\gamma^{(\bfA)}_i$ achieves the minimum $\gamma^{(\bfA)*}_{i}=\Big|1-\sqrt{\eta\gamma^{(\bf\Lambda)}_i}\Big|$ when $\beta= \Big(1-\sqrt{\eta\gamma^{(\bf\Lambda)}_i}\Big)^2$.
\Revise{From Lemma \ref{lemma: population_second_order_derivative}, for any $\bfa\in \mathbb{R}^d$ with $\|\bfa\|_2=1$, we have 
    \begin{equation}
        \begin{gathered}
            \bfa^T\nabla{f}(\W[\ell, t])\bfa = \int_{0}^1 \bfa^T\nabla^2 f\Big(\bfW^{(\ell,t)} + u \cdot(\bfW^{(\ell,t)}-\bfW^*)\Big)\bfa du \le \int_{0}^1 \gamma_{\max} \|\bfa\|_2^2du =\gamma_{\max},
            \\
            \bfa^T\nabla{f}(\W[\ell, t])\bfa = \int_{0}^1 \bfa^T\nabla^2 f\Big(\bfW^{(\ell,t)} + u \cdot(\bfW^{(\ell,t)}-\bfW^*)\Big)\bfa du \ge \int_{0}^1 \gamma_{\min} \|\bfa\|_2^2du =\gamma_{\min},
        \end{gathered}
    \end{equation}
    where $\gamma_{\max} =\frac{7(\lambda\delta^2+\widetilde{\lambda}\de^2)}{K}$, and $\gamma_{\min} = \frac{\lambda\rho(\delta)+\widetilde{\lambda}\rho(\de)}{12\kappa^2\gamma K^2}$.}
    % $$ a^T(\int_{0}^1 v(u) du)a = \int_{0}^1 a^Tv(u)a du \le \int_{0}^1 \gamma_{\max} \|a\|^2du =\gamma_{\max} \|a\|^2,$$
% $$ a^T(\int_{0}^1 v(u) du)a = \int_{0}^1 a^Tv(u)a du \ge \int_{0}^1 \gamma_{\min} \|a\|^2du =\gamma_{\min} \|a\|^2.$$
    Therefore, we have
    \begin{equation}
        \begin{split}
        \gamma^{(\bf\Lambda)}_{\min} 
        = \frac{\lambda\rho(\delta)+\widetilde{\lambda}\rho(\de)}{12\kappa^2\gamma K^2}, 
        \quad 
        \text{and}
        \quad
        \gamma^{(\bf\Lambda)}_{\max} 
        = \frac{7(\lambda\delta^2+\widetilde{\lambda}\de^2)}{K}.
        \end{split}
    \end{equation}
    Thus, we can select $\eta = \big(\frac{1}{\sqrt{\gamma^{(\bf\Lambda)}_{\max}} + \sqrt{\gamma^{(\bf\Lambda)}_{\min} }}\big)^2$, and $\|\bfA(\beta)\|_2$ can be bounded by
    \begin{equation}\label{eqn: beta}
        \begin{split}
        \min_{\beta}\|\bfA(\beta)\|_2 
        \le& 1-\sqrt{\big(\frac{\lambda\rho(\delta)+\widetilde{\lambda}\rho(\de)}{12\kappa^2\gamma K^2}\big)/\big(2\cdot \frac{7(\lambda\delta^2+\widetilde{\lambda}\de^2)}{K} \big)} \\
        = & 1- \frac{\mu(\delta,\de)}{\sqrt{168\kappa^2\gamma K}},
        \end{split}
    \end{equation}
    where $\mu(\delta,\de) = \Big( \frac{\lambda\rho(\delta)+\widetilde{\lambda}\rho(\de)}{\lambda\delta^2+\widetilde{\lambda}\de^2} \Big)^{1/2}$.
    
    From Lemma \ref{Lemma: first_order_distance}, we have 
    \begin{equation}\label{eqn:eta1}
        \begin{split}
            \|\nabla f(\W[\ell, t]) -\nabla \hat{f}(\W[\ell, t]) \|_2
            =&\Big(\frac{\lambda\delta^2}{K} \sqrt{\frac{d\log q}{N_t}} + \frac{\w[\lambda]\de^2}{K} \sqrt{\frac{d\log q}{M_t}}\Big)\cdot \| \W[\ell, t] -\bfW^* \|_2\\
            & + \frac{\w[\lambda]\de^2}{K}\Big( \sqrt{\frac{d\log q}{M_t}}+\frac{1}{2} \Big)\cdot\|\W[\ell, 0]-\bfW^* \|_2.
        \end{split}
    \end{equation}
    Given $\varepsilon>0$ and $\tilde{\varepsilon}>0$ with $\varepsilon+\tilde{\varepsilon}<1$, let
    \begin{equation}\label{eqn:eta2}
        \begin{split}
            &\eta \cdot \frac{\lambda\delta^2}{K} \sqrt{\frac{d\log q}{N_t}}
            \le \frac{\varepsilon\mu(\delta,\de)}{\sqrt{168\kappa^2\gamma K}} \text{,}\\
            \text{and}& \quad
            \eta \cdot \frac{\widetilde{\lambda}\de^2}{K} \sqrt{\frac{d\log q}{M_t}}
            \le \frac{\tilde{\varepsilon}\mu(\delta,\de)}{\sqrt{168\kappa^2\gamma K}},
        \end{split}
    \end{equation}
    where we need 
    \begin{equation}\label{eqn:proof_sample1}
    \begin{split}
        &N_t \ge \varepsilon^{-2}\mu^{-2}\big(\frac{\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2}\big)^2\kappa^2\gamma K^3 d\log q,\\
        \text{and}&\quad 
        M_t \ge 
        \tilde{\varepsilon}^{-2}\mu^{-2}\big(\frac{\w[\lambda]\de^2}{\lambda\delta^2+\w[\lambda]\de^2}\big)^2\kappa^2\gamma K^3 d\log q.
        \end{split}
    \end{equation}
    Therefore, from \eqref{eqn: beta}, \eqref{eqn:eta1} and \eqref{eqn:eta2}, we have
    \begin{equation}\label{eqn: induction_t}
        \begin{split}
            &\| \W[\ell, t+1]-\bfW^* \|_2\\
            \le& \Big( 1- \frac{(1-\varepsilon-\tilde{\varepsilon})\mu(\delta,\de)}{\sqrt{168\kappa^2\gamma K}} \Big)\| \W[\ell, t]-\bfW^* \|_2
            +\eta\cdot\frac{\w[\lambda]\de^2}{K}\Big( \sqrt{\frac{d\log q}{M_t}}+\frac{1}{2} \Big) \cdot\|\W[\ell, 0]-\bfW^* \|_2\\
            \le & \Big( 1- \frac{(1-\varepsilon-\tilde{\varepsilon})\mu(\delta,\de)}{\sqrt{168\kappa^2\gamma K}} \Big)\| \W[\ell, t]-\bfW^* \|_2
            +\eta \cdot \frac{\w[\lambda]\de^2}{K}\|\W[\ell, 0] -\bfW^*\|_2
        \end{split}
    \end{equation}
    when $M\ge 4d\log q$.
    % To make sure that $\W[\ell, t+1]$ satisfies \eqref{eqn: initialization}, we require that 
    % \begin{equation}
    %     \frac{\w[\lambda]\de^2}{\w[\lambda]\de^2+\lambda\delta^2}\le \frac{2\mu}{\sqrt{\kappa^2\gamma}}. 
    % \end{equation}
    By mathematical induction on \eqref{eqn: induction_t} over $t$, we have 
    \begin{equation}\label{eqn:inner_loop}
    \begin{split}
            &\| \W[\ell, t]-\bfW^* \|_2\\
            \le&\Big( 1- \frac{(1-\varepsilon-\tilde{\varepsilon})\mu}{\sqrt{168\kappa^2\gamma K}} \Big)^t\cdot\|\W[\ell, 0]-\bfW^* \|_2
            \\
            &+
            \frac{\sqrt{168\kappa^2\gamma K}}{(1-\varepsilon-\tilde{\varepsilon})\mu}\cdot \frac{\sqrt{K}}{14 (\lambda\delta^2+\w[\lambda]\de^2 )}\cdot\frac{\w[\lambda]\de^2}{K} 
            \|\W[\ell, 0]-\bfW^* \|_2\\
            \le& \bigg[\Big( 1- \frac{(1-\varepsilon-\tilde{\varepsilon})\mu}{\sqrt{168\kappa^2\gamma K}} \Big)^t+
            \frac{\sqrt{\kappa^2\gamma}\w[\lambda]\de^2}{(1-\varepsilon-\tilde{\varepsilon})\mu(\lambda\delta^2+\w[\lambda]\de^2)}\bigg]\cdot\|\W[\ell, 0]-\bfW^* \|_2
        \end{split}
    \end{equation}
    By mathematical induction on \eqref{eqn:inner_loop} over $\ell$, we have 
    \begin{equation}\label{eqn:outer_loop}
    \begin{split}
            &\| \W[\ell, T]-\bfW^* \|_2\\
            \le& \bigg[\Big( 1- \frac{(1-\varepsilon-\tilde{\varepsilon})\mu}{\sqrt{168\kappa^2\gamma K}} \Big)^T
            +
            \frac{\sqrt{\kappa^2\gamma}\w[\lambda]\de^2}{(1-\varepsilon-\tilde{\varepsilon})\mu(\lambda\delta^2+\w[\lambda]\de^2)}\bigg]^{\ell}\cdot\|\W[0, 0]-\bfW^* \|_2
        \end{split}
    \end{equation}
\end{proof}

==> Self-training (6)/simulation.tex <==
\section{Empirical results}\label{sec: empirical_results}
\subsection{Synthetic data experiments}
\vspace{-1mm}
We generate a ground-truth   neural network with the width $K=10$.  Each entry of $\bfW^*$ is uniformly selected from $[-2.5, 2.5]$. 
The input of    labeled  data $\bfx_n$ %\in\mathcal{D}$ is
are generated from Gaussian distribution $\mathcal{N}(0, \bfI_{d})$ independently, and the corresponding label $y_n$ is generated through \eqref{eqn: teacher_model} using $\bfW^*$. The unlabeled data % The input of unlabeled data 
$\w[\bfx]_m$ %\in \w[\mathcal{D}]$ belongs 
are generated from $\mathcal{N}(0, \widetilde{\delta}^2 \bfI_{d})$ independently with $\widetilde{\delta}=1$ except in Figure \ref{fig: delta}. $d$ is set as $50$ except in Figure \ref{fig: M_pt}. % and $K$ is fixed as $10$ per layer.
The value of $\lambda$ is selected as $\sqrt{N/(2Kd)}$ except in Figure \ref{fig: lambda}.
We consider one-hidden-layer except in Figure \ref{fig:GF_1M}.
%The entries of $\bfW^*$ are generated uniformly   from $[-2.5, 2.5]$ independently. Without special notations, the dimension of the input $d$ is selected as $50$, and the number of neurons $K$ is $10$. Both the variance $\delta^2$ and $\de^2$ are selected as $1$. 
%The preliminary model in the algorithm is implemented as the initial points
The initial teacher model $\bfW^{(0)}$ in self-training is randomly selected from $\{\bfW|\|\bfW-\bfW^* \|_F/\|\bfW^*\|_F \le 0.5  \}$ to reduce the computation. In each iteration, the  maximum number of SGD steps $T$ is   $10$. Self-training terminates if $\|\bfW^{(\ell+1)}-\bfW^{(\ell)}\|_F/\|\bfW^{(\ell)}\|_F\le 10^{-4}$ or reaching $1000$  iterations. In Figures \ref{fig: M_N} to \ref{fig: lambda}, all the points on the curves are averaged over $1000$ independent trials, and the regions in lower transparency indicate  the corresponding  one-standard-deviation error bars. Our \textbf{empirical observations} are summarized below.

\iffalse
The preliminary model in the pseudocode is implemented as the initial points $\bfW^{(0)}$ are randomly selected from $\{\bfW|\|\bfW-\bfW^* \|_F \le 0.5  \}$ to reduce the computation time. Additionally, the maximum number of the inner loop $T$ is selected as $10$, and the algorithm terminates if $\|\bfW^{(\ell+1)}-\bfW^{(\ell)}\|_F/\|\bfW^{(\ell)}\|_F\le 10^{-4}$ or reaching $1000$ number of iterations.
The input of labeled data $\bfx_n\in\mathcal{D}$ is randomly generated from Gaussian distribution $\mathcal{N}(0, \delta^2\bfI_{d})$ independently, and the corresponding output $y_n$ is generated through \eqref{eqn: teacher_model}. The input of unlabeled data $\w[\bfx]_m \in \w[\mathcal{D}]$ belongs to $\mathcal{N}(0, \de^2\bfI_{d})$ independently. 
The entries of $\bfW^*$ are generated uniformly   from $[-2.5, 2.5]$ independently. Without special notations, the dimension of the input $d$ is selected as $50$, and the number of neurons $K$ is $10$. Both the variance $\delta^2$ and $\de^2$ are selected as $1$.   
\fi



\textbf{(a) GF (testing performance) proportional to $\|\bfW -\bfW^*\|_F$.}
Figure \ref{fig:GF_1M} illustrates the GF in \eqref{eqn: GF} against the distance to the ground truth $\bfW^*$. To visualize results for different networks together, % make the results comparable within one figure, the value of the generalization function in each experiment 
GF is normalized  in $[0, 1]$, divided by its   largest value for each network architecture.  
%In Figure \ref{fig:GF_1M}(a), the results are 
All the results are averaged over $100$ independent choice of $\bfW$. 
One can see that for one-hidden-layer neural networks,  in a %sufficiently 
large region near  $\bfW^*$,   GF is almost linear in $\|\bfW -\bfW^*\|_F$. When the number of hidden layers increases, this region decreases, but the linear dependence still holds locally. This is an empirical justification of using $\|\bfW -\bfW^*\|_F$  to evaluate the GF and, thus, the testing error in Theorems 1 and 2. 
% \PY{(The last sentence seems incomplete)}
% $\bfW$ and $\bfW^*$ for Gaussian synthetic data. Therefore, we use the distance of weights of the learned $\bfW$ and ground truth $\bfW^*$ to represent the generalization error instead of the standard definition for the following experiments, which is also  consistent with our theoretical results. Figure \ref{fig:GF_1M}(b) is the supplementary results for deep neural networks. Although the linear region becomes smaller compared with one-hidden-layer case, one can still see that the generalization function is an increasing function of $\|\bfW-\bfW^* \|_F$.  

\textbf{(b) $\|\W[L]-\bfW^*\|_F$ as a linear function of $1/\sqrt{M}$.}
 Figure \ref{fig: M_N} shows the relative error $\|\W[L]-\bfW^*\|_F/\| \bfW^* \|_F$ when the number of unlabeled data and labeled data changes. 
%  All the points on the curves are averaged over $1000$ independent trials, and the regions in lower transparency indicate  the corresponding  one-standard-deviation error bars. % which indicate one standard deviation error. 
 One can see that the relative error decreases when either $M$ or $N$ increases. Additionally, the dash-dotted lines represent the best fitting of the linear functions of $1/\sqrt{M}$ using the least square method. Therefore, the relative error is indeed % and the performance improvement is approximately
 a linear function of $1/\sqrt{M}$, as predicted by our results in \eqref{eqn: p_convergence_*} and \eqref{eqn: convergence}. 
\begin{figure}[h]
\vspace{-2.5mm}
     \begin{minipage}{0.32\linewidth}
         \centering
         \includegraphics[width=0.9\textwidth]{Figure/generalization_error.pdf}
         \vspace{-2mm}
         \caption{The generalization function against the distance to the ground truth neural network}
        \label{fig:GF_1M}
    \end{minipage}
    ~
    \begin{minipage}{0.32\linewidth}
  	    \centering
  	    \includegraphics[width=0.95\linewidth]{Figure/M_N.pdf}
  	    \vspace{-2mm}
  	    \caption{The relative error against the number of unlabeled data.}
  	    \label{fig: M_N}
  	\end{minipage}
  	~
  	 \begin{minipage}{0.32\linewidth}
        \centering
  	    \includegraphics[width=0.95\linewidth]{Figure/convergence_rate_p.pdf}
        \vspace{-2mm}
        \caption{The convergence rate with different $M$ when $N<N^*$.}
        \label{fig:M_ite}
    \end{minipage}
  	\vspace{-4mm}
\end{figure}
\vspace{-2.5mm}
% \begin{figure}[h]
%     \centering
%     \begin{minipage}{0.45\linewidth}
%         \centering
%         \includegraphics[width=0.8\linewidth]{Figure/generalization_function.pdf}
%         \caption{The value of generalization function against the distance to the ground truth}
%         \label{fig:GF}
%     \end{minipage}
%     ~
%     \begin{minipage}{0.45\linewidth}
%         \centering
%         \includegraphics[width=0.8\linewidth]{Figure/generalization_error.pdf}
%         \caption{The value of generalization function for deep neural networks}
%         \label{fig:GF_m}
%     \end{minipage}
% \end{figure}


% \begin{wrapfigure}{r}{0.55\linewidth}
%     \vspace{-4mm}
%     \centering
%      \begin{subfigure}[b]{0.265\textwidth}
%          \centering
%   	    \includegraphics[width=1.0\linewidth]{Figure/convergence_rate_p.pdf}
%   	    \vspace{-5.5mm}
%   	    \caption{}
%   	    \label{fig: M_ite_1} 
%      \end{subfigure}
%      ~
%      \begin{subfigure}[b]{0.265\textwidth}
%          \centering
%       	\includegraphics[width=1.0\linewidth]{Figure/convergence_rate.pdf}
%   	    \vspace{-5.5mm}
%   	    \caption{}
%   	    \label{fig: M_ite_2}  
%      \end{subfigure}
%      \vspace{-8mm}
%      \caption{The convergence rate with different $M$ when (a) $N<N^*$ and (b) $N>N^*$.}
%      \vspace{-5mm}
%         \label{fig:M_ite}
% \end{wrapfigure}

% \begin{figure}[h]
%     \begin{minipage}{0.45\linewidth}
%         \centering
%   	    \includegraphics[width=0.75\linewidth]{Figure/convergence_rate_p.pdf}
%   	    \caption{The number of iterations against relative error with different $M$}
%   	    \label{fig: M_ite}  
%     \end{minipage}
%   	~
%   	\begin{minipage}{0.45\linewidth}
%   	    \centering
%       	\includegraphics[width=0.75\linewidth]{Figure/convergence_rate.pdf}
%   	    \caption{The number of iterations against relative error with different $M$}
%   	    \label{fig: M_ite_p}    
%   	\end{minipage}
% \end{figure}

% \textbf{Convergence rate w.r.t $\de$.}
% \begin{figure}[H]
%   	\centering
%   	\includegraphics[width=0.4\linewidth]{Figure/delta.pdf}
%   	\caption{The number of iterations against relative error with different $\de$}
%   	\label{fig: delta_ite}
% \end{figure}

% \begin{figure}[H]
%   	\centering
%   	\includegraphics[width=0.5\linewidth]{Figure/M_N.pdf}
%   	\caption{The relative error against the number of unlabeled data}
%   	\label{fig: M_N}
% \end{figure}


% \begin{wrapfigure}{r}{0.40\linewidth}
%         \centering
%   	    \includegraphics[width=1.0\linewidth]{Figure/convergence_rate_p.pdf}
%   	    \caption{The convergence rate with different $M$}
%   	    \label{fig: M_ite_1} 
% \end{wrapfigure}

\textbf{(c) Convergence rate as a linear function of $1/\sqrt{M}$.}
Figure \ref{fig:M_ite} illustrates the convergence rate when $M$ and $N$ change. 
% Similar to Figure \ref{fig: M_N}, the results are averaged over $1000$ independent trials for each point, and the regions in lower transparency indicates the corresponding error bars. 
We can see that the convergence rate is a linear function of ${1}/{\sqrt{M}}$, as predicted by our results \eqref{eqn: p_convergence_*} and \eqref{eqn: convergence}. When $M$ increases, {the convergence rate is improved, and the method converges faster.} 
% \PY{(rate "decreases" means faster reads non-smooth. Should it be "increases"?)}

%in both the cases that the number of $N$ is greater or smaller than $N^*$, which verified the conclusions about convergence analysis for both Theorems \ref{Thm: p_convergence} and \ref{Thm: sufficient_number}. 

% \begin{figure}[h]
%     \begin{minipage}{0.4\linewidth}
%         \vspace{-4mm}
%         \centering
%   	    \includegraphics[width=0.8\linewidth]{Figure/convergence_rate_p.pdf}
%         \caption{The convergence rate with different $M$ when $N<N^*$.}
%         \label{fig:M_ite}
%     \end{minipage}
%     ~
%     \begin{minipage}{0.5\linewidth}
%          \vspace{-5mm}
%         \centering
%   	    \includegraphics[width=1.0\linewidth]{Figure/M_pt.pdf}
%   	    \vspace{-5mm}
%   	    \caption{Empirical phase transition of the curves with (a) $M = 0$ and (b) $M = 1000$.}
%   	    \label{fig: M_pt}  
%     \end{minipage}
% \end{figure}

% \begin{figure}[h]
%     \begin{minipage}{0.5\linewidth}
%     \vspace{-4mm}
%     \centering
%      \begin{subfigure}[b]{0.48\textwidth}
%          \centering
%   	    \includegraphics[width=1.0\linewidth]{Figure/convergence_rate_p.pdf}
%   	    \vspace{-4.5mm}
%   	    \caption{}
%   	    \label{fig: M_ite_1} 
%      \end{subfigure}
%      ~
%      \begin{subfigure}[b]{0.48\textwidth}
%          \centering
%       	\includegraphics[width=1.0\linewidth]{Figure/convergence_rate.pdf}
%   	    \vspace{-4.5mm}
%   	    \caption{}
%   	    \label{fig: M_ite_2}  
%      \end{subfigure}
%      \vspace{-5mm}
%      \caption{The convergence rate with different $M$ when (a) $N<N^*$ and (b) $N>N^*$.}
%         \label{fig:M_ite}
%     \end{minipage}
%     ~
%     \begin{minipage}{0.4\linewidth}
%          \vspace{-5mm}
%         \centering
%   	    \includegraphics[width=1.0\linewidth]{Figure/M_pt.pdf}
%   	    \vspace{-5mm}
%   	    \caption{Empirical phase transition of the curves with (a) $M = 0$ and (b) $M = 1000$.}
%   	    \label{fig: M_pt}  
%     \end{minipage}
% \end{figure}

% \begin{wrapfigure}{r}{0.45\linewidth}
%         \centering
%   	    \includegraphics[width=1.0\linewidth]{Figure/M_pt_update.pdf}
%   	    \vspace{-6mm}
%   	    \caption{Empirical phase transition of the curves with (a) $M = 0$ and (b) $M = 1000$.}
%   	    \vspace{-3mm}
%   	    \label{fig: M_pt}
% \end{wrapfigure}

\textbf{(d) Increase of $\widetilde{\delta}$ slows down convergence.}  Figure \ref{fig: delta} shows that the convergence rate {becomes worse} when the variance of the unlabeled data $\widetilde{\delta}$ increases from $1$. When $\widetilde{\delta}$ is less than $1$, the convergence rate almost remains the same, which is consistent with our characterization in \eqref{eqn: p_convergence} that the convergence rate is linear in $\mu$. From the discussion after \eqref{eqn: definition_lambda}, $\mu$ increases as $\widetilde{\delta}$ increases from $1$ and stays constant when $\widetilde{\delta}$ is less than $1$.%and the change of $\widetilde{\delta}$ affects the value of $\mu$ defined in \eqref{eqn: definition_lambda}. One can see that the convergence stays the same when $\widetilde{\delta}$ is less than $1$, and a rapid  degeneration is observed when $\widetilde{\delta}$ is larger than 1 and keeps increasing, which verified our claims about \eqref{eqn: definition_lambda} and the dependency on $\mu$ in \eqref{eqn: p_convergence}.

\Revise{\textbf{(e) $\| \W[L] - \bfW^* \|_F/\|\bfW^* \|_F$ is improved as a linear function of $\hat{\lambda}$.}   Figure \ref{fig: lambda} shows that the relative errors of $\W[L]$ with respect to   $\bfW^*$ decrease almost linearly when $\hat{\lambda}$ increases, % in various labeled data amount, 
which is consistent with the theoretical result in  \eqref{eqn: p_convergence_*}. Moreover, when $\lambda$ exceeds a certain threshold positively correlated with $N$, the relative error increases rather than decreases. That is consistent with the analysis in  \eqref{eqn: thm1_condition1} that $\hat{\lambda}$  has an upper limit, and such a limit increases as $N$ increases.}

%In addition, there is an upper bound of feasible $\hat{\lambda}$, than which the relative error increase sharply when $\hat{\lambda}$ is greater. The upper bound is a positive function of the labeled data amount $N$, which verifies \eqref{eqn: thm1_condition1}.}

\textbf{(f) Unlabeled data reduce the sample complexity to learn $\bfW^*$.} Figure \ref{fig: M_pt} depicts %the comparison of 
the phase transition of {returning $\W[L]$}. %with different number of unlabeled data. 
For every pair of $d$ and $N$, we construct $100$ independent trials, and each trial is said to be successful if $\|\W[L]-\bfW^*\|_F/\| \bfW^* \|_F\le 10^{-2}$. \Revise{The white blocks correspond to the successful trials, while the block in black indicates all failures.} When $d$ increases, the required number of labeled data to learn $\bfW^*$ is linear in $d$. Thus, the sample complexity bound in \eqref{eqn: main_sample} is order-wise optimal for $d$. Moreover,  the phase transition line when $M=1000$ is below the one when $M=0$. Therefore, with unlabeled data, the required sample complexity of $N$ is reduced.    

\begin{figure}[h]
\vspace{-2mm}
    \begin{minipage}{0.29\linewidth}
        \centering
        \includegraphics[width=1.0\linewidth]{Figure/delta_c.pdf}
  	    \vspace{-4mm}
  	    \caption{Convergence rate with different $\hat{\delta}$.}
  	    \label{fig: delta}
    \end{minipage}
    ~
    \begin{minipage}{0.29\linewidth}
        \centering
        \includegraphics[width=1.0\linewidth]{Figure/lambda_number.pdf}
  	    \vspace{-4mm}
  	    \caption{\Revise{$\frac{\|\W[L] - \bfW^* \|_F}{\|\bfW^* \|_F}$ when $\hat{\lambda}$ and   $N$ change.}}
  	    \label{fig: lambda}
    \end{minipage}
    ~
    \begin{minipage}{0.40\linewidth}
        \centering
  	    \includegraphics[width=1.0\linewidth]{Figure/M_pt_update.pdf}
  	    \vspace{-4mm}
  	    \caption{Empirical phase transition of the curves with (a) $M = 0$ and (b) $M = 1000$.}
  	    \label{fig: M_pt}  
    \end{minipage}
    \vspace{-3mm}
\end{figure}

%Hence, one can see that the phase transition with unlabeled data (in Figure \ref{fig: M_pt}(b)) has a slightly large region than that without unlabeled data (in Figure \ref{fig: M_pt}(a)), which verified the improved sample complexity in Theorem \ref{Thm: sufficient_number}. Additionally, the curves in both the sub-figures are a linear function, which also verified that the dependence of sample complexity in Theorem \ref{Thm: sufficient_number} is order-wise optimal with respect to the input dimension $d$.
\vspace{-2mm}

\subsection{Image classification on augmented CIFAR-10 dataset}
\label{sec: result_practice}
\vspace{-2mm}
%In this section, the evaluation of 
We evaluate  self-training  on the augmented CIFAR-10 dataset, which has 50K labeled data. The unlabeled data are mined from 80 Million Tiny Images following the setup in \citep{CRSD19}\footnote{The codes are downloaded from https://github.com/yaircarmon/semisup-adv}, and additional 50K images are selected for each class, which is a total of 500K images, to form the unlabeled data. The self-training method is the same implementation as that in \citep{CRSD19}. $\lambda$ and $\widetilde{\lambda}$ is selected as ${N}/{(M+N)}$ and ${M}/{(N+M)}$, respectively, and the algorithm stops after $200$ epochs.
In Figure \ref{fig: real_accuracy}, the dash lines stand for the best fitting of the linear functions of $1/\sqrt{M}$ via the least square method. One can see that the test accuracy is improved by up to $7\%$ using unlabeled data, and the empirical evaluations match the theoretical predictions. Figure \ref{fig: real_rate} shows the convergence rate calculated based on the first $50$ epochs, and the convergence rate is almost a linear function of $1/\sqrt{M}$, as predicted by \eqref{eqn: p_convergence}.


\begin{figure}[h]
\vspace{-3mm}
\centering
     \begin{minipage}{0.45\linewidth}
                \centering
                \includegraphics[width=0.9\linewidth]{Figure/real_accuracy.pdf}
                \vspace{-2mm}
                \caption{The test accuracy against the number of unlabeled data}
                \label{fig: real_accuracy}
    \end{minipage}
    ~
    \begin{minipage}{0.45\linewidth}
                \centering
                \includegraphics[width=0.9\linewidth]{Figure/real_convergence.pdf}
                \caption{The convergence rate against the number of unlabeled data}
                \label{fig: real_rate}
    \end{minipage}
    \vspace{-2mm}
\end{figure}
\vspace{-4mm}

==> Thm1.tex <==
% Let us define $\overline{\bfW} = q\cdot \bfW^* + ( 1 - q )\cdot \bfW^{(0)}$, where $\W[0]$ denotes the initial point.
\iffalse
\begin{theorem}[Initialization]
\label{Thm: p_initialization}
     Assume  the number of samples of labeled data satisfies
     \begin{equation}\label{eqn: p_initial_sample}
         N = \Omega\big( p^2\mu^{4} K^3 d \log  q \big)
     \end{equation}
     for some large constant $q$ and $p\in[0,1]$, the tensor initialization method 
    outputs  ${\bfW}^{(0)}$  such that
    \begin{equation}\label{eqn: p_initialization}
        \| \bfW^{(0,0)} -\bfW^* \|_F  = \mathcal{O}\big(\frac{\sigma_K}{p\mu^{2}K}\big)
    \end{equation}
    with probability at least $1-q^{-d}$.
\end{theorem}
\begin{theorem}[Low labeled data regime]\label{Thm: p_convergence}
    Suppose $\W[0,0]$  satisfies \eqref{eqn: p_initialization}
    with
    \begin{equation}\label{eqn: p}
         \hat{\lambda}-\Theta\Big(\frac{1-M^{-{1}/{2}}}{\mu K^{1/2} }\Big) \cdot\hat{\lambda}
         \le p \le 
         \hat{\lambda}+\Theta\Big(\frac{1-M^{-{1}/{2}}}{\mu K^{1/2} }\Big) \cdot\hat{\lambda},
    \end{equation}
     where
    \begin{equation}\label{eqn: lambda_hat}
        \hat{\lambda} : =\frac{\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2}
        = \mathcal{O}\Big(\mu^{-1} \big(\frac{N}{K^3d \log q}\big)^{\frac{1}{2}}\Big),
    \end{equation}
    and 
    \begin{equation}\label{eqn: mu}
        \mu
        = \mu( \delta, \de) 
        = \frac{\lambda\delta^2+\w[\lambda]\de^2}{\lambda\rho(\delta)+\w[\lambda]\rho(\de)}.
    \end{equation}
    Then, if the number of samples in $\w[\mathcal{D}]$ further satisfies
    % \begin{equation}\label{eqn: p_main_sample}
    % \begin{split}
    %     &N= \Omega\Big( \varepsilon^{-2}\mu^{2}\big(\frac{\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2}\big)^2K^3 d\log q \Big),\\
    %     \end{split}
    % \end{equation}
    \begin{equation}\label{eqn: p_main_sample_M}
        \begin{split}
        M= \Omega \big(  \mu^2 \big( 1-  \hat{\lambda}\big)^2 K^3 d\log q \big),
        \end{split}
    \end{equation}
    the iterates $\{ \bfW^{(\ell,t)} \}_{\ell,t=1}^{L,T}$ converge to $\overline{\bfW}(\hat{\lambda})$ as 
    \begin{equation}\label{eqn: p_convergence}
        \begin{split}
            \| \W[L,T]-\overline{\bfW}(\hat{\lambda}) \|_F 
            \le& \bigg[\Big( 1-\frac{\Theta(1-M^{-{1}/{2}})}{\mu K^{1/2}} \Big)^T +\frac{\Theta(1-M^{-1/2})}{K} \bigg]^L \cdot \| \bfW^{(0,0)}-\overline{\bfW}(p) \|_2\\
            &+\Theta(1+M^{-{1}/{2}})\cdot \frac{1-\hat{\lambda}}{ K}\cdot \| \bfW^* - \bfW^{(0,0)} \|_F
        \end{split}
    \end{equation}
    % \begin{equation}\label{eqn: p_convergence}
    %     \begin{split}
    %         \lim_{\ell\to \infty, t\to \infty} 
    %         \| \W[\ell,t]-\overline{\bfW}(\hat{\lambda}) \|_F \le \Theta(1+M^{-{1}/{2}})\cdot \frac{1-\hat{\lambda}}{ K}\cdot \| \bfW^* - \bfW^{(0,0)} \|_F
    %     \end{split}
    % \end{equation}
    with probability at least $1-q^{-d}$, where $\overline{\bfW}(\hat{\lambda}) = \hat{\lambda}\bfW^* + (1-\hat{\lambda})\W[0,0]$.
\end{theorem}
\begin{corollary}\label{corollary: W*}
    Suppose $\hat{\lambda}$ can be $\Theta(\frac{1}{K})$ while all the conditions in Theorem \ref{Thm: p_convergence} still hold. Then, we have 
    \begin{equation}\label{eqn: p_convergence_*}
        \begin{split}
            \lim_{\ell\to \infty, t\to \infty} \| \W[\ell,t]-\bfW^* \|_F \le \Big(1-\Theta\big(\frac{1}{K^2}\big)\Big)\cdot \| \bfW^* - \bfW^{(0,0)} \|_F
        \end{split}
    \end{equation}
    with probability at least $1-q^{-d}$.
\end{corollary}
\fi
\begin{lemma}\label{lemma: rho_order}
    For ReLU activation function, we have $\rho(z) = \Theta(z^2)$ when $z$ is close to $0$, and $\rho(z) = \Omega(z^2)$ when $z>c$ for some large positive constant. Typically, $\max_{z>0} \rho(z) = 0.089$. 
\end{lemma}

Theorem \ref{Thm: p_convergence} indicates that  
the iterations converge to $\overline{\bfW}(\hat{\lambda})$, which is a weighted average of the ground truth $\bfW^*$ and the initial point $\WI$, up to an error bound that shown in the left-hand side of \eqref{eqn: p_convergence} provided two conditions hold. One condition is that the initial point $\WI$ is not far away from the ground truth up to a distance bounded by \eqref{eqn: p_initialization} with a large $p$ shown in \eqref{eqn: p}, and another one is that the number of unlabeled data $M$ is sufficiently large as shown in \eqref{eqn: p_main_sample_M}.
\\
\noindent
\textbf{Remark 1.1 (Parameter $\mu$):} From \eqref{eqn: mu}, we know $\mu$ is a function of $\delta$ and $\de$. From Lemma \ref{lemma: rho_order}, we know that $\rho(\delta)$ is in the order of $\delta^2$ when $\delta\to 0^+$ for any activation functions. Therefore, when $\delta$ and $\de$ are close to $0$, $\mu$ is a fixed constant. For Lipschitz continuous activation function, we have $\rho(\delta)<\mathcal{O}(\delta^2)$ when $\delta$ is sufficiently large. Hence, when $\delta$ and $\de$ are sufficiently large, increasing the value of $\de$ will lead to the increase of $\mu$, thus we need a higher requirement on the initial point from \eqref{eqn: p_initialization}, a larger $p$ from \eqref{eqn: p}, and a larger size of unlabeled data $M$ from \eqref{eqn: p_main_sample_M}.\\
\noindent
\textbf{Remark 1.2 (Parameter $p$):} From \eqref{eqn: p_initialization}, we know that $\|\WI - \bfW^*\|_F$ is a positive function of $p^{-1}$. If the lower bound of $p$ from \eqref{eqn: p} becomes smaller, then the algorithm can tolerate a larger range of initialization.  
\\
\noindent
\textbf{Remark 1.3 (Parameter $\hat{\lambda}$):} From \eqref{eqn: lambda_hat}, we know that the definition of $\hat{\lambda}$ is ${\lambda\delta^2}/{(\lambda\delta^2+\w[\lambda]\de^2)}$, and the value of $\hat{\lambda}$ should be less than $\mu^{-1}\sqrt{\frac{N}{K^3d\log q}}$. We can see that if we have a larger $N$, which means that the learning problems is accessible to a larger number of labeled data, the value of $\hat{\lambda}$ can be selected as a  larger number. With a larger $\hat{\lambda}$, the algorithm can tolerant a smaller number of unlabeled data from \eqref{eqn: p_main_sample_M} and $p$ from \eqref{eqn: p}, which thus suggests a less requirement on the initialization from \eqref{eqn: p_initialization}. Additionally, given a larger $\lambda$, the convergent point $\overline{\bfW}(\hat{\lambda})$ moves closer to the ground-truth $\bfW^*$, and the error bound between the convergence point and the iterates becomes smaller as well, which indicates that the iterates are closer to the ground-truth. \\
\noindent
\textbf{Remark 1.4 (parameter $M$):} When the number of labeled data $N$ is much less than $\mu^2K^3 d\log q$, where $\hat{\lambda}$ can only be as large as a small constant, then the number of unlabeled data needs to be at least in the order of $\mu^2 K^3 d \log q$ to guarantee the convergence from \eqref{eqn: p_main_sample_M}. 
In addition, suppose the training process is accessible to a larger size of unlabeled data $M$, the iterations converge faster to the convergent point from \eqref{eqn: p_convergence}.
Moreover, with a larger number of unlabeled data $M$, $p$ can achieve a smaller value while \eqref{eqn: p} still holds. Additionally, the error bound of the iteration $\W[\ell,t]$ and $\overline{\bfW}(\hat{\lambda})$ decreases as $M$ increases as well. 


\iffalse
\textbf{Remark 1.1 (Labeled data):} 
From \eqref{eqn: thm1_condition1}, we know that the $\hat{\lambda}$ bounded by $1/K$ and $\sqrt{N/N
^*}$ from below and above, respectively. To provide a meaningful bound, the number of labeled data needs to be at least $N^*/K^2$. 
In addition, since the value of $\hat{\lambda}$ should be less than $\sqrt{{N}/{N^*}}$,  the value of $\hat{\lambda}$ can be selected as a  larger number if we have a larger $N$. With a larger $\hat{\lambda}$, the algorithm can tolerant a smaller number of unlabeled data from \eqref{eqn: p_main_sample_M}. Moreover, given a larger $\hat{\lambda}$, the convergent point $\WL$ moves closer to the ground-truth $\bfW^*$, and the error bound between the convergence point and the iterates becomes smaller as well, which indicates that the iterates are closer to the ground-truth.
 
 
 
\textbf{Remark 1.2 (Unlabeled data):}
From \eqref{eqn: p_main_sample_M}, we can see that the number of unlabeled data needs to be at least in the order of $\mu^2(1-\hat{\lambda})^2K^3d\log q$ to provide analyzable performance.
In addition, suppose the training process is accessible to a larger size of unlabeled data $M$, the iterations converge faster to the convergent point from \eqref{eqn: p_convergence}.
Moreover, with a larger number of unlabeled data $M$, the range of $p$ to guarantee \eqref{eqn: p} enlarged, which indicates a larger range of initialization. Additionally, the error bound of the iteration $\W[\ell]$ and $\WL$ decreases as $M$ increases as well.

\textbf{Remark 1.3 (Initial weights):} From the definition of $p$ in \eqref{eqn: definition_p}, we know that $\|\W[0] - \bfW^*\|_F$ is a linear function of $p^{-1}$. 
Therefore, the constraint for $p$ in \eqref{eqn: p} is in fact the requirement of the initial weights $\W[0]$. From \eqref{eqn: p}, we know that the bounds of $p$ is the functions of $\hat{\lambda}$ and $M$. When the number of unlabeled data increases, the lower bound of $p$ becomes even smaller, and the upper bound becomes even larger, which indicates the range of selectable initial weights is enlarged as well. In contrast, given the same number of labeled data, if we choose a smaller $\hat{\lambda}$, then both the lower and upper bounds of $p$ decreases, which means that the region of selectable initial weights moves further away from the ground truth. It is equivalent to say that we need to select a small $\lambda$ such that $\hat{\lambda}$ is small as well to guarantee the learned model is improved over the initial model if the initialization is not good enough (far away from the ground truth weights $\bfW^*$). Moreover, the initialization can be found through tensor initialization, where the results are summarized in the following Lemma \ref{Thm: p_initialization}.
\begin{lemma}[Initialization]\label{Thm: p_initialization}
     Assuming the number of samples of labeled data satisfies
     \begin{equation}\label{eqn: p_initial_sample}
         N \ge  p^2 N^* 
     \end{equation}
     for some large constant $q$ and $p\in[0,1]$, the tensor initialization method 
    outputs  ${\bfW}^{(0)}$  such that
    \begin{equation}\label{eqn: p_initialization}
        \| \bfW^{(0)} -\bfW^* \|_F  \le \frac{\sigma_K}{p\cdot c(\kappa)\mu^{2}K}
    \end{equation}
    with probability at least $1-q^{-d}$.
\end{lemma}
\fi

\iffalse
\textbf{Remark 1.4 (Parameter $\mu$):} From \eqref{eqn: definition_lambda}, we know $\mu$ is a function of $\delta$ and $\de$. From the following Lemma \ref{lemma: rho_order} (in appendix), we know that $\rho(\delta)$ is in the order of $\delta^2$ when $\delta\to 0^+$ for ReLU activation functions. Therefore, when $\delta$ and $\de$ are close to $0$, $\mu$ is a fixed constant. Nonetheless, $\rho(\delta)$ is less than $\delta^2$ order-wisely when $\delta$ is sufficiently large. Hence, when $\delta$ and $\de$ are sufficiently large, increasing the value of $\de$ will lead to the increase of $\mu$, and thus we require a larger size of unlabeled data $M$ from \eqref{eqn: p_main_sample_M}. In this paper, we study the case that $\delta$ and $\de$ are relative small and fixed as constants.
\begin{lemma}\label{lemma: rho_order}
    For ReLU activation function, we have $\rho(z) = \Theta(z^2)$ when $z$ is close to $0$, and $\rho(z) = \Omega(z^2)$ when $z>c$ for some large positive constant. Typically, $\max_{z>0} \rho(z) = 0.089$. 
\end{lemma}

\fi

==> Thm1_old.tex <==
\section{Theoretical results: insufficient sample complexity}
% Let us define $\overline{\bfW} = q\cdot \bfW^* + ( 1 - q )\cdot \bfW^{(0)}$, where $\W[0]$ denotes the initial point.

\begin{theorem}[Initialization]
\label{Thm: p_initialization}
     Assume  the number of samples of labeled data satisfies
     \begin{equation}\label{eqn: p_initial_sample}
         N = \Omega\big( p^2\mu^{4} K^3 d \log  q \big)
     \end{equation}
     for some large constant $q$ and $p\in[0,1]$, the tensor initialization method 
    outputs  ${\bfW}^{(0)}$  such that
    \begin{equation}\label{eqn: p_initialization}
        \| \bfW^{(0)} -\bfW^* \|_F  = \mathcal{O}\big(\frac{\sigma_K}{p\mu^{2}K}\big)
    \end{equation}
    with probability at least $1-q^{-d}$, where $\overline{\bfW}(p) = p\cdot \bfW^* + ( 1 - p )\cdot \bfW^{(0)}$.
\end{theorem}
\begin{theorem}[Convergent point]\label{Thm: p_convergence}
    Let $\frac{\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2}=\Omega\big(\mu^{-1} (\frac{N}{K^3d \log q})^{\frac{1}{2}}\big)$.
     Suppose $\W[0]$ and $\overline{\bfW}(p)$ satisfy \eqref{eqn: p_initialization} 
     and the number of samples in $\w[\mathcal{D}]$ satisfy
    % \begin{equation}\label{eqn: p_main_sample}
    % \begin{split}
    %     &N= \Omega\Big( \varepsilon^{-2}\mu^{2}\big(\frac{\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2}\big)^2K^3 d\log q \Big),\\
    %     \end{split}
    % \end{equation}
    \begin{equation}\label{eqn: p_main_sample_M}
        \begin{split}
        M= \Omega \Big( \tilde{\varepsilon}^{-2} \big( \mu-  (\textstyle\frac{N}{K^3d \log q})^{\frac{1}{2}}\big)^2 K^3 d\log q \Big)
        \end{split}
    \end{equation}
    for some constant $\w[\varepsilon]\in (0, 1)$, where 
    \begin{equation}\label{eqn: mu}
        \mu
        = \mu( \delta, \de) 
        = \frac{\lambda\delta^2+\w[\lambda]\de^2}{\lambda\rho(\delta)+\w[\lambda]\rho(\de)}.
    \end{equation}
    Then, the iterates $\{ \bfW^{(t)} \}_{t=1}^{T}$ converge to the ground truth as 
    \begin{equation}\label{eqn: p_convergence}
        \begin{split}
            \| \W[T] -\overline{\bfW}(p) \|_F 
            \le& 
            \bigg[\Big(1- \Theta\big(\frac{1-\w[\varepsilon]}{\mu\sqrt{K}} 
            \big)\Big)^T + \w[\nu] \bigg]
            \| \W[0]-\overline{\bfW}(p) \|_F 
             + \nu \| \bfW^*-\overline{\bfW}(p) \|_F \\
            % & \| \W[0]-\overline{\bfW} \|_F
        \end{split}
    \end{equation}
    with probability at least $1-q^{-d}$, where
    \begin{equation}\label{eqn: nu}
        \nu = \frac{1}{1-\w[\varepsilon]}\cdot 
        \Big[
        \Theta\Big(\frac{\mu\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2}\Big) + \Theta\Big(\frac{1}{K}\Big)
        \Big],
    \end{equation}
    \begin{equation}\label{eqn: nu_tilde}
        \w[\nu] = \frac{1}{1-\w[\varepsilon]}\cdot 
        \Big[\Theta\Big(\frac{\mu\w[\lambda]\de^2}{\lambda\delta^2+\w[\lambda]\de^2}\Big)+\frac{\w[\varepsilon]}{K} \Big].
    \end{equation}
\end{theorem}
\begin{lemma}[Order analysis of $\rho$]
\label{lemma: rho_order}
    If $\rho(z)>0$ for $z\in(0, \xi)$ for some positive constant $\xi$ and the sub-gradient of $\rho(z)$ at $0$ can be non-zero,  then $\rho(z)=\Theta(z^r)$ when $z\to 0^+$.
\end{lemma}
\noindent
\textbf{Remark 1.1 (Influence of $\mu$):} From \eqref{eqn: mu}, we know $\mu$ is a function of $\delta$ and $\de$. From Lemma \ref{lemma: rho_order}, we know that $\rho(\delta)$ is in the order of $\delta^2$ when $\delta\to 0^+$ for any activation functions. Therefore, when $\delta$ and $\de$ are close to $0$, $\mu$ is a fixed constant. For Lipschitz continuous activation function, we have $\rho(\delta)<\mathcal{O}(\delta^2)$ when $\delta$ is sufficiently large. Hence, when $\delta$ and $\de$ are sufficiently large, increasing the value of $\de$ will lead to the increase of $\mu$, thus we need higher requirement on the initial point from \eqref{eqn: p_initialization} and slower convergence rate from \eqref{eqn: nu} and \eqref{eqn: nu_tilde} in terms of $\mu$. 

\noindent
\tcr{\textbf{Remark 1.2 (Influence of $M$):} 
When $N\ll K^3d$, the factor $\mu -\sqrt{\frac{N}{K^3d}}$ in \eqref{eqn: p_main_sample_M} is larger than $0$ and close to $\mu$. Therefore, with fixed $N$ and $N\ll K^3d$, to gaurantee \eqref{eqn: p_main_sample_M} hold, we need to increase $\w[\varepsilon]$ when $M$ decrease. From \eqref{eqn: nu_tilde}, we know that both $\nu$ and $\w[\nu]$ will increase accordingly, and thus the error term in  \eqref{eqn: p_convergence} will increase as well. Conversely, if we increase $M$, we can obtain smaller error bound, which means that
$\W[T]$ is closer to $\overline{\bfW}(p)$ and $\bfW^*$.}


\noindent
\tcr{\textbf{Remark 1.3 (Parameter $p$):} From \eqref{eqn: p_initialization} and \eqref{eqn: p_convergence}, we know that the best convergent point, where in terms of the distance to $\bfW^*$, returned by gradient descent method is $\overline{\bfW}(p_{\max})$, where $p_{\max}$ is the maximum value of $p$ while \eqref{eqn: p_initial_sample} still holds.
When $N = \Omega(\mu^4K^3d\log q)$, $p$ can be as large as $1$, which suggests that $\overline{\bfW}$ can be $\bfW^*$. However, when $N$ is small, we have $p_{\max}=\Theta(\mu^{-2}(\frac{N}{K^3d})^{\frac{1}{2}})$. Given a fixed initial point $\bfW^{(0)}$, The achievable weights with the smallest distance to $\bfW^*$ are $\overline{\bfW}(p_{\max})$. Also, with larger $N$, $\overline{\bfW}(p_{\max})$ is closer to $\bfW^*$.
}

\noindent
\tcr{\textbf{Remark 1.4 (Convergence analysis):} Suppose we have a good initial point, such that $p$ can be as large as $1$, which means that $\overline{\bfW}(p_{\max})$ can be $\bfW^*$ from Remark 1.3. However, with a small $N$ such that $N\ll K^3d$,  the iterates cannot guarantee to be arbitrarily close to $\overline{\bfW}(p_{\max})$, either. 
First, $\w[\nu]$ needs to be at least less than $1$ to gaurantee the outer loop can converge from \eqref{eqn: p_convergence}. Then, 
we know that $\frac{\w[\lambda]\de^2}{\lambda\delta^2+\w[\lambda]\de^2}$ needs to be smaller than $\Theta(\mu^{-1})$ from \eqref{eqn: nu_tilde}. However, it is equivalent to require $\frac{\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2}$ in the order of $1- \mathcal{O}(\mu^{-1})$, which contracts the statement in Theorem \ref{Thm: p_convergence} given $N\ll {K^3d}$. The details about analysis with $N=\Omega({K^3d})$ will be discussed in the following paragraphs.
}

\iffalse
\noindent
\tcr{\textbf{Remark 1.1 (Influence of $M$):} Since $\varepsilon$ can only be as large as a constant, it is clear that $\frac{\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2} = \mathcal{O}\big(\mu\sqrt{\frac{N}{K^3d}}\big)$ from \eqref{eqn: p_main_sample}, and $\frac{\w[\lambda]\de^2}{\lambda\delta^2+\w[\lambda]\de^2}$ needs to be in the order of $1-\mathcal{O}\big(\mu\sqrt{\frac{N}{K^3d}}\big)$. 
When $N\ll K^3d$, we know that $1-\mathcal{O}\big(\mu\sqrt{\frac{N}{K^3d}}\big)$ is lower-bounded and close to $1$. Therefore, with fixed $N$, if $M$ decreases, $\w[\varepsilon]$  will increase while $\w[\lambda]$ needs to stay the same. From \eqref{eqn: nu_tilde}, we know that $\w[\nu]$ will increase accordingly, and thus the error term in  \eqref{eqn: p_convergence} will increase as well. Conversely, if we increase $M$, we can obtain smaller error bound, and $\W[T]$ is closer to $\overline{\bfW}(p)$ and $\bfW^*$.}


\noindent
\tcr{\textbf{Remark (Parameter $p$):} From \eqref{eqn: p_initialization} and \eqref{eqn: p_convergence}, we know that the best convergent point, where in terms of the distance to $\bfW^*$, returned by gradient descent method is $\overline{\bfW}(p_{\max})$, where $p_{\max}$ is the maximum value of $p$ while \eqref{eqn: p_initial_sample} still holds.
When $N = \Omega(\mu^{-4}K^3d\log q)$, $p$ can be as large as $1$, which suggests that $\overline{\bfW}$ can be $\bfW^*$. However, when $N$ is small, we have $p_{\max}=\Theta(\mu^2\sqrt{\frac{N}{K^3d}})$. Given a fixed initial point $\bfW^{(0)}$, The achievable weights with the smallest distance to $\bfW^*$ are $\overline{\bfW}(p_{\max})$. Also, with larger $N$, $\overline{\bfW}(p_{\max})$ is closer to $\bfW^*$.
However, even we have a good initial point, such that $p$ can be $1$. With small $N$,  the iterates cannot guarantee to be arbitrarily close to $\overline{\bfW}(p_{\max})$, either. 
To guarantee that $\w[\nu]$ is less than $1$ and thus the outer loop can converge, we know that $\frac{\w[\lambda]\de^2}{\lambda\delta^2+\w[\lambda]\de^2}$ needs to be smaller than $\Theta(\mu)$ from \eqref{eqn: p_main_sample} and  \eqref{eqn: p_convergence}. However, it is equivalent to require $\frac{\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2}$ in the order of $1- \mathcal{\mu}$, which is a constant and $N$ still needs to be in the order of $K^3d\log q$.
}
\fi

==> Thm1_wrong.tex <==
\newpage
\section{Theoretical results: insufficient sample complexity}
\begin{theorem}
    
    Suppose the initial point $\W[0, 0]$ satisfies 
    \begin{equation}\label{eqn: p_initial_point}
        \|\bfW^* -\W[0,0] \| = \mathcal{O}\big( \frac{\mu^2\sigma_K}{p^2 K} \big)  \text{ for some $p\in(0,1]$}.
    \end{equation}
    Then, if the following conditions 
    \begin{equation}\label{eqn: p_condition1}
    \nu_1\cdot(1-p)+\w[\nu]_1\cdot p < 1,    
    \end{equation}
    \begin{equation}\label{eqn: p_main_sample}
    \begin{split}
        &N= \Omega\Big( \varepsilon^{-2}\mu^{-2}\big(\frac{\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2}\big)^2K^3 d\log q \Big),\\
        \end{split}
    \end{equation}
    \begin{equation}\label{eqn: p_main_sample_M}
        \begin{split}
        \text{and}&\quad 
        M= \Omega\Big(\tilde{\varepsilon}^{-2}\mu^{-2}\big(\frac{\w[\lambda]\de^2}{\lambda\delta^2+\w[\lambda]\de^2}\big)^2 K^3 d\log q\Big).
        \end{split}
    \end{equation}
    hold
    for some constant $\varepsilon$, $\w[\varepsilon]\in (0, \frac{1}{2})$,
    we have
    \begin{equation}
        \lim_{\ell\to \infty, t\to \infty} \| \W[\ell,t]-\overline{\bfW}(p) \|_F \le \frac{1}{1-\varepsilon-\w[\varepsilon]}\cdot \frac{\nu_1 (1-p)}{\nu_1 (1-p) + \w[\nu]_1 p } \|\bfW^* -\W[0,0]\|_F
    \end{equation}
    with probability at least $1-q^{-d}$, 
    where
    \begin{equation}\label{eqn: mu}
        \mu
        = \mu( \delta, \de) 
        = \frac{\lambda\rho(\delta)+\w[\lambda]\rho(\de)}{\lambda\delta^2+\w[\lambda]\de^2},
    \end{equation}
    \begin{equation}\label{eqn: nu1}
        \nu_1 = \Theta\Big(\frac{\lambda\delta^2}{\mu(\lambda\delta^2+\w[\lambda]\de^2)}\Big) + \frac{\varepsilon}{ K},
    \end{equation}
    \begin{equation}\label{eqn: nu1_tilde}
        \text{and \quad} \w[\nu]_1 = \Theta\Big(\frac{\w[\lambda]\de^2}{\mu(\lambda\delta^2+\w[\lambda]\de^2)}\Big) + \frac{\w[\varepsilon]}{ K}.
    \end{equation}
\end{theorem}

\noindent
\textbf{Remark 1 (Conditions for \eqref{eqn: p_condition1}):} Since $\varepsilon$ can only be as large as a constant, it is clear that $\frac{\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2} = \mathcal{O}\big(\mu\sqrt{\frac{N}{K^3d}}\big)$ from \eqref{eqn: p_main_sample}. When $N\ll K^3d$, we know $\frac{\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2}$ is a small positive constant, and $\frac{\w[\lambda]\de^2}{\lambda\delta^2+\w[\lambda]\de^2}$ is close to $1$. Therefore, we have $\w[\nu]_1\in\Theta(\mu^{-1})$, and $p$ needs to be less than $\mu$ in order to guarantee $\w[\nu]_1 p $ is small and thus \eqref{eqn: p_condition1} holds. Therefore, even we are given a good initial point such that $p$ can be $1$ in \eqref{eqn: p_initial_point}, without enough samples in $\mathcal{D}$, we cannot guarantee the algorithm converges to $\overline{\bfW}(1)$, which is actually the ground truth $\bfW^*$, but $\overline{\bfW}(\mu)$ at best (w.r.t the distance to the ground truth).

\noindent
\textbf{Remark 2 (Influence of $M$):} 

==> Thm2.tex <==
\begin{theorem}\label{Thm: sufficient_number}
    Suppose $\bfW^{(0)}$ satisfies \eqref{eqn: p_initialization} with $p=1$ and the number of samples in $\mathcal{D}$ and $\w[\mathcal{D}]$ satisfy
    \begin{equation}\label{eqn:main_sample}
    \begin{split}
        &N= \Omega\big( \mu^{2}\hat{\lambda}^2K^3 d\log q \big),
        \quad
        \text{and}\quad 
        M= \Omega\big(\mu^{2}(1-\hat{\lambda})^2 K^3 d\log q\big).
        \end{split}
    \end{equation}
     where
    \begin{equation}\label{eqn: lambda_hat_s}
        \hat{\lambda} : =\frac{\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2}
        = 1 - \mathcal{O}\big(\frac{1}{\mu\sqrt{K}}\big). 
    \end{equation}
    Then, the iterates $\{ \bfW^{(\ell,t)} \}_{\ell=1, t=1}^{L, T}$ converge to the ground truth as 
    \begin{equation}\label{eqn: convergence}
        \| \W[L,T] -\bfW^* \|_F \le \big( \nu_1^T(\beta) + \nu_2 \big)^L 
        \| \W[0,0]-\bfW^* \|_F,
    \end{equation}
    where 
    \begin{equation}\label{eqn: convergence_rate}
    \begin{split}
        &\nu_1(\beta^*) = 1- \Theta
        \Big(
        \frac{1-\Theta(\frac{\hat{\lambda}}{\sqrt{N}})-\Theta(\frac{1-\hat{\lambda}}{\sqrt{M}})}{\mu\sqrt{K}} 
        \Big),\\
        % \nu_2 = \Theta\Big( \frac{\w[\varepsilon]\mu}{\sqrt{K}}\Big) + \Theta\Big( \frac{\w[\lambda]\de^2}{\lambda\delta^2+\w[\lambda]\de^2} \Big).
        &\tcr{\nu_2 =  \Theta\Big(1+\Theta\big(\frac{\hat{\lambda}}{\sqrt{N}}\big)+\Theta\big(\frac{1-\hat{\lambda}}{\sqrt{M}}\big)\Big)\cdot\mu\sqrt{K}(1-\hat{\lambda}).}
    \end{split}
    \end{equation}
\end{theorem}

Theorem \ref{Thm: sufficient_number} indicates that the iterates returned by Algorithm \ref{Algorithm: Alg1} converge to the ground truth $\bfW^*$ with exponential decay as long as the number of samples satisfy \eqref{eqn:main_sample} with $\hat{\lambda}$ meeting \eqref{eqn: lambda_hat_s}. The linear convergence rates of the inner loop and outer loop are denoted as $\nu_1$ and $\nu_2$ as shown in \eqref{eqn: convergence_rate}.
\\
\noindent
\textbf{Remark 2.1 (Parameter $N$):}
Suppose we do not have unlabeled data, which is equivalent to say that $\hat{\lambda} =1$, the required number of samples are in the order of $\mu^{2}K^3d \log q$.  Therefore, the sample complexity of $N$ can be reduced by a factor of $\hat{\lambda}$ at the cost of a slower convergence rate, where $\nu_1$ in \eqref{eqn: convergence_rate} has an additional factor of $\frac{1-\hat{\lambda}}{\sqrt{M}}$ and $\nu_2$ is non-zero as $\hat{\lambda}$ is less than $1$ compared with training without unlabeled data.  

\noindent
\textbf{Remark 2.2 (Convergence rate $\nu_1$ and $\nu_2$):} 
From \eqref{eqn: convergence_rate}, we know that both the convergence rates decrease, which indicates a faster convergence rate, if either $N$ or $M$ increases. While if  $\mu$ increases, both the values of $\nu_1$ and $\nu_2$ will increase, which suggests a slower convergence rate.
Additionally, given $N$ and $M$ are in the same order as shown in \eqref{eqn:main_sample}, only $\nu_2$ depends on $\hat{\lambda}$ and is a negative function of $\hat{\lambda}$. Therefore, if we increase the value of $\hat{\lambda}$, algorithms will enjoy a faster convergence rate, however, which also suggests a larger number of labeled data $N$. 
 
\iffalse
\noindent
\textbf{Remark 2.1 (Range of $\lambda$):} From \eqref{eqn: convergence}, we know that $\nu_2$ needs to be less than $1$ in order to guarantee the convergence to $\bfW^*$. Therefore, $\w[\lambda]=\mathcal{O}(\mu^{-1}K^{-1/2})$ and $\lambda=1-\mathcal{O}(\mu^{-1}K^{-1/2} )$.

\noindent
\textbf{Remark 2.2 (Influence of $M$ and $N$):}  Suppose we do not have unlabeled data, which is equivalent to say that $\w[\lambda] =0$, the required number of samples are in the order of $\varepsilon^{-2}\mu^{-2}K^3d \log q$ with $\varepsilon\in(0,1)$. When we are accessible to infinite number of unlabeled samples, where $\w[\varepsilon]$ can be arbitrary close to $0$, the sample complexity of $N$ is reduced by a factor of $\big(\frac{\lambda\delta^2}{\lambda\delta^2 + \w[\lambda] \de^2}\big)^2$ with $\varepsilon\in(0,1)$. From another point of view, with fixed $\de$, $\varepsilon$ and $\w[\varepsilon]$ are in the order of $\frac{1}{\sqrt{N}}$ and $\frac{1}{\sqrt{M}}$. Thus, increase the value of $M$  or $N$ will lead to the decrease of $\nu_1$ and $\nu_2$ and thus faster convergence rate.



\noindent
\textbf{Remark 2.3 (Influence of $\de$):} The value of $\de$ will directly control the values of $\varepsilon$, $\w[\varepsilon]$ and $\nu$, and thus the sample complexity and convergence rate are affected. When $\de$ and $\delta$ are fixed or relative small,  $\mu$ is a fixed constant. 
With fixed finite number of samples $M$ and $N$, $\varepsilon$ and $\w[\varepsilon]$ are in the order of  $\frac{\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2}$ and $\frac{\w[\lambda]\de^2}{\lambda\delta^2+\w[\lambda]\de^2}$, respectively. Hence, changing the value of $\de$ will not affect the sum of $\varepsilon$ and $\w[\varepsilon]$, and the convergence rate of the inner loop $\nu_1$ stays the same as well. On contrast, the value of $\nu_2$ decreases as $\de$ decreases, thus the convergence rate of the outer loop, which is $\nu_1^T+\nu_2$, will become faster if we decrease the value of $\de$. However, $T$ is usually a relatively small number in training \tcr{(citation)}, and thus the value of $\nu_1$ plays a more important role in determining the convergence rate of the outer loop. Thus, decreasing the value of $\de$ when $\de$ is already close to $0$ will only increase the convergence rate of the outer loop slightly. Moreover, suppose we have the infinite number of unlabeled data, that is $M$ is sufficiently large, and $\w[\varepsilon]$ can be arbitrarily close to $0$. Decreasing the value of $\de$ will lead to the higher requirement on the sample complexity of labeled data $N$ with $\varepsilon\in(0,1)$. 
\fi

==> Thm2_old.tex <==
\section{Theoretical results: sufficient number of samples}
\subsection{Local convex region}
\begin{equation}\label{eqn: initialization}
    \|\bfW-\bfW^*\|_F\lesssim \frac{\sigma_K}{\mu^2 K}
\end{equation}
\tcr{\begin{lemma}[Initialization]\label{Thm: initialization}
    Assume  the number of samples $N = \Omega\big( \mu^{4} K^3 d \log  q \big)$ for some large constant $q$, the tensor initialization method 
    outputs  $\bfW^{(0,0)}$  such that \eqref{eqn: initialization} holds, i.e., $\| \bfW^{(0,0)} -\bfW^* \|_F  = \mathcal{O}\big(\frac{\sigma_K}{\mu^2K}\big)$ with probability at least $1-q^{-d}$.
%	\end{equation}
\end{lemma}}


\subsection{Convergence analysis}
\begin{theorem}\label{Thm: sufficient_number}
    Suppose $\bfW^{(0)}$ satisfies \eqref{eqn: initialization} and the number of samples in $\mathcal{D}$ and $\w[\mathcal{D}]$ satisfy
    \begin{equation}\label{eqn:main_sample}
    \begin{split}
        &N= \Omega\big( \varepsilon^{-2}\mu^{2}\hat{\lambda}^2K^3 d\log q \big),\\
        \end{split}
    \end{equation}
    \tcr{\begin{equation}
        \begin{split}
        \text{and}&\quad 
        M= \Omega\big(\tilde{\varepsilon}^{-2}\mu^{2}(1-\hat{\lambda})^2 K^3 d\log q\big).
        \end{split}
    \end{equation}}
    for some constant $\varepsilon$, $\w[\varepsilon]>0$ with $\varepsilon+\w[\varepsilon]<1$.
    Then, the iterates $\{ \bfW^{(\ell,t)} \}_{\ell=1, t=1}^{L, T}$ converge to the ground truth as 
    \begin{equation}\label{eqn: convergence}
        \| \W[L,T] -\bfW^* \|_F \le \big( \nu_1^T(\beta) + \nu_2 \big)^L 
        \| \W[0,0]-\bfW^* \|_F,
    \end{equation}
    where 
    \begin{equation}
    \begin{split}
        &\nu_1(\beta^*) = 1- \Theta
        \Big(
        \frac{1-\varepsilon-\w[\varepsilon]}{\mu\sqrt{K}} 
        \Big),
        \text{and}\quad
        % \nu_2 = \Theta\Big( \frac{\w[\varepsilon]\mu}{\sqrt{K}}\Big) + \Theta\Big( \frac{\w[\lambda]\de^2}{\lambda\delta^2+\w[\lambda]\de^2} \Big).
        \tcr{\nu_2 =  \Theta\Big(\frac{\mu\sqrt{K} \hat{\lambda}}{1-\varepsilon-\tilde{\varepsilon}}\Big).}
    \end{split}
    \end{equation}
\end{theorem}
\noindent
\textbf{Remark 2.1 (Range of $\lambda$):} From \eqref{eqn: convergence}, we know that $\nu_2$ needs to be less than $1$ in order to guarantee the convergence to $\bfW^*$. Therefore, $\w[\lambda]=\mathcal{O}(\mu^{-1}K^{-1/2})$ and $\lambda=1-\mathcal{O}(\mu^{-1}K^{-1/2} )$.

\noindent
\textbf{Remark 2.2 (Influence of $M$ and $N$):}  Suppose we do not have unlabeled data, which is equivalent to say that $\w[\lambda] =0$, the required number of samples are in the order of $\varepsilon^{-2}\mu^{-2}K^3d \log q$ with $\varepsilon\in(0,1)$. When we are accessible to infinite number of unlabeled samples, where $\w[\varepsilon]$ can be arbitrary close to $0$, the sample complexity of $N$ is reduced by a factor of $\big(\frac{\lambda\delta^2}{\lambda\delta^2 + \w[\lambda] \de^2}\big)^2$ with $\varepsilon\in(0,1)$. From another point of view, with fixed $\de$, $\varepsilon$ and $\w[\varepsilon]$ are in the order of $\frac{1}{\sqrt{N}}$ and $\frac{1}{\sqrt{M}}$. Thus, increase the value of $M$  or $N$ will lead to the decrease of $\nu_1$ and $\nu_2$ and thus faster convergence rate.



\noindent
\textbf{Remark 2.3 (Influence of $\de$):} The value of $\de$ will directly control the values of $\varepsilon$, $\w[\varepsilon]$ and $\nu$, and thus the sample complexity and convergence rate are affected. When $\de$ and $\delta$ are fixed or relative small,  $\mu$ is a fixed constant. 
With fixed finite number of samples $M$ and $N$, $\varepsilon$ and $\w[\varepsilon]$ are in the order of  $\frac{\lambda\delta^2}{\lambda\delta^2+\w[\lambda]\de^2}$ and $\frac{\w[\lambda]\de^2}{\lambda\delta^2+\w[\lambda]\de^2}$, respectively. Hence, changing the value of $\de$ will not affect the sum of $\varepsilon$ and $\w[\varepsilon]$, and the convergence rate of the inner loop $\nu_1$ stays the same as well. On contrast, the value of $\nu_2$ decreases as $\de$ decreases, thus the convergence rate of the outer loop, which is $\nu_1^T+\nu_2$, will become faster if we decrease the value of $\de$. However, $T$ is usually a relatively small number in training \tcr{(citation)}, and thus the value of $\nu_1$ plays a more important role in determining the convergence rate of the outer loop. Thus, decreasing the value of $\de$ when $\de$ is already close to $0$ will only increase the convergence rate of the outer loop slightly. Moreover, suppose we have the infinite number of unlabeled data, that is $M$ is sufficiently large, and $\w[\varepsilon]$ can be arbitrarily close to $0$. Decreasing the value of $\de$ will lead to the higher requirement on the sample complexity of labeled data $N$ with $\varepsilon\in(0,1)$. 

==> algorithm.tex <==
\subsection{Algorithm}\label{sec: algorithm}
We consider an iterative self-training method such as \citep{Lee13}, which can be divided into   steps: 



\begin{enumerate}
    \item Initial $\ell =0$ and obtain a  model $\W[\ell]$, denoted as the teacher model,   using labeled data $\mathcal{D}$ only;
%\noindent   For $\ell = 0 , 1, \cdots, L-1$
    \item Use the teacher model    to calculate  pseudo labels $\w[y]_m$ of unlabeled data in $\w[\mathcal{D}]$. %=\{\w[\bfx]_m \}_{m=1}^M$. 
    \item Train the neural network by solving (\ref{eqn: empirical_risk_function}) %via minimizing the objective function as shown in \eqref{eqn: empirical_risk_function} 
    via $T$-step  mini-batch stochastic gradient descent method using disjoint subsets $\{\mathcal{D}_t\}_{t=0}^{T-1}$ and $\{\widetilde{\mathcal{D}}_t\}_{t=0}^{T-1}$. Let $\W[\ell]$ denote the obtained student model. 
    \item Use $\W[\ell]$ as the current teacher model. Let $\ell=\ell+1$ and go back to step 2.
\end{enumerate}
The pseudocode of the self-training method is summarized in Algorithm
\ref{Algorithm: Alg1}.
\begin{algorithm}[h]
	\caption{Mini-batch stochastic gradient Descent Algorithm}\label{Algorithm: Alg1}
	\begin{algorithmic}
		\State \textbf{Input:} labeled $\mathcal{D}=\{(\bfx_n, y_n) \}_{n=1}^{N}$,  
		 unlabeled data $\w[\mathcal{D}]=\{\widetilde{\bfx}_m \}_{m=1}^{M}$,
		gradient step size $\eta$;
		\State \textbf{Initialization:} preliminary teacher model with weights $\bfW^{(0)}$;
		\State \textbf{Partition:} divide $\mathcal{D}$ and $\widetilde{\mathcal{D}}$ into $T$ disjoint subsets $\{ \mathcal{D}_t \}_{t=0}^{T-1}$ and $\{\widetilde{\mathcal{D}}_t\}_{t = 0}^{T-1}$, respectively; \For{$\ell = 0 , 1, \cdots, L-1$}
		    \State 1. Use the estimated teacher model $\bfW^{(\ell)}$ to generate pseudo labels for $\{\widetilde{\bfx}_m\}_{m=1}^M$:
		    \State \qquad $y_m = g(\bfW^{(\ell)};\w[\bfx]_m)$ for $m =1, 2, \cdots, M$;
		    \State 2. Obtain the student model ${\bfW}$ through minimizing \eqref{eqn: empirical_risk_function} via  mini-batch stochastic gradient descent method using $\mathcal{D}_t$ and $\widetilde{\mathcal{D}}_t$;
		    \State 3. Update the new teacher model  as the obtained student model: \qquad $\bfW^{(\ell+1)} = \bfW$;
		 \EndFor
	\end{algorithmic}
\end{algorithm}


==> useful_lemmas.tex <==
% \section{Useful Lemmas}
% In this section, we present some useful lemmas that are used for proving the theorems in the main contexts.  


% \begin{lemma}\label{lemma: rho_order}
%     For ReLU activation function, we have $\rho(z) = \Theta(z^2)$ when $z$ is close to $0$, and $\rho(z) = \Omega(z^2)$ when $z>c$ for some large positive constant. Typically, $\max_{z>0} \rho(z) = 0.089$. 
% \end{lemma}




